Robust Learning Meets Generative Models: Can Proxy Distributions Improve Adversarial Robustness?

While additional training data improves the robustness of deep neural networks against adversarial examples, it presents the challenge of curating a large number of specific real-world samples. We circumvent this challenge by using additional data from proxy distributions learned by advanced generative models. We first seek to formally understand the transfer of robustness from classifiers trained on proxy distributions to the real data distribution. We prove that the difference between the robustness of a classifier on the two distributions is upper bounded by the conditional Wasserstein distance between them. Next we use proxy distributions to significantly improve the performance of adversarial training on five different datasets. For example, we improve robust accuracy by up to 7.5% and 6.7% in $\ell_{\infty}$ and $\ell_2$ threat model over baselines that are not using proxy distributions on the CIFAR-10 dataset. We also improve certified robust accuracy by 7.6% on the CIFAR-10 dataset. We further demonstrate that different generative models bring a disparate improvement in the performance in robust training. We propose a robust discrimination approach to characterize the impact of individual generative models and further provide a deeper understanding of why current state-of-the-art in diffusion-based generative models are a better choice for proxy distribution than generative adversarial networks.

==> Proxy distributions [ICLR 2022]/macros.tex <==
\newcommand{\OblFt}{\mathbf{OblFtrSel}}
\newcommand{\FullFt}{\mathbf{FullFtrSel}}

\newcommand{\OblRisk}{\mathbf{OblRisk}}
\newcommand{\FullRisk}{\mathbf{FullRisk}}

\newcommand{\LearnFtr}{\mathsf{FtrSelector}}
\newcommand{\inj}{\mathsf{inj}}
\newcommand{\elim}{\mathsf{elim}}
\newcommand{\sub}{\mathsf{sub}}

\newcommand{\add}{\mathsf{add}}
\newcommand{\rem}{\mathsf{rem}}
\newcommand{\flip}{\mathsf{flip}}


\newcommand{\pop}{\mathsf{pop}}
\newcommand{\targ}{\mathsf{targ}}

\newcommand{\Advan}{\mathrm{Adv}}


\newcommand{\SaeedNote}[1]{{[{\color{teal} \bf Saeed: #1}]}}
\newcommand{\Snote}[1]{\SaeedNote{#1}}


% \newcommand{\nicholas}[1]{{[{\color{green} \bf Nicholas: #1}]}}



% \usepackage{enumitem}

% \usepackage{centernot}
% \DeclareMathOperator*{\argmax}{arg\,max}
% \DeclareMathOperator*{\argmin}{arg\,min}
\newcommand{\fot}{\bff}
\newcommand{\fto}{\bfg}
\newcommand{\htet}{\hat{\theta}}

\newcommand{\fhat}[2]{\ifthenelse{\equal{#2}{}}{\hat{f}(#1)}{\ifthenelse{\equal{#2}{0}}{\hat{f}(\emptyset)}{\hat{f}(#1_{\leq #2})}}}
\newcommand{\ftild}[2]{\ifthenelse{\equal{#2}{}}{\tilde{f}(#1)}{\ifthenelse{\equal{#2}{0}}{\tilde{f}(\emptyset)}{\tilde{f}(#1_{\leq #2})}}}
\newcommand{\ftildstar}[2]{\ifthenelse{\equal{#2}{}}{\tilde{f^*}(#1)}{\ifthenelse{\equal{#2}{0}}{\tilde{f^*}(\emptyset)}{\tilde{f^*}(#1_{\leq #2})}}}
\newcommand{\ghat}[2]{\ifthenelse{\equal{#2}{}}{\hat{g}(#1)}{\ifthenelse{\equal{#2}{0}}{\hat{g}(\emptyset)}{\hat{g}(#1_{\leq #2})}}}
\newcommand{\mfix}[2]{\ifthenelse{\equal{#2}{}}{m(#1)}{\ifthenelse{\equal{#2}{0}}{m(\emptyset)}{m(#1_{\leq #2})}}}


\newcommand{\fapp}[2]{\ifthenelse{\equal{#2}{}}{\tilde{f}(#1)}{\ifthenelse{\equal{#2}{0}}{\tilde{f}(\emptyset)}{\tilde{f}(#1_{\leq #2})}}}

\newcommand\aug{\hspace{-2.5mm}\rule[-1mm]{0.1mm}{4.5mm}\hspace{-2.5mm}}
\newcommand\augp{\hspace{-2.5mm}\rule[-2mm]{0.1mm}{5mm}\hspace{-2.5mm}}
\newcommand\augt{\hspace{-2.5mm}\rule[-1mm]{0.1mm}{5mm}\hspace{-2.5mm}}
\newcommand{\concatt}[4]{\begin{bmatrix}
\vspace{-5mm}\\
   #1&\augp&#2\\
   #3&\augt&#4\\
   \vspace{-5mm}\\
    \end{bmatrix}}
\newcommand{\concat}[2]{\begin{bmatrix}
\vspace{-5mm}\\
   #1&
   \aug
   &#2\\
   \vspace{-5mm}\\
    \end{bmatrix}}
\newcommand{\concatv}[2]{\begin{bmatrix}
   #1\\
   #2\\
    \end{bmatrix}}
    
    \newcommand{\concatvv}[3]{\begin{bmatrix}
   #1\\
   #2\\
   #3\\
    \end{bmatrix}}

%\newcommand{\gain}[2]{\ifthenelse{\equal{#2}{}}{g[#1]}{g[#1_{\leq #2}]}}


% CONVENTION for VECTOR and DISTRIBUTION notation:  
%For x,y,z, use \xDist \yDist etc to get their distribution, for d exceptionally use just \dist. for their vector version add Vec at the end of these operations or just get \xVec to get the vector that is not a distribution
%\newcommand{\againAp}[2]{\ifthenelse{\equal{#2}{}}{\tilde{g}({#1})}{\ifthenelse{\equal{#2}{0}}{\tilde{g}(\emptyset)}{\tilde{g}({#1}_{\leq #2})}}}
\renewcommand{\t}{\mathsf{t}}
% \renewcommand{\Case}{\mathrm{C}}
\newcommand{\Otilde}{\wt{O}}
\newcommand{\PrTam}{\mathsf{PT}}

\newcommand{\metric}{{{\mathsf{d}}}}
\newcommand{\metr}{\metric}
\newcommand{\Ball}{\mathcal{B}all}
\newcommand{\Sph}{\mathcal{S}phr}

\newcommand{\diam}{\mathsf{Diam}}
% \usepackage[utf8]{inputenc}
\newcommand{\Levy}{Lévy\xspace}
\newcommand{\Lovasz}{Lovász\xspace}
\newcommand\numberthis{\addtocounter{equation}{1}\tag{\theequation}}
\newcommand{\paragcompact}[1]{\noindent{\bf #1}}

%\newcommand{\parag}[1]{\noindent{\bf #1}}
%\renewcommand{\paragraph}[1]{\parag{#1}}
\newcommand{\distdist}{\mathfrak{D}}

%\newcommand{\Y}{\ensuremath{\mathcal{Y}}\xspace} % X
%\newcommand{\X}{\ensuremath{\mathcal{X}}\xspace} % X

\newcommand{\HD}{\mathsf{HD}}
\newcommand{\con}{{\bm \upalpha}}
\newcommand{\ERM}{\mathsf{ERM}}

\newcommand{\msr}{{\bm{\upmu}}}
\newcommand{\CentDist}{{\bm{\upsigma}}}

\newcommand{\OnlTam}{\mathsf{On}\Tam}
\newcommand{\OnTam}{\OnlTam}
\newcommand{\OffTam}{\mathsf{Off}\Tam}
%\newcommand{\OnlTam}{\OnlTam}
%\newcommand{\OnTam}{\OnTam}
%\newcommand{\OffTam}{\OffTam}

\newcommand{\mal}{\wt}
\newcommand{\X}{\cX} % X
\newcommand{\Y}{\cY} % X
%\newcommand{\msr}{{\mathbf{D}}}
%\newcommand{\dist}{\mathbf{d}}
%\newcommand{\dDist}{\dist}
%\newcommand{\dVec}{\ol{d}}
%\newcommand{\distVec}{\ol{\dist}}
\newcommand{\hypo}{h}
%\newcommand{\Dist}{\msr}
\newcommand{\C}{\cC}
\newcommand{\D}{\cD}
\renewcommand{\H}{\cH}
\newcommand{\error}{\mathsf{Err}}
\newcommand{\Error}{\error}
\newcommand{\Conf}{\mathsf{Conf}}
\newcommand{\conf}{\Conf}
\newcommand{\alphaDist}{{\bm \upalpha}}
\newcommand{\Risk}{\mathsf{Risk}}
\newcommand{\Rob}{\mathsf{Rob}}
% \newcommand{\cwd}{\mathsf{cwd}}


\newcommand{\Tam}{\mathsf{Tam}}
\newcommand{\TamAb}{\mathsf{TamAb}}
\newcommand{\AppTam}{\mathsf{AppTam}}
\newcommand{\AppTamAb}{\mathsf{AppTamAb}}
%\newcommand{\ORTam}{\mathsf{ORSam}}
%\newcommand{\KRTam}{\mathsf{KRSam}}
\newcommand{\Inv}{\mathsf{Inv}}
\newcommand{\Ideal}{\mathsf{Ideal}}
\newcommand{\Trans}{\mathsf{Trans}}
\newcommand{\Small}{\mathsf{Small}}
\newcommand{\UnBal}{\mathsf{UnBal}}
\newcommand{\Good}{\mathsf{Good}}
\newcommand{\High}{\mathrm{High}}
\newcommand{\Low}{\mathrm{Low}}
\newcommand{\BigOut}{\mathrm{Big}}
\newcommand{\SmallOut}{\mathrm{Small}}


\newcommand{\xDist}{\mathbf{x}}
\newcommand{\yDist}{\mathbf{y}}
\newcommand{\zDist}{\mathbf{z}}
\newcommand{\tDist}{\mathbf{t}}
\newcommand{\TDist}{\mathbf{T}}
\newcommand{\WDist}{\mathbf{W}}
\newcommand{\sDist}{\mathbf{s}}
\newcommand{\uDist}{\mathbf{u}}
\newcommand{\vDist}{\mathbf{v}}
\newcommand{\wDist}{\mathbf{w}}



\newcommand{\XDist}{\mathbf{X}}
\newcommand{\UDist}{\mathbf{U}}
\newcommand{\trainDist}{\UDist}

\newcommand{\xDistVec}{\ol{\xDist}}
\newcommand{\yDistVec}{\ol{\yDist}}
\newcommand{\zDistVec}{\ol{\zDist}}
\newcommand{\tDistVec}{\ol{\tDist}}
\newcommand{\sDistVec}{\ol{\sDist}}
\newcommand{\uDistVec}{\ol{\uDist}}
\newcommand{\vDistVec}{\ol{\vDist}}
\newcommand{\wDistVec}{\ol{\wDist}}


\newcommand{\insDist}{\xDist}
\newcommand{\instDist}{\insDist}

\newcommand{\xVec}{\ol{x}}
\newcommand{\yVec}{\ol{y}}
\newcommand{\zVec}{\ol{z}}
\newcommand{\tVec}{\ol{t}}
\newcommand{\sVec}{\ol{s}}
\newcommand{\uVec}{\ol{u}}
\newcommand{\vVec}{\ol{v}}
\newcommand{\wVec}{\ol{w}}

\newcommand{\alVec}{{\ol{\alpha}}}
\newcommand{\alK}{{\bfK_\alVec}}
\newcommand{\alk}{{\bfK_\alVec}}
\newcommand{\alHD}{\HD_{\alVec}}

\newcommand{\SDist}{\mathbf{S}}

\newcommand{\uRP}{{\wt{\uDist}}}

\renewcommand{\th}{^\mathrm{th}}
\newcommand{\jointSamp}[2]{\langle #1 \,\, \| \, {#2}\rangle}
\newcommand{\fvers}{(Please see the full version for the proof.) }

\newcommand{\overbar}[1]{\mkern 1.9mu\overline{\mkern-2.9mu#1\mkern-0.5mu}\mkern 1.9mu}
\newcommand{\overbarr}[1]{\mkern 1.9mu\overline{\mkern-0.9mu#1\mkern-3.5mu}\mkern 1.9mu}
%\newcommand{\X}{\overbar{X}}
%\newcommand{\Y}{\overline{Y}}
%\newcommand{\Yd}{\overbarr{Y_\delta}}
%\newcommand{\Z}{\overbar{Z}}

%\renewcommand{\R}{\olverline{R}}
\newtheorem{thm}{Theorem}
\newtheorem{lem}{Lemma}
\newcommand{\spn}{\mathrm{Span}}
\newcommand{\EQref}[1]{Equation~(\ref{#1})}
\newcommand{\VP}{\mathrm{ValPrf}}
\newcommand{\EX}{\mathsf{Ext}}
\newcommand{\Dn}{D^{\scriptscriptstyle (n)}}

\newcommand{\cost}{\mathsf{cost}}
\newcommand{\avgcost}{\overline{\cost}}


\newcommand{\KLsimp}{D_\mathsf{\scriptscriptstyle KL}}
% \newcommand{\KL}[2]{D_\mathsf{\scriptscriptstyle KL}(#1||#2)}
\newcommand{\KLn}[2]{D^{\scriptscriptstyle (n)}_\mathsf{\scriptscriptstyle KL}(#1||#2)}

\newcommand{\MDsimp}{D_{\scriptscriptstyle \infty}}
\newcommand{\MD}[2]{D_{\scriptscriptstyle \infty}(#1||#2)}
\newcommand{\MDn}[2]{D^{\scriptscriptstyle (n)}_{\scriptscriptstyle\infty}(#1||#2)}

\newcommand{\SDsimp}{D_\mathsf{\scriptscriptstyle SD}}
\newcommand{\SD}[2]{D_\mathsf{\scriptscriptstyle SD}(#1,#2)}
\newcommand{\SDn}[2]{D^{\scriptscriptstyle (n)}_\mathsf{\scriptscriptstyle SD}(#1,#2)}

\newcommand{\minE}[1]{\mathrm{H}_{\scriptscriptstyle \infty}(#1)}

\newcommand{\pfix}[2]{ {#1}_{\leq #2}}
\newcommand{\pofix}[2]{#1_{\geq #2 }}
\newcommand{\dmax}{\mathsf{max}_\delta}
%\newcommand{\avr}[2]{\Ex[#1(#2)]}
\newcommand{\dMax}{\mathsf{Max}_{\geq \delta}}
\newcommand{\dlMax}{\mathsf{Max}_{< \delta}}

\newcommand{\Exists}{\exists\,}
\newcommand{\Forall}{\forall\,}
\newcommand{\fDist}{\mathbf{f}}
\newcommand{\aSF}{\mathsf{a}}
\newcommand{\gSF}{\mathsf{g}}
\newcommand{\hSF}{\mathsf{h}}

\newcommand{\avr}[2]{\ifthenelse{\equal{#2}{}}{\aSF({#1})}{\ifthenelse{\equal{#2}{0}}{\aSF(\emptyset)}{\aSF({#1}_{\leq #2})}}}

\newcommand{\avrMax}[2]{\ifthenelse{\equal{#2}{}}{\aSF^*({#1})}{\ifthenelse{\equal{#2}{0}}{\aSF^*(\emptyset)}{\aSF^*({#1}_{\leq #2})}}}

\newcommand{\avrApp}[2]{\ifthenelse{\equal{#2}{}}{\tilde{\aSF}({#1})}{\ifthenelse{\equal{#2}{0}}{\tilde{\aSF}(\emptyset)}{\tilde{\aSF}({#1}_{\leq #2})}}}

\newcommand{\avrAppMax}[2]{\ifthenelse{\equal{#2}{}}{\tilde{\aSF}^*({#1})}{\ifthenelse{\equal{#2}{0}}{\tilde{\aSF}^*(\emptyset)}{\tilde{\aSF}^*({#1}_{\leq #2})}}}

\newcommand{\ArgMax}[2]{\ifthenelse{\equal{#2}{}}{\hSF({#1})}{\ifthenelse{\equal{#2}{0}}{\hSF(\emptyset)}{\hSF({#1}_{\leq #2})}}}

\newcommand{\AppArgMax}[2]{\ifthenelse{\equal{#2}{}}{\tilde{\hSF}({#1})}{\ifthenelse{\equal{#2}{0}}{\tilde{\hSF}(\emptyset)}{\tilde{\hSF}({#1}_{\leq #2})}}}

\newcommand{\Err}{\mathcal{E}}
\newcommand{\expectedsub}[2]{\ensuremath{\mathop{{}\mathbf{E}}_{#1}\left[#2\right]}\xspace}
\newcommand{\charac}{\mathbf{1}}


\newcommand{\gain}[2]{\ifthenelse{\equal{#2}{}}{\gSF(#1)}{\gSF(#1_{\leq #2})}}
\newcommand{\gainMax}[2]{\ifthenelse{\equal{#2}{}}{\gSF^*(#1)}{\gSF^*(#1_{\leq #2})}}
\newcommand{\gainApp}[2]{\ifthenelse{\equal{#2}{}}{\tilde{\gSF}(#1)}{\tilde{\gSF}(#1_{\leq #2})}}
\newcommand{\gainAppMax}[2]{\ifthenelse{\equal{#2}{}}{\tilde{\gSF}^*(#1)}{\tilde{\gSF}^*(#1_{\leq #2})}}

%\newcommand{\avGain}(3]{{\mathcal{G}}_{#3}(#1_{\leq #2 -1}]}
%\newcommand{\avAbGain}(3]{\mathcal{A}_{#3}(#1_{\leq #2 -1}]}
%\newcommand{\avSqGain}(3]{\mathcal{Q}_{#3}(#1_{\leq #2 -1}]}



\newcommand{\RTam}{\mathsf{RejSam}}
\newcommand{\RTamk}{\mathsf{RejSam}_{k}}
%\newcommand{\RTamd}{\mathsf{RSam}_\delta}


\newcommand{\var}[2]{\Var[#1(#2)]}

\newcommand{\pr}[2][]{\Pr_{\ifthenelse{\isempty{#1}}{}{{#1}}}\left[{#2}\right]}

\newcommand{\GTam}{\mathsf{GTam}}
\newcommand{\EGTam}{\mathsf{EGTam}}

\newcommand{\LimSup}{\operatorname{limSup}}
%\newcommand{\sup}{\operatorname{sup}}
\newcommand{\pmbits}{\{+1,-1\}}
\newcommand{\pmint}{[-1,+1]}
%\newcommand{\Tam}{\Tam}
\newcommand{\IdealTam}{\mathsf{IdTam}}
\newcommand{\EffTam}{\mathsf{EffTam}}




% Oracle subroutines
\newcommand{\distO}{\mathbf{O}}
\newcommand{\setup}{\mathsf{G}}
\newcommand{\findsk}{{\mathsf{G}^{-1}}}
\newcommand{\enc}{\operatorname{Enc}}
\newcommand{\dec}{\operatorname{Dec}}
\newcommand{\rev}{\mathsf{rev}}
\newcommand{\decFull}{\operatorname{DecFull}}
\newcommand{\eval}{\mathsf{eval}}
\newcommand{\gi}{\mathsf{gi}}
\newcommand{\gc}{\mathsf{gc}}

\newcommand{\kgen}{\mathsf{K}}
% \newcommand{\test}{\mathsf{T}}
\newcommand{\testatt}{mathsf{T}}
\newcommand{\V}{\mathsf{V}}
\newcommand{\Pred}{\mathsf{P}}
\newcommand{\Func}{\mathsf{F}}

% Garbling and RE
\newcommand{\lbl}{\mathsf{label}}
\newcommand{\GCircuit}{\mathsf{Garb}}
\newcommand{\GInput}{\mathsf{GInput}}
\newcommand{\GEval}{\mathsf{Eval}}
\newcommand{\Circuit}{\mathsf{C}}
\newcommand{\hCircuit}{\hat{\mathsf{C}}}
\newcommand{\hFun}{\hat{\mathsf{F}}}
\newcommand{\Fun}{\mathsf{F}}
\newcommand{\GarbledCircuit}{\widetilde{\Circuit}}
\newcommand{\wire}{w}
\newcommand{\inp}{\mathsf{inp}}
\newcommand{\inpsize}{\mathsf{inpsize}}
\newcommand{\out}{\mathsf{out}}
\newcommand{\CircSim}{\mathsf{CircSim}}
\newcommand{\Garbled}[1]{\widetilde{#1}}
\newcommand{\Output}{y}
\newcommand{\Input}{x}
\newcommand{\GarbledInput}{\widetilde x}
\newcommand{\InputKey}{s^{\mathsf{in}}}
\newcommand{\InputSize}{m}
\def\indc{\stackrel{{\tiny{\mathrm{comp}}}}{\approx}}
\newcommand{\RE}{\mathsf{RE}}
\newcommand{\REenc}{\mathsf{RE.enc}}
\newcommand{\REdec}{\mathsf{RE.dec}}

\newcommand{\HandleEval}{\mathtt{HandleEval}}
\newcommand{\ConstructHelpers}{\mathtt{ConstHelp}}
\newcommand{\Reduct}{\mathtt{SecurityRed}}
\newcommand{\Reduc}{\Reduct}

% Algorithms
\newcommand{\scheme}{\mathcal{E}}
\newcommand{\newScheme}{\dot{\scheme}}
\newcommand{\newSchemex}{\ddot{\scheme}}
\newcommand{\newG}{\dot{G}}
\newcommand{\newE}{\dot{E}}
\newcommand{\newD}{\dot{D}}
\newcommand{\newpk}{\dot{pk}}
\newcommand{\newsk}{\dot{sk}}
\newcommand{\newc}{\dot{c}}
\newcommand{\newGx}{\ddot{G}}
\newcommand{\newEx}{\ddot{E}}
\newcommand{\newDx}{\ddot{D}}
\newcommand{\newpkx}{\ddot{pk}}
\newcommand{\newskx}{\ddot{sk}}
\newcommand{\newcx}{\ddot{c}}
\newcommand{\newp}{\dot{p}}
\newcommand{\newpx}{\ddot{p}}
\newcommand{\newq}{\dot{q}}
\newcommand{\newqx}{\ddot{q}}


% Events Notation
\newcommand{\Bad}{\mathrm{Bad}}
\newcommand{\Miss}{\mathrm{Miss}}
\newcommand{\Hit}{\mathrm{Hit}}
\newcommand{\Disjoint}{\mathrm{Disjoint}}

% Query Set Notation
\newcommand{\sets}[1]{\mathsf{#1}}
\newcommand{\Q}[2]{(#2 \xrightarrow[#1]{} \; ?)}
\newcommand{\QA}[3]{(#2 \xrightarrow[#1]{} #3)}
\newcommand{\OrigG}{\sets{OrigG}}
\newcommand{\OrigE}{\sets{OrigE}}
\newcommand{\OrigD}{\sets{OrigD}}
\newcommand{\LearnG}{\sets{LearnG}}
\newcommand{\LocalE}{\sets{LocalE}}
\newcommand{\AllE}{\sets{AllE}}
\newcommand{\LocalD}{\sets{LocalD}}
\newcommand{\EvalD}{\sets{EvalD}}
\newcommand{\SO}{S}
\newcommand{\HintGEnc}{\sets{H}}
\newcommand{\HintGEnci}[1]{\sets{H}^{#1}_{\newE}}
\newcommand{\HintEDec}{\sets{H}}
\newcommand{\HintEDeci}[1]{\sets{H}^{#1}_{\newDx}}
\newcommand{\HintGEncSim}{\HintGEnc^*}
\newcommand{\HintEDecSim}{\HintEDec^*}
\newcommand{\OrigESim}{\sets{\OrigE^*}}
\newcommand{\LocalESim}{\sets{\LocalE^*}}
\newcommand{\LearnGSim}{\LearnG}
\newcommand{\EvalDSim}{\EvalD^*}
\newcommand{\QueryDist}[1]{\mathrm{Query}(#1)}
\newcommand{\AllDist}{DistGen_1}
\newcommand{\Diff}{\sets{Diff}}


\newcommand{\dhat}[1]{\wh{\wh{#1}}}


\newcommand{\tmclass}{\fclass}
\newcommand{\Sim}{\mathsf{Sim}}
\newcommand{\ext}{^{\mathsf{ext}}}

\newcommand{\MSK}{\mathsf{MSK}}
\newcommand{\MPK}{\mathsf{MPK}}
\newcommand{\ID}{f}
\newcommand{\nand}{\barwedge}

\newcommand{\fclass}{\cF}
\newcommand{\secp}{\mathrm{\kappa}}
\newcommand{\secpar}{\secp}

%\newcommand{\Samp}{\mathsf{OnSam}}

\newcommand{\Sam}{\mathsf{Sam}}

%\newcommand{\Att}{\textsc{Attack}}
\newcommand{\Hyb}{\textsc{Hybrid}}
\newcommand{\Idl}{\textsc{Ideal}}
\newcommand{\Lzy}{\textsc{Lazy}}

\newcommand{\HIT}{\mathsf{HIT}}
\newcommand{\MAL}{\mathsf{MAL}}
\newcommand{\INT}{\mathsf{INT}}

\newcommand{\sm}{\setminus}
%\newcommand{\att}{_\mathsf{att}}
\newcommand{\hyb}{_\mathsf{hyb}}
\newcommand{\idl}{_\mathsf{idl}}

\newcommand{\oAtt}{\mathbf{Out}\att}
\newcommand{\oHyb}{\mathbf{Out}\hyb}
\newcommand{\oIdl}{\mathbf{Out}\idl}

\newcommand{\bHyb}{B_\mathsf{hyb}}
\newcommand{\bAtt}{B_\mathsf{att}}

\newcommand{\chal}{\mathbf{chal}}
\newcommand{\gen}{\mathbf{gen}}

\newcommand{\Clsr}{\CLSR}

\newcommand{\OR}{\mathsf{OR}}
\newcommand{\AND}{\mathsf{AND}}

\newcommand{\BadE}{\mathsf{BE}} % bad event

% keys mathsf
\newcommand{\sk}{\mathsf{sk}}
\newcommand{\SK}{\mathsf{SK}}
\newcommand{\pk}{\mathsf{pk}}
\newcommand{\PK}{\mathsf{PK}}
\newcommand{\dk}{\mathsf{dk}}
\newcommand{\DK}{\mathsf{DK}}
\newcommand{\problem}{\ensuremath{\mathcal{P}}\xspace}
\newcommand{\Rplus}{\R_+}
\newcommand{\Loss}{\mathrm{Risk}}
\newcommand{\loss}{\ell\mathrm{oss}}
% algorithms mahtbf
\newcommand{\e}{\mathrm{e}}
% \newcommand{\E}{\mathrm{E}}
\renewcommand{\d}{\mathbf{d}}
\newcommand{\id}{\mathbf{id}}
\renewcommand{\D}{\cD}
\newcommand{\g}{\mathbf{g}}
\newcommand{\G}{\mathbf{G}}
\renewcommand{\k}{\mathbf{k}}
\newcommand{\K}{\mathbf{K}}
\newcommand{\p}{\mathbf{p}}


\newcommand{\clg}{\ol{\g}}
\newcommand{\clk}{\ol{\k}}
\newcommand{\clid}{\ol{\id}}
\newcommand{\cle}{\ol{\e}}
\newcommand{\cld}{\ol{\d}}



% sets
\newcommand{\atA}{\mathbb{A}}
\newcommand{\atB}{\mathbb{B}}

\newcommand{\prF}{\mathbb{F}}
\newcommand{\prG}{\mathbb{G}}


\newcommand{\PE}{\mathbf{PE}}
\newcommand{\TPE}{\mathbf{TPE}}
\newcommand{\IBE}{\mathbf{IBE}}
\newcommand{\FPE}{\prF\text{-}\PE}
\newcommand{\GPE}{\prG\text{-}\PE}
\newcommand{\tTPE}{\tau\text{-}\TPE}
\newcommand{\ttTPE}{$\tau$-TPE\xspace}

%\newcommand{\att}{\cA}
%\newcommand{\prd}{\cP}
% \usepackage{graphicx}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%55
\newcommand{\remove}[1]{}
\newcommand{\num}[1]{{\bf (#1)}}

\newcommand{\ol}{\overline}
\newcommand{\wt}[1]{\widetilde{#1}}
\newcommand{\wh}[1]{\widehat{#1}}
\renewcommand{\nin}{\not \in}

\newcommand{\es}{\varnothing} % empty set
\newcommand{\se}{\subseteq}
\newcommand{\nse}{\not \se}
\newcommand{\nf}[2]{\nicefrac{#1}{#2}}
% \newcommand{\rv}[1]{\mathbf{#1}} % Random Variable
\newcommand{\rvV}{\rv{V}}




%%%  English %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\etal}{et~al.\ }
\newcommand{\aka}{also known as,\ }
\newcommand{\resp}{resp.,\ }
\newcommand{\ie}{i.e.,\ }
\newcommand{\wolog}{w.l.o.g.\ }
\newcommand{\Wolog}{W.l.o.g.\ }
\newcommand{\eg}{e.g.,\ }
\newcommand{\wrt} {with respect to\ }
\newcommand{\cf}{{cf.,\ }}

%%%  math %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\round}[1]{\lfloor #1 \rceil}
% \newcommand{\ceil}[1]{\lceil #1 \rceil}
% \newcommand{\floor}[1]{\lfloor #1 \rfloor}
\newcommand{\angles}[1]{\langle #1 \rangle}
\newcommand{\parens}[1]{( #1 )}
\newcommand{\bracks}[1]{[ #1 ]}
\newcommand{\bra}[1]{\langle#1\rvert}
\newcommand{\ket}[1]{\lvert#1\rangle}
\newcommand{\set}[1]{\left\{ #1 \right\}}

\newcommand{\adjRound}[1]{\left\lfloor #1 \right\rceil} % Adjusted Round
\newcommand{\adjCeil}[1]{\left\lceil #1 \right\rceil}
\newcommand{\adjFloor}[1]{\left\lfloor #1 \right\rfloor}
\newcommand{\adjAngles}[1]{\left\langle #1 \right\rangle}
\newcommand{\adjParens}[1]{\left( #1 \right)}
\newcommand{\adjBracks}[1]{\left[ #1 \right]}
\newcommand{\adjBra}[1]{\left\langle#1\right\rvert}
\newcommand{\adjKet}[1]{\left\lvert#1\right\rangle}
\newcommand{\adjSet}[1]{\left\{ #1 \right\}}
\newcommand{\half}{\tfrac{1}{2}}
\newcommand{\third}{\tfrac{1}{3}}
\newcommand{\quarter}{\tfrac{1}{4}}
\newcommand{\eqdef}{:=}
\newcommand{\zo}{\{0,1\}}
\newcommand{\bits}{\{0,1\}}
\newcommand{\xor}{\oplus}
\newcommand{\tensor}{\otimes}
\newcommand{\getsr}{\mathbin{\stackrel{\mbox{\,\tiny \$}}{\gets}}}
\newcommand{\from}{\gets}
\newcommand{\size}[1]{\left|#1\right|}
\newcommand{\abs}[1]{\size{#1}}
%\newcommand{\norm}[1]{\abf{#1}}
\newcommand{\norm}[1]{\left\lVert#1\right\rVert}
\newcommand{\To}{\mapsto}
\newcommand{\mcom}{\, ,}
\newcommand{\mper}{\, .}
% \newcommand{\sign}{\ensuremath {\pm 1}}
\newcommand{\nbyn}{\ensuremath {n \times n}}
\renewcommand{\L}{\ensuremath L\:}
\newcommand{\LA}{\ensuremath L_A}
\newcommand{\Learn}{\mathsf{Lasso}}
\newcommand{\LASSO}{\mathsf{Lasso}}
\newcommand{\Lasso}{\mathsf{Lasso}}

%%%% Font Abbreviations

% \newcommand{\R}{{\mathbb R}}
\newcommand{\N}{{\mathbb N}}
\newcommand{\F}{{\mathbb F}}

\newcommand{\trainTam}{\vVec}
\newcommand{\Adv}{\mathsf{A}}

% \newcommand{\train}{\uVec}
\newcommand{\tamped}[1]{\wh{#1}}

\newcommand{\cA}{{\mathcal A}}
\newcommand{\cB}{{\mathcal B}}
\newcommand{\cC}{{\mathcal C}}
\newcommand{\cD}{{\mathcal D}}
\newcommand{\cE}{{\mathcal E}}
\newcommand{\cF}{{\mathcal F}}
\newcommand{\cG}{{\mathcal G}}
\newcommand{\cH}{{\mathcal H}}
\newcommand{\cI}{{\mathcal I}}
\newcommand{\cJ}{{\mathcal J}}
\newcommand{\cK}{{\mathcal K}}
\newcommand{\cL}{{\mathcal L}}
\newcommand{\cM}{{\mathcal M}}
\newcommand{\cN}{{\mathcal N}}
\newcommand{\cO}{{\mathcal O}}
\newcommand{\cP}{{\mathcal P}}
\newcommand{\cQ}{{\mathcal Q}}
\newcommand{\cR}{{\mathcal R}}
\newcommand{\cS}{{\mathcal S}}
\newcommand{\cT}{{\mathcal T}}
\newcommand{\cU}{{\mathcal U}}
\newcommand{\cV}{{\mathcal V}}
\newcommand{\cW}{{\mathcal W}}
\newcommand{\cX}{{\mathcal X}}
\newcommand{\cY}{{\mathcal Y}}
\newcommand{\cZ}{{\mathcal Z}}

\newcommand{\bfA}{\mathbf{A}}
\newcommand{\bfB}{\mathbf{B}}
\newcommand{\bfC}{\mathbf{C}}
\newcommand{\bfD}{\mathbf{D}}
\newcommand{\bfE}{\mathbf{E}}
\newcommand{\bfF}{\mathbf{F}}
\newcommand{\bfG}{\mathbf{G}}
\newcommand{\bfH}{\mathbf{H}}
\newcommand{\bfI}{\mathbf{I}}
\newcommand{\bfJ}{\mathbf{J}}
\newcommand{\bfK}{\mathbf{K}}
\newcommand{\bfL}{\mathbf{L}}
\newcommand{\bfM}{\mathbf{M}}
\newcommand{\bfN}{\mathbf{N}}
\newcommand{\bfO}{\mathbf{O}}
\newcommand{\bfP}{\mathbf{P}}
\newcommand{\bfQ}{\mathbf{Q}}
\newcommand{\bfR}{\mathbf{R}}
\newcommand{\bfS}{\mathbf{S}}
\newcommand{\bfT}{\mathbf{T}}
\newcommand{\bfU}{\mathbf{U}}
\newcommand{\bfV}{\mathbf{V}}
\newcommand{\bfW}{\mathbf{W}}
\newcommand{\bfX}{\mathbf{X}}
\newcommand{\bfY}{\mathbf{Y}}
\newcommand{\bfZ}{\mathbf{Z}}


\newcommand{\bfa}{\mathbf{a}}
\newcommand{\bfb}{\mathbf{b}}
\newcommand{\bfc}{\mathbf{c}}
\newcommand{\bfd}{\mathbf{d}}
\newcommand{\bfe}{\mathbf{e}}
\newcommand{\bff}{\mathbf{f}}
\newcommand{\bfg}{\mathbf{g}}
\newcommand{\bfh}{\mathbf{h}}
\newcommand{\bfi}{\mathbf{i}}
\newcommand{\bfj}{\mathbf{j}}
\newcommand{\bfk}{\mathbf{k}}
\newcommand{\bfl}{\mathbf{l}}
\newcommand{\bfm}{\mathbf{m}}
\newcommand{\bfn}{\mathbf{n}}
\newcommand{\bfo}{\mathbf{o}}
\newcommand{\bfp}{\mathbf{p}}
\newcommand{\bfq}{\mathbf{q}}
\newcommand{\bfr}{\mathbf{r}}
\newcommand{\bfs}{\mathbf{s}}
\newcommand{\bft}{\mathbf{t}}
\newcommand{\bfu}{\mathbf{u}}
\newcommand{\bfv}{\mathbf{v}}
\newcommand{\bfw}{\mathbf{w}}
\newcommand{\bfx}{\mathbf{x}}
\newcommand{\bfy}{\mathbf{y}}
\newcommand{\bfz}{\mathbf{z}}

% \usepackage{upgreek}
% \usepackage{bm}

% note the short forms: eps and ups
\newcommand{\bfalpha}{{\bm \alpha}}
\newcommand{\bfbeta}{{\bm \beta}}
\newcommand{\bfgamma}{{\bm \gamma}}
\newcommand{\bfdelta}{{\bm \delta}}
\newcommand{\bfeps}{{\bm \epsilon}}
\newcommand{\bfveps}{{\bm \varepsilon}}
\newcommand{\bfzeta}{{\bm \zeta}}
\newcommand{\bftheta}{{\bm \theta}}
\newcommand{\bfvtheta}{{\bm \vartheta}}
\newcommand{\bfiota}{{\bm \iota}}
\newcommand{\bfkappa}{{\bm \kappa}}
\newcommand{\bflambda}{{\bm \lambda}}
\newcommand{\bfmu}{{\bm \mu}}
\newcommand{\bfnu}{{\bm \nu}}
\newcommand{\bfxi}{{\bm \xi}}
\newcommand{\bfoo}{{\bm \o}}% not to confuse with regular o
\newcommand{\bfpi}{{\bm \pi}}
\newcommand{\bfvarpi}{{\bm \varpi}}
\newcommand{\bfrho}{{\bm \rho}}
\newcommand{\bfvrho}{{\bm \varrho}}
\newcommand{\bfsigma}{{\bm \sigma}}
\newcommand{\bfvsigma}{{\bm \varsigma}}
\newcommand{\bftau}{{\bm \tau}}
\newcommand{\bfups}{{\bm \upsilon}}
\newcommand{\bfphi}{{\bm \phi}}
\newcommand{\bfvphi}{{\bm \varphi}}
\newcommand{\bfchi}{{\bm \chi}}
\newcommand{\bfpsi}{{\bm \psi}}
\newcommand{\bfomega}{{\bm \omega}}


\newcommand{\sfA}{\mathsf{A}}
\newcommand{\sfB}{\mathsf{B}}
\newcommand{\sfC}{\mathsf{C}}
\newcommand{\sfD}{\mathsf{D}}
\newcommand{\sfE}{\mathsf{E}}
\newcommand{\sfF}{\mathsf{F}}
\newcommand{\sfG}{\mathsf{G}}
\newcommand{\sfH}{\mathsf{H}}
\newcommand{\sfI}{\mathsf{I}}
\newcommand{\sfJ}{\mathsf{J}}
\newcommand{\sfK}{\mathsf{K}}
\newcommand{\sfL}{\mathsf{L}}
\newcommand{\sfM}{\mathsf{M}}
\newcommand{\sfN}{\mathsf{N}}
\newcommand{\sfO}{\mathsf{O}}
\newcommand{\sfP}{\mathsf{P}}
\newcommand{\sfQ}{\mathsf{Q}}
\newcommand{\sfR}{\mathsf{R}}
\newcommand{\sfS}{\mathsf{S}}
\newcommand{\sfT}{\mathsf{T}}
\newcommand{\sfU}{\mathsf{U}}
\newcommand{\sfV}{\mathsf{V}}
\newcommand{\sfW}{\mathsf{W}}
\newcommand{\sfX}{\mathsf{X}}
\newcommand{\sfY}{\mathsf{Y}}
\newcommand{\sfZ}{\mathsf{Z}}

\newcommand{\sfa}{\mathsf{a}}
\newcommand{\sfb}{\mathsf{b}}
\newcommand{\sfc}{\mathsf{c}}
\newcommand{\sfd}{\mathsf{d}}
\newcommand{\sfe}{\mathsf{e}}
\newcommand{\sff}{\mathsf{f}}
\newcommand{\sfg}{\mathsf{g}}
\newcommand{\sfh}{\mathsf{h}}
\newcommand{\sfi}{\mathsf{i}}
\newcommand{\sfj}{\mathsf{j}}
\newcommand{\sfk}{\mathsf{k}}
\newcommand{\sfl}{\mathsf{l}}
\newcommand{\sfm}{\mathsf{m}}
\newcommand{\sfn}{\mathsf{n}}
\newcommand{\sfo}{\mathsf{o}}
\newcommand{\sfp}{\mathsf{p}}
\newcommand{\sfq}{\mathsf{q}}
\newcommand{\sfr}{\mathsf{r}}
\newcommand{\sfs}{\mathsf{s}}
\newcommand{\sft}{\mathsf{t}}
\newcommand{\sfu}{\mathsf{u}}
\newcommand{\sfv}{\mathsf{v}}
\newcommand{\sfw}{\mathsf{w}}
\newcommand{\sfx}{\mathsf{x}}
\newcommand{\sfy}{\mathsf{y}}
\newcommand{\sfz}{\mathsf{z}}
% \newcommand{\eps}{\varepsilon}
%\newcommand{\e}{\epsilon}
\newcommand{\veps}{\varepsilon}
%\newcommand{\vare}{\varepsilon}
\newcommand{\vphi}{\varphi}
\newcommand{\vsigma}{\varsigma}
\newcommand{\vrho}{\varrho}
\newcommand{\vpi}{\varpi}
% \newcommand{\tO}{\widetilde{O}}
\newcommand{\tOmega}{\widetilde{\Omega}}
\newcommand{\tTheta}{\widetilde{\Theta}}
\newcommand{\field}{\ensuremath \Bbbk}
\newcommand{\reals}{\ensuremath \mathbb{R}}
% \DeclareMathOperator{\Rig}{Rig}
% \DeclareMathOperator{\rk}{rank}

% \DeclareMathOperator{\rank}{rank}

%%%%%%%%%%%%%%%% Operators %%%%%%

\newcommand{\poly}{\operatorname{poly}}
\newcommand{\polylog}{\operatorname{polylog}}
\newcommand{\loglog}{\operatorname{loglog}}
\newcommand{\GF}{\operatorname{GF}}
\newcommand{\Exp}{\operatorname*{\mathbb{E}}}
\newcommand{\Ex}{\Exp}
%\newcommand{\view}{\operatorname{view}}
\newcommand{\View}[1]{\mathsf{View}\angles{#1}}
% \newcommand{\Var}{\operatorname*{\mathbb{V}}}
\newcommand{\ShH}{\operatorname{H}}
\newcommand{\maxH}{\operatorname{H_0}}
\newcommand{\minH}{\operatorname{H_{\infty}}}
\newcommand{\Enc}{\operatorname{Enc}}
\newcommand{\Setup}{\operatorname{Setup}}
\newcommand{\KGen}{\operatorname{KGen}}
\newcommand{\Dec}{\operatorname{Dec}}
\newcommand{\Sign}{\operatorname{Sign}}
\newcommand{\Ver}{\operatorname{Ver}}
\newcommand{\Gen}{\operatorname{Gen}}
\newcommand{\negl}{\operatorname{negl}}
\newcommand{\Supp}{\operatorname{Supp}}
\newcommand{\maj}{\operatorname*{maj}}
% \newcommand{\argmax}{\operatorname*{argmax}}
% \newcommand{\argmin}{\operatorname*{argmin}}
\newcommand{\Image}{\operatorname{Im}}


%%% Computational Problems %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\newcommand{\SAT}{\mathrm{SAT}}
\newcommand{\UNSAT}{\mathrm{UNSAT}}
%\newcommand{\ED}{\mathrm{ED}} % Entropy Difference
%\newcommand{\GapSVP}{\mathrm{GapSVP}}
%\newcommand{\GapSIVP}{\mathrm{GapSIVP}}
%\newcommand{\GapCVP}{\mathrm{GapCVP}}
%\newcommand{\COLOR}{\mathrm{3COL}}

%%% Complexity Classes %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\class}[1]{\ensuremath{\mathbf{#1}}}
\newcommand{\coclass}[1]{\class{co\mbox{-}#1}} %  their complements
\newcommand{\prclass}[1]{\class{Pr#1}}
\newcommand{\PPT}{\class{PPT}}
\newcommand{\BPP}{\class{BPP}}
\newcommand{\NC}{\class{NC}}
\newcommand{\AC}{\class{AC}}
\newcommand{\NP}{\ensuremath{\class{NP}}}
\newcommand{\coNP}{\ensuremath{\coclass{NP}}}
\newcommand{\RP}{\class{RP}}
\newcommand{\coRP}{\coclass{RP}}
\newcommand{\ZPP}{\class{ZPP}}
\newcommand{\IP}{\class{IP}}
\newcommand{\coIP}{\coclass{IP}}
\newcommand{\AM}{\class{AM}}
\newcommand{\coAM}{\class{coAM}}
\newcommand{\MA}{\class{MA}}
\renewcommand{\P}{\class{P}}
\newcommand\prBPP{\prclass{BPP}}
\newcommand\prRP{\prclass{RP}}
%\newcommand\prP{\prclass{P}}
\newcommand{\Ppoly}{\class{P/poly}}
\newcommand{\DTIME}{\class{DTIME}}
\newcommand{\ETIME}{\class{E}}
\newcommand{\BPTIME}{\class{BPTIME}}
\newcommand{\AMTIME}{\class{AMTIME}}
\newcommand{\coAMTIME}{\class{coAMTIME}}
\newcommand{\NTIME}{\class{NTIME}}
\newcommand{\coNTIME}{\class{coNTIME}}
\newcommand{\AMcoAM}{\class{AM} \cap \class{coAM}}
\newcommand{\NPcoNP}{\class{N} \cap \class{coN}}
\newcommand{\EXP}{\class{EXP}}
\newcommand{\SUBEXP}{\class{SUBEXP}}
\newcommand{\qP}{\class{\wt{P}}}
\newcommand{\PH}{\class{PH}}
\newcommand{\NEXP}{\class{NEXP}}
\newcommand{\PSPACE}{\class{PSPACE}}
%\newcommand{\E}{\class{E}}
\newcommand{\NE}{\class{NE}}
\newcommand{\coNE}{\class{coNE}}
\newcommand{\SharpP}{\class{\#P}}
\newcommand{\prSZK}{\prclass{SZK}}
\newcommand{\BPPSZK}{\BPP^{\SZK}}
\newcommand{\TFAM}{\class{TFAM}}
\newcommand{\RTFAM}{{\R\text{-}\class{TUAM}}}
% relations decidable by a randomized algorithm
\newcommand{\FBPP}{\class{BPP}}
% relations decidable by a RTFAM oracle
\newcommand{\BPPR}{\FBPP^{\RTFAM}}
\newcommand{\TFNP}{\mathbf{TFNP}}
\newcommand{\MIP}{\mathbf{MIP}}
% zero-knowledge complexity classes
\newcommand{\ZK}{\class{ZK}}
\newcommand{\SZK}{\class{SZK}}
\newcommand{\SZKP}{\class{SZKP}}
\newcommand{\SZKA}{\class{SZKA}}
\newcommand{\CZKP}{\class{CZKP}}
\newcommand{\CZKA}{\class{CZKA}}
\newcommand{\coSZKP}{\coclass{SZKP}}
\newcommand{\coSZKA}{\coclass{SZKA}}
\newcommand{\coCZKP}{\coclass{CZKP}}
\newcommand{\coCZKA}{\coclass{CZKA}}
\newcommand{\NISZKP}{\class{NI\mbox{-}SZKP}}
\newcommand{\phcc}{\ensuremath \PH^{\mathrm{cc}}}
\newcommand{\pspacecc}{\ensuremath \PSPACE^{\mathrm{cc}}}
\newcommand{\sigcc}[1]{\ensuremath \class{\Sigma}^{\mathrm{cc}}_{#1}}
\newcommand{\aco}{\ensuremath \AC^0}
\newcommand{\ncone}{\ensuremath \NC^1}

%%%%% Theorem environments
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


%\ifllncs
\newtheorem{aclaim}{Claim}
%\fi


\newtheorem{theorem}{Theorem}%[section]
% \theoremstyle{plain}
\newtheorem{claim}{Claim}
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{conjecture}[theorem]{Conjecture}

\newtheorem{observation}[theorem]{Observation}
\newtheorem{fact}[theorem]{Fact}
% \theoremstyle{definition}

\newtheorem{definition}{Definition}
\newtheorem{construction}[theorem]{Construction}
\newtheorem{example}[theorem]{Example}
\newtheorem{algorithm1}[theorem]{Algorithm}
%\newtheorem{protocol}[theorem]{Protocol} defined below
\newtheorem{assumption}[theorem]{Assumption}

% \theoremstyle{definition}
% \newtheorem*{remark}{Remark}
\newtheorem{note}[theorem]{Note}


% Protocol env
\newcommand{\sdotfill}{\textcolor[rgb]{0.8,0.8,0.8}{\dotfill}} %change to \cdotfill later
\newenvironment{protocol}{\begin{proto}}{\vspace{-\topsep}\sdotfill\end{proto}}

\makeatletter
\def\th@protocol{%
    \normalfont % body font
    \setbeamercolor{block title example}{bg=orange,fg=white}
    \setbeamercolor{block body example}{bg=orange!20,fg=black}
    \def\inserttheoremblockenv{exampleblock}
  }
\makeatother
% \theoremstyle{protocol}

\newtheorem{proto}[theorem]{Protocol}
\newtheorem{protoc}[theorem]{Protocol}
\newenvironment{protocolS}{\begin{protoc}}{\vspace{-\topsep}\sdotfill\end{protoc}}

% state/restate
\newcommand{\namedref}[2]{#1~\ref{#2}}

\newcommand{\torestate}[3]{%
\expandafter \def \csname BBRESTATE #2 \endcsname{#3}
\theoremstyle{plain}
\newtheorem{BBRESTATETHMNUM#2}[theorem]{#1}
\begin{BBRESTATETHMNUM#2}\label{#2}\csname BBRESTATE #2 \endcsname   \end{BBRESTATETHMNUM#2}
\newtheorem*{BBRESTATETHMNONNUM#2}{\namedref{#1}{#2}}
}

\newcommand{\restate}[1]{\begin{BBRESTATETHMNONNUM#1}[Restated] \csname BBRESTATE #1 \endcsname
\end{BBRESTATETHMNONNUM#1}}

%%% refs macros (hopefully will help in transforming to pdf) %%%%%%


\newcommand{\theoremref}[1]{Theorem~\ref{#1}}
\newcommand{\sectionref}[1]{Sect.~\ref{#1}}
\newcommand{\definitionref}[1]{Definition~\ref{#1}}
\newcommand{\defref}[1]{Definition~\ref{#1}}
\newcommand{\propref}[1]{Proposition~\ref{#1}}
\newcommand{\stepref}[1]{Step~\ref{#1}}
\newcommand{\figureref}[1]{Fig.~\ref{#1}}
\newcommand{\lemmaref}[1]{Lemma~\ref{#1}}
\newcommand{\claimref}[1]{Claim~\ref{#1}}
\newcommand{\remarkref}[1]{Remark~\ref{#1}}
\newcommand{\corollaryref}[1]{Corollary~\ref{#1}}
\newcommand{\inequalityref}[1]{Inequality~\ref{#1}}
\newcommand{\constructionref}[1]{Construction~\ref{#1}}
\newcommand{\itemref}[1]{Item~\ref{#1}}
\newcommand{\propertyref}[1]{Property~\ref{#1}}
\newcommand{\protocolref}[1]{Protocol~\ref{#1}}
\newcommand{\algorithmref}[1]{Algorithm~\ref{#1}}
\newcommand{\appendixref}[1]{Appendix~\ref{#1}} 

==> Proxy distributions [ICLR 2022]/math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> Proxy distributions [ICLR 2022]/sections/background.tex <==
% Adversarial training~\citep{Goodfellow2014ExplainAdv, madry2017towards, zhang2019tradeoff, gowal2020uncoveringadv, wu2020adversarial} remains the most effective defense against adversarial examples~\citep{szegedy2013intriguing}. 
% % Subsequent works further improve its performance using larger architectures~\citep{gowal2020uncoveringadv}, early stopping~\citep{rice2020overfitadv}, smooth activations~\citep{xie2020smooth}, weight perturbations~\citep{wu2020adversarial}.
% However, earlier works have also shown that adversarial training suffers from a large robust generalization gap~\citep{cchmidt2018robustgeneralization, raghunathan2019adversarialgen}. We refer the reader to RobustBench~\citep{croce2020robustbench} for comparison and overview of state-of-the-art methods. 

% In our work, we also find that state-of-the-art diffusion process-based models provide much higher gain than state-of-the-art GAN. 

% Recent works have also explored the use of synthetic samples in training deep neural networks~\citep{ravuri2019CAS, shmelkov2018good}. While these earlier works focus on benign training our focus is on adversarial training. Another concurrent work~\citep{rebuffi2021fixingaugmentation} also uses samples from generative models to improve adversarial robustness. While ~\citet{rebuffi2021fixingaugmentation} broadly focuses on the effect of data augmentation, our goal is to understand the effect of different proxy distributions. However, similar benefits of using the generative model from two independent works further ascertain the importance of this direction. 


\subsection{Robust Machine learning}

\noindent \textbf{Adversarial examples.} Adversarial examples, crafted using an adversarial attack, aim to evade the classifier at the test time~\citep{biggio2013evasion, Szegedy2013IntrigueAdv, biggio2018wildPatterns}. While we focus on $\ell_p$ perturbation based adversarial examples~\citep{Goodfellow2014ExplainAdv}, there exist multiple other threat models~\citep{wong2019wassersteinAdv, sehwag2019analyzing, hosseini2018semanticAdv, Laidlaw2019functionalAdv, kang2019unforseenAdv}. Adversarial examples have been successful against almost all applications of machine learning~\citep{xu2020AdvImageGraphText, xu2016autoEvadePdfAdv, rahman2019mockingbird}. 

\noindent \textbf{On use of $l_p$ threat model.} We consider $\ell_p$ perturbation based adversarial examples since it's the most widely studied threat model~\citep{croce2020robustbench}. Additionally, robustness achieved in this threat model has also led to further benefits in  explainability~\citep{chalasani2020advExplain}, image recognition~\citep{xie2020advImproveCV, salman2020Unadversarial}, transfer learning~\citep{Salman2020AdvTransfer, utrera2021AdvTransfer}, self-supervised learning~\citep{Ho2020SSLAdvExamples}, and image synthesis~\citep{Santurkar2019AdvImageSynthesis}. 

\noindent \textbf{Adversarial training.} 
Adversarial training~\citep{Goodfellow2014ExplainAdv, madry2017towards} still remains the most effective defense against adversarial examples. The performance of the baseline technique~\citep{madry2017towards} is further improved using adaptive loss functions~\citep{zhang2019tradeoff}, larger networks~\citep{gowal2020uncoveringadv}, pretraining~\citep{hendrycks2019AdvPretrain}, smooth activation function~\citep{xie2020smooth}, and weight perturbations~\citep{wu2020adversarial}. The fundamental min-max robust optimization behind adversarial training has also been successful in robustifying other model architectures, such as decision trees \citep{chen2019robustTree} and graph neural networks~\citep{feng2019AdvTraingraph}, while also extending to other domains like reinforcement learning~\citep{Gleave2020AdvRL} and natural language processing~\citep{liu2020advTrainNLP}.

\noindent \textbf{Progress on improving adversarial robustness.}
Improving adversarial robustness in deep neural networks remains a challenging problem and its progress has been slow, as tracked by the RobustBench~\citep{croce2020robustbench}. Following initial success of baseline adversarial training in \citep{madry2017towards}, robust accuracy has improved by only $12$\% in the setting where networks architecture is fixed to \wrn{28-10} and no extra real-world images are used (from $44.0$\% in \citet{madry2017towards} to $56.2$\% in \citet{wu2020adversarial}). Additionally, there have been more than twenty failed attempts in improving it over the baseline~\citep{croce2020robustbench}. To put our work in context, we further improve robust accuracy on the CIFAR-10 dataset to $59.5$\%, without using additional techniques like smooth activations or weight perturbations.


\noindent \textbf{Certified robustness.} Here the goal is to certify the robustness of each examples~\citep{Wong2018ScalingProve, cohen2019certified, Zhang2020crownIbp}. Certified robustness provides a lower bound on the adversarial robustness against all attacks in the threat model. We use randomized smoothing~\citep{cohen2019certified} to achieve certified robustness, since it achieves much better performance over other methods in this domain~\citep{cohen2019certified, carmon2019unlabeled}. Further improvements in randomized smoothing includes integration with adversarial training~\citep{salman2019AdvSmooth}, using sub-networks~\citep{sehwag2020Hydra}, and using sample-specific smoothing~\citep{alfarra2020dataDependSmooth}.

\subsection{Intriguing properties of adversarial training}

\noindent \textbf{Sample complexity of adversarial training.} Multiple earlier works provide theoretical results studying the effect of the number of training samples on adversarial robustness~\citep{wei2019allLayerMargin, bhagoji2019lowerBounds, schmidt2018AdvMoreData, chen2020dataHurtsAdv, min2020datahurts}. \citet{chen2020dataHurtsAdv} and \citet{min2020datahurts} further suggest that more data may hurt generalization in adversarial training. We explore this direction empirically by adversarial training deep neural networks on an increasing number of training images.

\noindent \textbf{Trade-off in adversarial training.} There also exists an accuracy vs robustness trade-off where improvement in robust accuracy comes at the cost of clean accuracy in adversarial training~\citep{Raghunathan2020advtradeoff, balaji2019instAdaptAdvtrain, javanmard2020preciseTradeoff}. We empirically demonstrate that increase in the number of training samples can significantly reduce this trade-off. 

\noindent \textbf{Transfer of adversarial robustness.}
This line of work focuses on the transfer of adversarial robustness, i.e., correct classification even under adversarial perturbations, when testing the model on different data distributions~\citep{shafahi2020AdvRobustTransfer, sehwag2019analyzing}. Note that this is different from just achieving correct classification on unmodified images across different distributions~\citep{taori2020NatShiftRobust, hendrycks2019CommonCorrupt}. Here we provide a theoretical analysis of the transfer of adversarial robustness between data distributions. 
%\vikash{Are we first to do it. Not likely. Can also include complementary works.}


\noindent \textbf{Using extra curated real-world data.} Prior works \citep{zhai2019advJustmoreData, carmon2019unlabeled, alayrac2019unsupadv, najafi2019advIncompleteData, deng2020AdvExtraOutDomain} have argued for using more training data in adversarial training and often resort to curating additional real-world samples. In contrast, we don't require additional real-world samples, as we model the proxy distribution from the limited training images available and sample additional synthetic images from this distribution. %In spirit, our approach is similar to techniques like mixup~\citep{zhang2018mixup, Pang2020MixupInfer}, which adds novel samples in training by interpolating along samples in the available training data. 


% Cite the result for the gaussian case. Cite min et al. for a more convoluted case. We put this to rest by conducting an experiment with 1k-10M training images. Some earlier works to study this are following: \citep{wei2019allLayerMargin, bhagoji2019lowerBounds, schmidt2018AdvMoreData}. 

% \noindent \textbf{More data in adversarial training.} Both \citep{chen2020dataHurtsAdv, min2020datahurts} provide theoretical results suggesting more data may hurt in adversarial training.  Empirically earlier work \citep{zhai2019advJustmoreData, carmon2019unlabeled, alayrac2019unsupadv, najafi2019advIncompleteData, deng2020AdvExtraOutDomain} have argued for using more data and often resort to curating additional real-world samples.

\subsection{Using generative models for proxy distributions}
\noindent \textbf{Generative models for proxy distributions.}
State-of-the-art generative models are capable of modeling the distribution of current large-scale image datasets. In particular, generative adversarial networks (GANs) have excelled at this task~\citep{goodfellow2014GAN, karras2020styleganAda, gui2020ganreview}. Though GANs generate images with high fidelity, they often lack high diversity~\citep{ravuri2019CAS}. However, samples from recently proposed diffusion process based models achieve both high diversity and fidelity~\citep{ho2020denoisingdiffusion, nichol2021improvedDdpm}.

\noindent \textbf{Evaluating quality of samples from a generative model.} Fréchet Inception Distance (FID)~\citep{Heusel2017FID} and Inception Score (IS)~\citep{Heusel2017FID} are two key metrics to evaluate the quality of samples from generative models. While IS considers only generated images, FID considers both generative and real-world images. We find that better FID or Inception score may not translate to higher robustness with synthetic data. Another line of work evaluates generative models by training a classifier on its generated samples and testing it on real-world data~\citep{ravuri2019CAS, semeniuta2018accGanEval}. \vikash{\url{https://www.cs.cmu.edu/~clean-fid/} More evidence on subtle nature of FID.}

\noindent \textbf{Using generative models to improve adversarial robustness.} Earlier works have used generative models to learn training data manifold and the use it to map input samples to data manifold~\citep{samangouei2018defenseGan, jalal2017robustmanifold, Xu2018featsqueeze}. However, most of these techniques are broken against adaptive attacks~\citep{athalye2018obfuscatedGrad, Tramer2020AdaptiveAttack}. We use generative models to sample additional training samples which lead to further improvement in adversarial robustness. 
%\vikash{Make sure we aren't missing any work here.}

\noindent \textbf{Additional applications of proxy distributions.} While we use proxy distributions to improve robustness, synthetic samples from proxy distributions are also useful in privacy-preserving healthcare~\citep{jordon2018pateGan}, autonomous driving~\citep{mayer2016synDriving}, crowd-counting~\citep{wang2019countCrowd}, text recognition~\citep{jaderberg2014synTextReco, ye2018AnotherCaptcha}, and natural language processing~\citep{marzoev2020unnaturalLangProcess, puri2020syntheticQA}. Earlier works have also created dedicated synthetic datasets for some of these applications~\citep{gaidon2016virtualkitti, mayer2018viewSynthetic}. \vikash{Add domain randomization citation.}

\noindent \textbf{Comparison with} \citep{rebuffi2021fixingaugmentation}\textbf{.}  A concurrent work by ~\citep{rebuffi2021fixingaugmentation} also uses samples from generative models to improve adversarial robustness. While it broadly focuses on the effect of different data augmentations, with synthetic samples from a proxy distribution being one of them, our goal is to delve deeper into the integration of proxy distribution in adversarial training. This includes providing tight bounds on the transfer of adversarial robustness from the proxy distribution followed by empirical analysis of the transfer of robustness, accuracy vs robustness trade-off, and sample complexity of adversarial training. We also demonstrate an improvement in certified robust accuracy using proxy distributions. However, despite the differences, similar benefits of using generative models in two independent works further ascertain the importance of this research direction. 
%\vikash{Go over todo list again.}
\vikash{Relate to active learning, core-set estimation. Relate to Sanjeev's Simons'17 talk on how bounded capacity discriminator can have hard time distinguishing this may not achieve sufficient diversity. We can also see if smaller networks can still distiguish between real and synthetic.}

==> Proxy distributions [ICLR 2022]/sections/concise_background.tex <==
\noindent \textbf{Transfer of adversarial robustness.} This line of work focuses on the transfer of adversarial robustness, i.e., correct classification even under adversarial perturbations, when testing the model on different data distributions~\citep{shafahi2020AdvRobustTransfer, sehwag2019analyzing}. Note that this is different from just achieving correct classification on unmodified images across different distributions~\citep{taori2020NatShiftRobust, hendrycks2019CommonCorrupt}. Here we provide a theoretical analysis of the transfer of adversarial robustness between data distributions. 

\noindent \textbf{Using extra curated real-world data in robust training.} Prior works \citep{zhai2019advJustmoreData, carmon2019unlabeled, alayrac2019unsupadv, najafi2019advIncompleteData, deng2020AdvExtraOutDomain} have argued for using more training data in adversarial training and often resort to curating additional real-world samples. In contrast, we model the proxy distribution from the limited training images available and sample additional synthetic images from this distribution.

\noindent \textbf{Generative models for proxy distributions.}
State-of-the-art generative models are capable of modeling the distribution of current large-scale image datasets. In particular, generative adversarial networks (GANs) have excelled at this task~\citep{goodfellow2014GAN, karras2020styleganAda, gui2020ganreview}. Though GANs generate images with high fidelity, they often lack high diversity~\citep{ravuri2019CAS}. However, samples from recently proposed diffusion process based models achieve both high diversity and fidelity~\citep{ho2020denoisingdiffusion, nichol2021improvedDdpm}. Fréchet Inception Distance (FID)~\citep{Heusel2017FID} and Inception Score (IS)~\citep{Heusel2017FID} are two common metrics to evaluate the quality of samples from generative models.

\noindent \textbf{Using generative models to improve adversarial robustness.} Earlier works have used generative models to learn training data manifold and the use it to map input samples to data manifold~\citep{samangouei2018defenseGan, jalal2017robustmanifold, Xu2018featsqueeze}. However, most of these techniques are broken against adaptive attacks~\citep{athalye2018obfuscatedGrad, Tramer2020AdaptiveAttack}. We use generative models to sample additional training samples which further improve the adversarial robustness. 

\noindent \textbf{Comparison with \citet{rebuffi2021fixingaugmentation}.} A concurrent work by ~\citet{rebuffi2021fixingaugmentation} also uses randomly sampled synthetic images to improve adversarial robustness. In comparison, we provide a theoretical analysis of when synthetic data helps along with metrics to optimize the selection of both generative models and individual samples. We also demonstrate an improvement in certified robust accuracy using synthetic samples. Despite these differences, similar benefits of using proxy distributions in two independent and concurrent works further ascertain the importance of this research direction.

==> Proxy distributions [ICLR 2022]/sections/discussion.tex <==
Using synthetic data has been a compelling solution in many applications, such as healthcare~\citep{jordon2018pateGan} and autonomous driving~\citep{mayer2016synDriving} since it makes collecting a large amount of data feasible. In a similar spirit, we use synthetic data to make deep neural networks more robust against adversarial attacks. \bluetext{We investigate foundational questions such as determining the transfer of robustness from synthetic to real data and determining selection criteria for how to choose generative models or individual samples.}
\bluetext{Finally, we note that while it is crucial to improve robustness against the threat of adversarial examples, it also has an unwanted side-effect in domains where adversarial examples are used for good. Recent works use them to provide privacy on the web~\citep{shan2020fawkes} or to evade website fingerprinting methods~\citep{rahman2020mockingbird}. Improving defenses against adversarial examples will negatively hurt these applications.}

==> Proxy distributions [ICLR 2022]/sections/experiments.tex <==
First, we show that our proposed approach of using proxy distributions brings significant improvements in the performance of both adversarial training and randomized smoothing across both $\ell_{\infty}$ and $\ell_2$ threat models (Section~\ref{sec: sota}).
\newtext{ We also uncover that diffusion-based generative models are more effective proxy distributions than generative adversarial networks (GANs) on multiple datasets. Next we delve deeper into why diffusion-based generative models are highly effective proxy distributions (Section~\ref{sec:AURCP_calculation}). We find that the key reason behind the success of diffusion based models is the that there is no \emph{robust} discriminator that can \emph{robustly} distinguish between the samples from diffusion based models and real data distribution. We demonstrate that our proposed metric (\emph{\aurpc}) provides a better characterization of the effectiveness of diffusion-based models than other widely used metrics. Finally, we investigate the effectiveness of adaptively selecting synthetic images in our framework.}

% First, we discuss the choice of proxy distribution in Section~\ref{sec:AURCP_calculation} where we demonstrate that our proposed \emph{\aurpc} metric significantly outperforms other metrics (like FID, IS) at this task. Second, we delve deeper into the question of which synthetic samples to select (Section~\ref{sec: rejection_sampling}). We demonstrate the effectiveness of the proposed synthetic score in making this selection. 
% %
% We use this optimized selection of both proxy distribution and individual samples in our final results in Section~\ref{sec: sota}. We show that our proposed approach provides significant improvements in the performance of both adversarial training and randomized smoothing across both $\ell_{\infty}$ and $\ell_2$ threat model. \vikash{Cut it down. Update the flow.}
% }


\subsection{Improving robustness using synthetic images from proxy distributions} \label{sec: sota}

\noindent \textit{Setup.}
\newtext{We consider five datasets, namely CIFAR-10~\citep{krizhevsky2014cifar}, CIFAR-100~\citep{krizhevsky2014cifar}, CelebA~\citep{liu2015CelebA}, AFHQ~\citep{choi2020starganv2}, and ImageNet~\citep{deng2009imagenet}. We also work with commonly used $l_{\infty}$ and $l_2$ threat models for adversarial attacks and use AutoAttack~\citep{croce2020autoattack} to measure robustness. We provide extensive details on the setup in Appendix~\ref{app: setup}.}

\noindent \textit{Evaluation metrics for robust training.} We use two key metrics to evaluate performance of trained models: \textit{clean accuracy} and \textit{robust accuracy}. While the former refers to the accuracy on unmodified test set images, the latter refers to the accuracy on adversarial examples generated from test set images. \bluetext{We refer to the robust accuracy of any discriminator trained to distinguish between synthetic and real data as robust discrimination accuracy.} We also use randomized smoothing to measure certified robust accuracy, i.e., robust accuracy under strongest possible adversary in the threat model.

\noindent \textit{Synthetic data.} \newtext{We sample synthetic images from a generative models, in particular from denoising diffusion-based probabilistic models (DDPM)~\citep{ho2020denoisingdiffusion, nichol2021improvedDdpm}. We provide extensive details on the number of images sampled and the sampling procedure in Appendix~\ref{app: setup}. We use $\gamma=0.4$ as it achieves best results (Appendix~\ref{app: sota}). We combine real and synthetic images in a $1$:$1$ ratio in each batch, thus irrespective of the number of synthetic images, our training time is only twice of the baseline methods.} 

% We use a set of $10$M randomly sampled synthetic images from the \ddpm model for the random sampling setup. For adaptive sampling, we sample an additional $5$M images and select $10$M images with the lowest synthetic score from the combined set of $15$M\footnote{\bluetext{We use the $6$M randomly sampled images made available by \citet{nakkiran2021deepbootstrap} along with $9$M more sampled by us using improved sampling techniques~\citep{nichol2021improvedDdpm} from the \ddpm model}.} images. We use a very high number of synthetic images as more synthetic images lead to better performance transfer (Appendix~\ref{app: sample_complexity}). We use $\gamma=0.4$ as it achieves best results (Appendix~\ref{app: sota}). We combine real and synthetic images in a $1$:$1$ ratio in each batch and train for 200 epochs, which is equivalent to a single pass through all synthetic images. 

\begin{table}[!htb]
    \centering
    \caption{\textbf{State-of-the-art adversarial robustness.} \bluetext{Comparing experimental results of our framework (\ours) with baselines for adversarial training on the CIFAR-10 dataset for both $\ell_{\infty}$ and $\ell_2$ threat model.} We sample synthetic images from the diffusion-based generative model (DDPM). 
    %Using additional synthetic data brings a large gain in adversarial robustness across network architectures and threat models. \bluetext{We also show further improvements brought in by adaptive sampling, in comparison to random sampling, of synthetic images.} 
    \textit{Clean}/\textit{Auto} refers to clean/robust accuracy measured with AutoAttack.}
    \label{tab: sota}
    \vspace{-5pt}
    \begin{subtable}[h]{0.49\textwidth}
        \centering
        \caption{$\ell_{\infty}$ threat model.}
        % \label{tab: sota_1}
        \renewcommand{\arraystretch}{1.2}
        \resizebox{0.99\linewidth}{!}{\begin{tabular}{ccccc}
        \toprule
        Method & Architecture & Parameters (M) & \textit{Clean} & \textit{Auto} \\ \midrule
        \citet{zhang2019tradeoff} & ResNet-18 & $11.2$ & $82.0$ & $48.7$ \\ 
        \ours & ResNet-18 & $11.2$ & $\boldsymbol{84.6}$ & $\boldsymbol{55.7}$ \\ \midrule
        % \citet{madry2017towards} &  ResNet-50 & 23.5 & 87.0 & 49.0  \\
        \citet{rice2020overfitadv} & \wrn{34-20} & $184.5$ & $85.3$ & $53.4$ \\
        \citet{gowal2020uncoveringadv} & \wrn{70-16} & $266.8$ & $85.3$ & $57.2$
        \\ \midrule
        \citet{zhang2019tradeoff} & \wrn{34-10} & $46.2$ & $84.9$ & $53.1$ \\
        \ours  & \wrn{34-10} & $46.2$ & $\boldsymbol{87.0}$ & $\boldsymbol{60.6}$ \\
        \bottomrule
        \end{tabular}}
    \end{subtable} \hfill
    \begin{subtable}[h]{0.49\textwidth}
        \centering
        \caption{$\ell_2$ threat model.}
        \renewcommand{\arraystretch}{1.2}
        \resizebox{0.99\linewidth}{!}{\begin{tabular}{cccccc}
        \toprule
        Method & Architecture & Parameters (M) & \textit{Clean} & \textit{Auto} \\ \midrule
        \citet{rice2020overfitadv} & ResNet-18 & $11.2$ & $88.7$ & $67.7$ \\
        \ours & ResNet-18 & $11.2$ & $\boldsymbol{89.8}$ & $\boldsymbol{74.4}$
        \\ \midrule
        \citet{madry2017towards} & ResNet-50 & $23.5$ & $90.8$ & $69.2$ \\
        \citet{gowal2020uncoveringadv} & \wrn{70-16} & $266.8$ & $90.9$  & $74.5$
        \\ \midrule
        \citet{wu2020adversarial} & \wrn{34-10} & $46.2$ & $88.5$ & $73.7$ \\
        \ours & \wrn{34-10} & $46.2$ & $\boldsymbol{90.8}$ & $\boldsymbol{77.8}$
        \\ \bottomrule
        \end{tabular}}
     \end{subtable}
\end{table}


\subsubsection{Improving performance of adversarial training} \label{sec: sota_adv}
\textbf{State-of-the-art robust accuracy synthetic images (Table~\ref{tab: sota}, \ref{tab: sota_new}).} 
Using synthetic images from diffusion-based generative models (DDPM), our approach achieves state-of-the-art robust accuracy in the category of not using any extra real world data~\citep{croce2020robustbench}. \newtext{We improve robust accuracy by up to $7.5$\% and $6.7$\% over previous works in $\ell_{\infty}$ and $\ell_2$ threat model, respectively. Notably, the gain in performance is highest for the CIFAR-10 and Celeb-A datasets. Note that by using only synthetic images, our work also achieves competitive performance with previous works that use extra real-world images. For example, using additional real-data \citet{carmon2019unlabeled} achieve $59.53$\% robust accuracy on CIFAR-10 ($\ell_{\infty}$) while we achieve $60.6$\% robust accuracy by using only synthetic data.}
% In the $\ell_{\infty}$ threat model and using a \wrn{34-10} network, it improves it to $60.6$\% robust accuracy, an improvement of $7.5$\% over previous work using the same network. Similarly, we observe an improvement by up to $6.7$\% in the $l_2$ threat model. Our adaptive sampling achieves an average of $0.5$\% and $0.2$\% improvement in robust accuracy over random sampling in the $\ell_2$ and $\ell_{\infty}$ threat model, respectively.}



%%%% FIX comilation issue in this table.
\begin{table}[!htb]
    \vspace{-5pt}
    \caption{\textbf{Similar improvement on additional datasets}. \newtext{Our approach further improves both clean and robust accuracy on each of datasets of Tables \ref{tab: sota} and \ref{tab: sota_new}. Unless a better baseline is available in previous works, we compare our results with baseline robust training approach from \citet{madry2017towards}.  \textit{Clean}/\textit{Auto} refers to clean/robust accuracy measured with AutoAttack. We provide results for AFHQ dataset in Table~\ref{tab: afhq_table} in Appendix.}}
    \vspace{-5pt}
    \label{tab: sota_new}
    \begin{subtable}{.35\linewidth}
        \centering
        \caption{CelebA ($64\times64$)}
        \renewcommand{\arraystretch}{1.3}
        % \Large
        \resizebox{\linewidth}{!}{
        \begin{tabular}{cccccc} \toprule
         & \multicolumn{2}{c}{$\ell_\infty (\epsilon=8/255)$} &  & \multicolumn{2}{c}{$\ell_2 (\epsilon=1.0)$} \\ \cmidrule{2-3} \cmidrule{5-6}
         & \textit{Clean} & \textit{Auto} &  & \textit{Clean} & \textit{Auto} \\ \midrule
        Baseline & $82.4$ & $60.2$ &  & $80.6$ & $58.9$ \\
        \ours & $84.8$ & $63.4$ &  & $82.3$ & $60.0$ \\
        $\Delta$ & $\boldsymbol{\texttt{+}2.4}$ & $\boldsymbol{\texttt{+}3.2}$	&  & $\boldsymbol{\texttt{+}1.7}$ & $\boldsymbol{\texttt{+}1.1}$ \\ \bottomrule
    \end{tabular}}
    \end{subtable} \hfill
    \begin{subtable}{.35\linewidth}
        \centering
        \caption{CIFAR-100 ($32\times32$)}
        \renewcommand{\arraystretch}{1.3}
        % \Large
        \resizebox{\linewidth}{!}{
        \begin{tabular}{cccccc} \toprule
         & \multicolumn{2}{c}{$\ell_\infty (\epsilon=8/255)$} &  & \multicolumn{2}{c}{$\ell_2 (\epsilon=0.5)$} \\ \cmidrule{2-3} \cmidrule{5-6}
         & \textit{Clean} & \textit{Auto} &  & \textit{Clean} & \textit{Auto} \\ \midrule
        Baseline & $58.4$ & $27.8$ &  & $62.9$ & $42.1$ \\
        \ours & $65.9$ & $31.2$ &  & $70.7$ & $47.8$ \\
        $\Delta$ & $\boldsymbol{\texttt{+}7.5}$ &  $\boldsymbol{\texttt{+}3.4}$	&  &  $\boldsymbol{\texttt{+}7.8}$ &  $\boldsymbol{\texttt{+}5.7}$ \\ \bottomrule
    \end{tabular}}
    \end{subtable} \hfill 
    \begin{subtable}{.23\linewidth}
    \centering
    \caption{ImageNet ($64\times64$)}
    \renewcommand{\arraystretch}{1.3}
    \tiny
    \resizebox{\linewidth}{!}{
    \begin{tabular}{ccc} \toprule
         & \multicolumn{2}{c}{$\ell_\infty (\epsilon=2/255)$} \\ \cmidrule{2-3}
         & \textit{Clean} & \textit{Auto}  \\ \midrule
        Baseline & $54.8$ & $28.1$\\
        \ours & $55.1$ & $28.4$ \\
        $\Delta$ & $\boldsymbol{\texttt{+}0.3}$ & $\boldsymbol{\texttt{+}0.3}$ \\ \bottomrule
    \end{tabular}}
\end{subtable}
\vspace{-10pt}
\end{table}

% \begin{table}[!htb]
%     \centering
%     \caption{Additional baselines. When comparing with trades, we uses PORT with trades loss. }
%     \centering
%     \caption{ImageNet ($64\times64$)}
%     \renewcommand{\arraystretch}{1.3}
%     \tiny
%     \resizebox{0.4\linewidth}{!}{
%     \begin{tabular}{ccccccc} \toprule
%          & \multicolumn{2}{c}{\begin{tabular}[c]{@{}c@{}}CIFAR-100 \\ $\left(\ell_\infty (\epsilon=8/255)\right)$\end{tabular}} & & & \multicolumn{2}{c}{\begin{tabular}[c]{@{}c@{}}CelebA \\ $\left(\ell_\infty (\epsilon=8/255)\right)$\end{tabular}} \\ \cmidrule{2-3} \cmidrule{6-7}
%          & \textit{Clean} & \textit{Auto} & &  & \textit{Clean} & \textit{Auto} \\ \midrule
%         \citet{wu2020AdvWeightPerturb} & $60.4$ & $28.9$ & & TRADES & $86.1$ & $61.2$ \\
%         \citet{rade2021helperBasedAdvTrain} & $61.5$ & $28.9$ &  & \ours & $86.1$ & $62.7$ \\
%         \citet{cui2021BoundaryGuideAdv} & $60.6$ & $29.3$ & & $\Delta$  & $0.0$ & $\boldsymbol{1.5}$ \\
%         \ours & $60.6$ & $\boldsymbol{30.5}$ & & -- & -- & -- \\ \bottomrule
%     \end{tabular}}
% \end{table}


\begin{wraptable}{r}{0.4\linewidth}
    \centering
    % \vspace{-10pt}
    \newbluetext{
    \caption{\newbluetext{\textbf{Additional baselines.} Using $\ell_\infty (\epsilon=8/255)$ attack for both datasets.}}
    \vspace{-5pt}
    \renewcommand{\arraystretch}{1.3}
    \tiny
    \resizebox{\linewidth}{!}{
    \begin{tabular}{ccc} \toprule
        %  & \multicolumn{2}{c}{\begin{tabular}[c]{@{}c@{}}CIFAR-100\end{tabular}} \\ \cmidrule{2-3}
        CIFAR-100 & \textit{Clean} & \textit{Auto} \\ \midrule
        \citet{wu2020AdvWeightPerturb} & $60.4$ & $28.9$ \\
        \citet{rade2021helperBasedAdvTrain} & $\boldsymbol{61.5}$ & $28.9$ \\
        \citet{cui2021BoundaryGuideAdv} & $60.6$ & $29.3$ \\
        \ours & $60.6$ & $\boldsymbol{30.5}$ \\ \midrule
        % & \multicolumn{2}{c}{\begin{tabular}[c]{@{}c@{}}CelebA\end{tabular}} \\  \cmidrule{2-3}
        CelebA & \textit{Clean} & \textit{Auto} \\ \midrule
        TRADES & $86.1$ & $61.2$ \\
        \ours & $86.1$ & $62.7$ \\
        $\Delta$  & $0.0$ & $\boldsymbol{1.5}$ \\ \bottomrule
    \end{tabular}}
    }
    \vspace{-15pt}
\end{wraptable}



% \begin{table}[!hb]
%     \caption{\textbf{Additional datasets}. Using synthetic data also improves clean and robust accuracy on CelebA~\citep{liu2015CelebA} and AFHQ~\citep{choi2020starganv2} datasets. Note that the improvement in robust accuracy is significantly higher than the improvement in clean accuracy. Baseline refers to adversarial training based on Madry et al.~\citep{madry2017towards}. \textit{Clean}/\textit{Auto} refers to clean/robust accuracy measured with AutoAttack. We use a ResNet-18 network and randomly sampled synthetic images for each dataset. \vikash{Only keep one epsilon number in the main paper.}}
%     \label{tab: add_datasets}
%     \begin{subtable}{.48\linewidth}
%         \centering
%         \caption{CelebA ($64\times64$)}
%         \renewcommand{\arraystretch}{1.4}
%         \Large
%         \resizebox{\linewidth}{!}{
%         \begin{tabular}{cccccccccccc} \toprule
%              & \multicolumn{5}{c}{$\ell_\infty$} &  & \multicolumn{5}{c}{$\ell_2$} \\ \cmidrule{2-6} \cmidrule{8-12}
%             $\epsilon$ & \multicolumn{2}{c}{$4/255$} &  & \multicolumn{2}{c}{$8/255$} &  & \multicolumn{2}{c}{$0.5$} &  & \multicolumn{2}{c}{$1.0$} \\ \midrule
%              & \textit{Clean} & \textit{Auto} &  & \textit{Clean} & \textit{Auto} &  & \textit{Clean} & \textit{Auto} &  & \textit{Clean} & \textit{Auto} \\
%             Baseline & $87.0$ & $72.4$ &  & $82.4$ & $61.5$ &  & $85.8$ & $73.3$ &  & $81.1$ & $63.0$ \\
%             \ours & $87.5$ & $74.9$	&  & $84.2$ & $64.5$ &  & $86.7$ & $75.3$ &  & $82.3$ & $64.6$ \\
%             $\Delta$ & $\boldsymbol{\texttt{+}0.5}$ & $\boldsymbol{\texttt{+}2.5}$	&  & $\boldsymbol{\texttt{+}1.8}$ & $\boldsymbol{\texttt{+}3.0}$ &  & $\boldsymbol{\texttt{+}0.9}$ & $\boldsymbol{\texttt{+}2.0}$ &  & $\boldsymbol{\texttt{+}1.2}$	& $\boldsymbol{\texttt{+}1.6}$ \\ \bottomrule
%         \end{tabular}}
%     \end{subtable} \hfill
%     \begin{subtable}{.48\linewidth}
%         \centering
%         \caption{CIFAR-100 ($32\times32$)}
%         % \renewcommand{\arraystretch}{1.4}
%         % \Large
%         \resizebox{\linewidth}{!}{
%         \begin{tabular}{cccccccccccc} \toprule
%           -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\
%           -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\
%           -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\
%           -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\
%           -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\
%           -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\ \bottomrule
%         \end{tabular}}
%     \end{subtable}

% \end{table}

\noindent \textbf{Proxy distribution offsets increase in network parameters.} We find that gains from using synthetic samples are equivalent to ones obtained by scaling network size by an order of magnitude (Table~\ref{tab: sota}). For example, a ResNet-18 network with synthetic data achieves higher robust accuracy ($\ell_{\infty}$) than a \wrn{34-20} trained without it, while having $16\times$ fewer parameters than the latter. Similar trend holds for \wrn{34-10} networks, when compared with a much larger \wrn{70-16} network. This trend also holds for both $\ell_{\infty}$ and $\ell_2$ threat models.

\noindent \textbf{Simultaneous improvement in clean accuracy.} Due to the accuracy vs robustness trade-off in adversarial training, improvement in robust accuracy often comes at the cost of clean accuracy. However synthetic samples provide a boost in both clean and robust accuracy, simultaneously. Using adaptively sampled synthetic images, we observe improvement in clean accuracy by up to $7.5$\% and $7.8$\% across $\ell_{\infty}$ and $\ell_2$ threat models, respectively. 

\newtext{\noindent \textbf{Comparison across generative models.} We find that synthetic samples from diffusion-based generative models~\citep{ho2020denoisingdiffusion, nichol2021improvedDdpm} provides significantly higher improvement in performance than generative adversarial networks (GANs) (Table~\ref{tab: gan_vs_ddpm}). We further investigate this phenomenon in the next section.
}

We further analyze sample complexity of adversarial training using synthetic data in Appendix~\ref{app: sample_complexity}. We also provide visual examples of real and synthetic images for each dataset at the end of the paper. 

\begin{figure*}[!htb]
	\centering
	\vspace{-5pt}
	\begin{minipage}{0.32\linewidth}
		\centering
		\captionof{table}{\newtext{\textbf{Comparing generative models.} When choosing proxy distribution in \ours ($\ell_{\infty}$), DDPM model outperforms the leading generative adversarial network (GAN) on each dataset.}}
		\label{tab: gan_vs_ddpm}
		\renewcommand{\arraystretch}{1.1}
		\resizebox{0.9\linewidth}{!}{
		\begin{tabular}{cccc} \toprule
            Dataset & \begin{tabular}[c]{@{}c@{}}Proxy \\ Distribution\end{tabular} & \textit{Clean} & \textit{Auto} \\ \midrule
            \multirow{3}{*}{CIFAR-10} & None & $84.9$ & $53.1$ \\ 
             & StyleGAN & $86.0$ & $52.5$ \\
             & DDPM & $\boldsymbol{87.0}$ & $\boldsymbol{60.6}$ \\ \midrule
            \multirow{3}{*}{CelebA} & None & $82.4$ & $60.2$ \\ 
             & StyleFormer & $84.1$ & $63.1$ \\
             & DDPM & $\boldsymbol{84.8}$ & $\boldsymbol{63.4}$ \\ \midrule
            \multirow{3}{*}{ImageNet} & None & $54.8$ & $28.1$ \\
             & BigGAN & $54.5$ & $28.2$ \\
             & DDPM & $\boldsymbol{55.1}$ & $\boldsymbol{28.4}$ \\ \bottomrule
        \end{tabular}}
	\end{minipage} \hfill
	\begin{minipage}{0.32\linewidth}
		\centering
	    \includegraphics[width=0.98\linewidth]{images/smoothing_results.pdf}
        \caption{\textbf{Certified robustness.} Certified robust accuracy of baseline randomized smoothing technique, i.e., RST~\citep{carmon2019unlabeled} and our work at different perturbation budgets across two different network architectures.}
        \label{fig: vra}
	\end{minipage}
	\hfill
	\begin{minipage}{0.32\linewidth}
		\centering
		\captionof{table}{\textbf{Comparison of certified robustness.} Comparing clean accuracy (\textit{Clean}) and certified robust accuracy (\textit{Certified}) of our work with earlier approaches at $110/255$ $\ell_2$ perturbation budget (equivalent to $2/255$ $\ell_{\infty}$ perturbation budget) on the CIFAR-10 dataset.}
		\label{tab: vra}
		\renewcommand{\arraystretch}{1.1}
		\resizebox{\linewidth}{!}{
		\large
		\begin{tabular}{ccc}
		   \toprule
		   Method  &  \textit{Clean} & \textit{Certified} \\ \midrule
		   \citet{Wong2018ScalingProve} (single) & $68.3$ & $53.9$\\
		   \citet{Wong2018ScalingProve} (ensemble) & $64.1$ & $63.6$ \\
		   \newbluetext{CROWN-IBP (\cite{Zhang2020crownIbp})} & $71.5$ & $54.0$ \\
		   \citet{balunovic2019advPlusProve} & $78.4$ & $60.5$ \\
		   RST (\citet{carmon2019unlabeled}) & $77.9$ & $58.6$ \\
		   RST$_{500K}$ (\citet{carmon2019unlabeled}) &  $80.7$ & $63.8$ \\ 
		   \ours (ResNet-18) & $79.4$ & $\boldsymbol{64.6}$ \\
		   \ours (\wrn{28-10}) & $80.4$ & $\boldsymbol{66.2}$ \\
		   \bottomrule
		\end{tabular}}
	\end{minipage}
\end{figure*}



% \begin{table}[!htb]
% \centering
% \caption{ToDo.}
% \label{tab: gan_vs_ddpm}
% \begin{tabular}{cccc} \toprule
% Dataset & \begin{tabular}[c]{@{}c@{}}Proxy \\ Distribution\end{tabular} & \textit{Clean} & \textit{Auto} \\ \midrule
% \multirow{3}{*}{CIFAR-10} & None & -- & -- \\ 
%  & StyleGAN & -- & -- \\
%  & DDPM & -- & -- \\ \midrule
% \multirow{3}{*}{CelebA} & None & -- & -- \\ 
%  & StyleFormer & -- & -- \\
%  & DDPM & -- & -- \\ \midrule
% \multirow{3}{*}{ImageNet} & None & -- & -- \\
%  & BigGAN & -- & -- \\
%  & None & -- & -- \\ \bottomrule
% \end{tabular}
% \end{table}


% \noindent \textbf{Similar trend on additional datasets.}  We further experimented with two more datasets, namely Celeb-A [3] and AFHQ [4]. Similar to the trend on the CIFAR-10 dataset, proxy distribution consistently improves both clean accuracy and robustness on both datasets (Table~\ref{tab: add_datasets}). We provide further details on the experimental setup in Appendix~\ref{app: setup}. 

% \noindent \textbf{Limitation of generative models on ImageNet dataset.} \bluetext{We combine synthetic images from the two state-of-the-art generative models, namely BigGAN~\citep{brock2018bigGandeep} and Improved-DDPM~\citep{nichol2021improvedDdpm}, with training image of ImageNet ($64\times64$) dataset for adversarial training. Using additional synthetic images here led to a degradation of performance (Table~\ref{tab: beyond_cifar}).} 

\subsubsection{Improving certified robustness with randomized smoothing} \label{sec: sota_certify}

We provide results on certified adversarial robustness in Table~\ref{tab: vra}.
% We provide results on certified adversarial robustness in Figure~\ref{fig: vra} and Table~\ref{tab: vra}. 
We first compare the performance of our proposed approach with the baseline technique, i.e., RST~\citep{carmon2019unlabeled}. We achieve significantly higher certified robust accuracy than the baseline approach at all $\ell_2$ perturbations budgets for both ResNet-18 and \wrn{28-10} network architectures. Additionally, the robustness of our approach decays at a smaller rate than the baseline. At $\ell_{\infty}$ perturbation of $2/255$, equivalent to $\ell_2$ perturbation of $111/255$, our approach achieves $7.6$\% higher certified robust accuracy than RST. We also significantly outperform other certified robustness techniques which aren't based on randomized smoothing~\citep{Zhang2020crownIbp, Wong2018ScalingProve, balunovic2019advPlusProve}. Along with better certified robust accuracy, our approach also achieves better clean accuracy than most previous approaches, simultaneously. 

\noindent \textbf{Synthetic images vs real-world images.} 
Using only synthetic samples ($10$M), we also outperform RST where it uses an additional curated set of $500$K real-world images (RST$_{500K}$). While the latter achieves $63.8$\% certified robust accuracy, we improve it to $66.2$\%. \vikash{Discuss results when using only 500k synthetic images.}


\subsection{Delving deeper into use of proxy distributions in robust training}\label{sec:AURCP_calculation}
\newtext{Earlier in Section~\ref{sec: sota} we showed that diffusion-based generative models are an excellent choice for a proxy distribution for many datasets. Now we characterize the benefit of individual proxy distributions in our robust training framework. We consider seven different generative models, which are well-representative of the state-of-the-art on the CIFAR-10 dataset.  } 

% \noindent \textit{Proxy distributions.} \newtext{We consider seven different generative models for CIFAR-10 and four generative models for CelebA dataset. Due to space constraint, we present CelebA results in Appendix xyz.}

% \subsubsection{Why diffusion based models are an excellent choice as proxy distributions?}

\noindent \emph{Using synthetic-to-real transfer of robustness as ground truth.} From each generative model we sample one million synthetic images. We adversarially train a ResNet-18~\citep{he2016resnet} network on these images and rank generative models in order of robust accuracy achieved on the CIFAR-10 test set. We provide further experimental setup details in Appendix~\ref{app: aurpc}.

\noindent \emph{Calculating \aurpc.} At each perturbation budget ($\epsilon$), we adversarially train a ResNet-18 classifier to distinguish between synthetic and real images. We measure robust discrimination accuracy of trained classifier on a balanced held-out validation set. We calculate \aurpc by measuring the area under the robust discrimination accuracy and perturbation budget curve\footnote{We use \texttt{numpy.trapz(Racc-0.5, $\epsilon$)} to calculate \emph{\aurpc}.} (Figure~\ref{fig: aurpc}). We provide a detailed comparison of it with other metrics in Table~\ref{tab: gan_comaprison}.

\begin{figure*}[!htb]
	\centering
	\begin{minipage}{0.32\linewidth}
		\centering
        \includegraphics[width=0.9\linewidth]{images/robust_synthetic_real_binary_classification_with_epsilon_adv.pdf}
        \caption{\bluetext{\textbf{Calculating \emph{\aurpc}.} For every generative model and perturbation budget ($\epsilon$), we first adversarially train a binary classifier on adversarial perturbed synthetic and CIFAR-10 images. Next we measure its robust discrimination accuracy on the validation set at the $\epsilon$ value used in training. \emph{\aurpc} is the area under the robust discrimination accuracy vs $\epsilon$ curve.}}
        \label{fig: aurpc}
	\end{minipage}
	\hfill
	\begin{minipage}{0.65\linewidth}
		\centering
		\captionof{table}{\textbf{Comparing different generative models.} \bluetext{We first adversarially train a ten class ResNet-18 model \textit{only} on $1$M synthetic images and measure its robust accuracy on the CIFAR-10 test set. We use this transferred robustness as a ground truth for benefit of each model. Next we match ranking predicted by each metric with the ground truth ranking. In contrast to all three three baseline, ranking from our proposed metric (\emph{\aurpc}) accurately matches the ground-truth.} \vikash{Use AA robust accuracy. Report FID/IS of our sampled images? Add other FID variations too. Color table header.}}
        \label{tab: gan_comaprison}
        \renewcommand{\arraystretch}{1.2}
        \resizebox{0.9\linewidth}{!}{
        \begin{tabular}{ccc||cccc}
            \toprule
            Rank & Model & \begin{tabular}[c]{@{}c@{}}Robust \\ accuracy\end{tabular} & \begin{tabular}[c]{@{}c@{}}FID ($\downarrow$)\end{tabular} & IS ($\uparrow$) & \oneNN ($\downarrow$) & \aurpctt ($\downarrow$) \\ \midrule
            -- & CIFAR-10 \footnote{\tiny Using 50,000 training images from the CIFAR-10 dataset.} & $48.7$ & --  & -- & -- & -- \\ \midrule
            $1$ & \ddpm (UC) \footnote{\tiny UC and C refers to unconditional and conditional generative models, respectively.} & $53.1$ & $3.17$ (2) & $9.46$ (2) &  $9.34$ (2) &  $0.06$ (\textbf{1}) \\
            $2$ & \styleC (C) & $45.0$ & $2.92$ (1) & $10.24$ (1) &  $9.42$ (3) & $0.32$ (\textbf{2})  \\
            $3$ & WGAN-ALP (UC) & $43.5$ & $12.96$ (7) & $8.34$ (7) & $10.10$ (7) & $1.09$ (\textbf{3})  \\ 
            $4$ & E2GAN (UC)  & $39.6$ & $11.26$ (5) & $8.51$ (5) & $8.96$ (1)  & $1.19$ (\textbf{4})  \\
            $5$ & DiffCrBigGAN (C) & $33.7$ & $4.30$ (3) & $9.17$ (3) &  $9.84$ (6)  & $1.30$ (\textbf{5})  \\ 
            $6$ & NDA  (C)& $33.4$ & $12.61$ (6) & $8.47$ (6) & $9.72$ (5) & $1.43$ (\textbf{6}) \\
            $7$ & DiffBigGAN (C) & $32.4$ & $4.61$ (4) & $9.16$ (4) &  $9.73$ (4) & $1.55$ (\textbf{7}) \\  \midrule
            \multicolumn{3}{c||}{Mean absolute ranking difference} & $1.7$ &  $1.7$ & $2.0$ & $\boldsymbol{0.0}$\\ \bottomrule
        \end{tabular}
        }
	\end{minipage}
\end{figure*}

\noindent \textbf{\textit{\aurpc} is highly effective at determining synthetic to real transfer of robustness (Table~\ref{tab: gan_comaprison}).}
\newtext{Each of the baseline metrics, including FID which is widely used, fail in accurately predicting the transfer of robustness from synthetic to real distributions. Even more, they also fail to identify DDPM~\citep{ho2020denoisingdiffusion} as the most successful proxy distribution.} Our proposed metric (\textit{\aurpc}), which measures the distinguishability of perturbed synthetic and real images, exactly predicts the ranking of different generative models in terms of the transfer of robustness. It also provides deeper insight into why synthetic samples from DDPM models are highly effective compared to other models. As shown in Figure~\ref{fig: aurpc}, discrimination between DDPM samples and real images becomes almost impossible even at very small perturbations budgets. A more detailed comparison is provided in Appendix~\ref{app: robust_disc}. 

% \noindent \textbf{FID and other existing metrics are not predictive of synthetic-to-real performance transfer.} Existing metrics, most importantly FID which is widely used, fail in accurately predicting the transfer of robustness from synthetic to real distributions. Generative models, such as WGAN-ALP~\citep{terjek2019wganALP}, E2GAN~\citep{tian2020e2gan}, which rank very low along these metrics exhibit very high transfer of robustness. Similarly, among top ranking models, they assign a higher rank to StyleGAN~\citep{karras2020styleganAda} samples, where DDPM~\citep{ho2020denoisingdiffusion} samples achieve $8.1$\% higher robust accuracy than the former. 

% \noindent \textbf{\emph{\aurpc} is most effective at predicting relative synthetic-to-real transfer of robustness.} Our proposed metric, which measures the distinguishability of perturbed synthetic and real images, exactly predicts the ranking of different generative models in terms of the transfer of robustness. It also provides deeper insight into why synthetic samples from DDPM models are highly effective compared to other models. As shown in Figure~\ref{fig: aurpc}, discrimination between DDPM samples and real images becomes almost impossible even at very small perturbations budgets. A more detailed comparison is provided in Appendix~\ref{app: robust_disc}. 

\noindent \textbf{Adaptive sampling of synthetic data based on ARC (Appendix~\ref{appsubsec: adaptive}).} We compare the benefit of adaptive sampling with random sampling on CIFAR-10 dataset (for both $\ell_2$ and $\ell_{\infty}$ threat models). Our adaptive sampling achieves an average of $0.5\%$ and $0.2\%$ improvement in robust accuracy over random sampling in the $\ell_{\infty}$ and $\ell_{\infty}$ threat models, respectively.


==> Proxy distributions [ICLR 2022]/sections/introduction.tex <==
Deep neural networks are powerful tools but their success depends strongly on the amount of training data~\citep{sun2017revisitData, mahajan2018BillionWSL}. 
Recent works show %have shown 
that for improving robust training against adversarial examples~\citep{biggio2013evasion, Szegedy2013IntrigueAdv, biggio2018wildPatterns}, additional training data is 
helpful~\citep{carmon2019unlabeled, schmidt2018AdvMoreData, alayrac2019unsupadv, deng2020AdvExtraOutDomain}.
However, curating more real-world data from the actual data distribution is usually 
challenging and costly~\citep{recht2019ImageNetv2}. 
To circumvent this challenge, we ask: can robust training be enhanced using a proxy distribution, i.e., an approximation of the \realdist distribution? 
In particular, can additional samples from a proxy distribution, that is perhaps cheaper to sample from, improve robustness. If so, can generative models that are trained on limited training images 
in small scale datasets~\citep{lecun2010mnist, krizhevsky2014cifar}, act as such a proxy distribution?\footnote{Proxy distributions may not necessarily be modeled by generative models. When a proxy distribution is the output of a generative model, we call it \emph{synthetic distribution} and refer to data sampled from it as \emph{synthetic data}.}

When training on synthetic samples from generative models, a natural question is whether robustness on synthetic data will also transfer to real world data. Even if it does, can we determine the features of synthetic data that enable this \emph{synthetic-to-real} robustness transfer and optimize our selection of generative models based on these features? Finally, can we also optimize the selection of individual synthetic samples to maximize the robustness transfer? 

\emph{Q.1} \emph{When does robustness transfer from proxy distribution to real data distribution?} This question is fundamental to develop a better understanding of whether a proxy distribution will help. \bluetext{For a classifier trained on only synthetic samples, we argue that in addition to empirical and generalization error, \emph{distribution shift} penalty also determines its robustness on the real data distribution.} We prove that this penalty is upper bounded by the \cwdfull between the \approxdist distribution and \realdist  distribution. Thus robustness will transfer from proxy distributions that are in close proximity to \realdist distribution with respect to \cwdfull. 

\emph{Q.2} \emph{\newtext{How effective are proxy distributions in boosting adversarial robustness on real-world dataset?}}
\newtext{Our experimental results on \textit{five} datasets demonstrate that the use of samples from \textit{PrOxy distributions in Robust Training} (PORT) can significantly improve robustness. In particular, PORT achieves up to to $7.5$\% improvement in adversarial robustness over existing state-of-the-art~\citep{croce2020robustbench}. Its improvement is consistent across different threat models ($\ell_{\infty}$ or $\ell_2$), network architectures, datasets, and robustness criteria (empirical or certified robustness).  We also uncover that synthetic images from diffusion-based generative models are most helpful in improving robustness on real datasets. We further investigate the use of proxy distributions in robust training. In particular, we investigate why current state-of-the-art in diffusion-based models are significantly more helpful than their counterparts, such as generative adversarial networks (GANs). 
% \vikashnew{Make sure we have enough results to back this claim? Clearly highlight its results.} 
}

\newtext{
\emph{Q.3} \emph{Can we develop a metric to characterize which proxy distribution will be most helpful in robust training?} 
% We further investigate the use of proxy distributions in robust training, in particular, to determine why diffusion-based are significantly more helpful than their counterparts, such as generative adversarial networks (GANs). 
% Though \cwdfull can determine the effective of a proxy distribution, calculating it requires knowledge of the underlying distribution of \realdist which is generally not known. 
Our theory motivates the design of a measure of proximity between two distributions that incorporates the geometry of the distributions and can empirically predict the transfer of robustness.}
We propose a robust learning based approach where we use the success of a discriminator in distinguishing adversarially perturbed samples of synthetic and real data as a measure of proximity. Discriminating between synthetic and real data is a common practice~\citep{goodfellow2014GAN, gui2020ganreview},
\bluetext{however, we find that considering adversarial perturbations on synthetic and real data samples is the key to making the discriminator an effective measure for this task.} 
We demonstrate that the rate of decrease in discriminator success with an increasing size of perturbations can effectively measure proximity and it accurately predicts the relative transfer of robustness from different generative models. 

We also leverage our robust discriminators to identify most helpful synthetic samples. We use the proximity of each synthetic sample to \realdist distribution, referred to as synthetic score, as a metric to judge their importance. This score can be computed using output probability from a discriminator that is robustly trained to distinguish between adversarially perturbed samples from \approxdist and \realdist distribution. \bluetext{We demonstrate that selecting synthetic images based on their synthetic scores can further improve performance.}  

% \saeed{Can we optimize the proxy distribution base on our metric?}
% \emph{Q.3} \emph{Can we optimize on which synthetic samples to choose?} We find that some samples lead to higher robustness transfer than others from a proxy distribution. Understanding this sample-wise importance can enable us to adaptively sample the most helpful data points. We use the proximity of each synthetic sample to \realdist distribution, referred to as \textit{synthetic score}, as a metric to judge their importance. This score can be computed using output probability from a discriminator that is robustly trained to distinguish between adversarially perturbed samples from \approxdist and \realdist distribution. We use rejection sampling based on this score where we discard samples with a score higher than a predetermined threshold. 

% \saeed{I feel like the contributions below are a bit redundant. Can we merge them with paragraphs above? another idea is to move it to conclusion section.}
\noindent \textbf{Contributions.}
We make the following key contributions.
\begin{itemize}[noitemsep, topsep=0pt]
    \item We provide an analytical bound on the transfer of robustness from proxy distributions to \realdist distribution using the notion of conditional Wasserstein distance and further validate it experimentally.

    \item Overall, using additional synthetic images, we improve both clean and robust accuracy on \textit{five} different datasets. In particular, we improve robust accuracy by up to $7.5$\% and $6.7$\% in $\ell_{\infty}$ and $\ell_2$ threat models, respectively, and certified robust accuracy ($\ell_2$) by $7.6$\% on the CIFAR-10 dataset.
    
    \item When selecting a proxy distribution, we show that existing metrics, such as FID, fail to determine the synthetic-to-real transfer of robustness. We propose a new metric (\emph{\aurpc}) based on the distinguishability of adversarially perturbed synthetic and real data, that accurately determines the performance transfer.  
     
    \item We also develop a metric, named synthetic score, to determine the importance of each synthetic sample in synthetic-to-real robustness transfer. We demonstrate that choosing samples with lower synthetic scores provide better results than randomly selected samples.
\end{itemize}

%  given high expressive power of deep network, 
%Given dataset bias, ImageNet trained network may not best capture semantics of CIFAR-10 classes, so we also measure FID in the feature space of a 
% which measure proximity of synthetic samples to real data,
% In our analytical results, we use \cwdfull between synthetic and \realdist distribution to determine this. 
% However underlying distribution of \realdist is unknown, making it infeasible to calculate this bound. 


% To achieve robustness against adversarial examples, adversarial training remains the most effective technique~\citep{madry2017towards, zhang2019tradeoff, pang2021bagoftricks}. However, it is largely used with limited training samples available in current image datasets (such as only 50,000 training images in the CIFAR-10 dataset) where it suffers from multiple challenges, such as poor generalization on the test set~\citep{madry2017towards} and accuracy vs robustness trade-off~\citep{Raghunathan2020advtradeoff}. Recent works have demonstrated that more training data can improve the performance of adversarial training~\citep{schmidt2018AdvMoreData, alayrac2019unsupadv, deng2020AdvExtraOutDomain}. However, this approach runs into the challenge of curating a large set of real-world images for training. We circumvent this challenge using proxy distributions, distributions that closely approximate the underlying distribution of the original training dataset. Note that the proxy distributions are modeled using only available training images in current datasets. Proxy distributions when modeled with deep neural networks, such as Generative adversarial networks (GAN), allow us to generate a potentially unlimited number of high-fidelity images~\citep{goodfellow2014GAN, gui2020ganreview, ho2020denoisingdiffusion}. Our key goal is to improve the adversarial robustness of deep neural networks by taking advantage of samples from such proxy distributions.

% Note that proxy distributions are only an approximation of the underlying distribution of the training data. This begs the question of whether robustness achieved on samples from the proxy distribution will transfer to the original dataset. A more generic version of this question is \textit{how much the robustness of a classifier transfers between data distributions?} We prove that the difference in the robustness of a classifier on two distributions is \textit{tightly} upper bounded by the conditional Wasserstein distance between them. We refer to Wasserstein distance conditioned on class labels as conditional Wasserstein distance. This result confirms the intuition that samples from a proxy distribution that closely approximates training data distribution should be able to improve robustness on the latter. We also empirically validate this claim where we show that adversarial training only on samples from the proxy distribution indeed achieves non-trivial robustness on samples from the original distribution. 

% To improve adversarial robustness on current datasets, we aim to leverage samples from a \approxdist distribution which \textit{closely} approximates the underlying distribution of these datasets. Here we propose to simultaneously train on both the original training set and a set of additional images sampled from the \approxdist distribution. We use state-of-the-art generative models as a model for proxy distribution since they can closely approximate the data distribution from only a limited number of training samples~\citep{karras2020styleganAda, ho2020denoisingdiffusion, gui2020ganreview}.  Our experimental results demonstrate that the use of samples from the proxy distribution improves robust accuracy by up to $6.1$\% and $5.7$\% in $l_{\infty}$ and $l_2$ threat models, respectively, over baselines not using proxy distributions on the CIFAR-10 dataset. In the category of not using any extra real-world data, our models achieve the first rank on RobustBench~\citep{croce2020robustbench}, a standardized benchmark for adversarial training. We also improve the certified robust accuracy~\citep{cohen2019certified} by up to $6.7$\% with randomized smoothing on the CIFAR-10 dataset. Intriguingly, we achieve better certified robust accuracy with proxy distribution samples than using an additional set of $500$K curated real-world images~\citep{carmon2019unlabeled}.

% Since access to proxy distributions gives us the ability to generate a large number of images, this allows us to delve deeper into the relationship of adversarial robustness with the number of training samples on the scale of image classification with deep neural networks. Next, we work solely with a proxy distribution, where we train multiple networks with an increasing amount of training images (we use $2$K-$10$M training images) and test each on another fixed set of images from it. Our goal is to analyze multiple intriguing properties of the adversarial training w.r.t. the number of training samples. We first analyze the sample complexity of adversarial training. Earlier works \citep{wei2019allLayerMargin, bhagoji2019lowerBounds, schmidt2018AdvMoreData} have derived sample complexity bounds in simplified settings such as classifying a mixture of Gaussian distributions. On the scale of deep neural networks for image classification, we empirically demonstrate that more data continues to improve adversarial robustness. 
% %%Recently, \citep{chen2020dataHurtsAdv} and \citep{min2020datahurts} provided theoretical results suggesting more data may hurt generalization in adversarial training. We observe that both clean and robust generalization continue to improve with the number of training samples. 
% Next, we analyze the accuracy vs robustness trade-off: earlier works showed that robustness in adversarial training is achieved at a cost of clean accuracy of deep neural networks~\citep{Raghunathan2020advtradeoff, javanmard2020preciseTradeoff}. We demonstrate that increase in the number of training samples significantly reduces this trade-off for deep neural networks. To the best of our knowledge, this is the \textit{first} empirical investigation into adversarial training of deep neural networks on millions of images on the scale of CIFAR-10 dataset. \vikash{Add a summary of key results in a table.}

%% However, without access to the training data distribution, we are bounded by the limited training images available in these datasets. We aim to circumvent this issue using proxy distributions. We refer to approximations of the underlying distribution of these datasets as proxy distributions. Since we have access to this distribution, we can now sample a potentially unlimited number of samples from it, overcoming the challenges of limited training samples in current datasets\Snote{why do we have unlimited access to proxy distributions? would be good to elaborate on this.}.} 

%% \Snote{We can make a better connection to next sentense here. For example, saying generalization requires more data->we don't have more data -> we have proxy data} In this work, we analyze adversarial training through the lens of \textit{proxy} distributions. 
% We refer to approximations of the underlying distribution of these curated datasets as proxy distributions. In contrast to the limited number of training samples in the current dataset, we can now sample a potentially unlimited number of images from the proxy distribution. Our key goals are following. 

%% \bluetext{Our key goal is to improve the performance of adversarial training using samples from the proxy distribution. Though this integration looks straightforward, it poses multiple intriguing questions. Since the key advantage of a proxy distribution is to allow sampling of unlimited data points, the first question is how much does increase the number of training samples help in adversarial training on deep neural networks? Note that our goal is to improve robustness on the underlying data distribution of the training dataset. Proxy distributions remain an approximation of the underlying data distribution. So even if more training images improve robustness significantly, would it help if they are sampled from a proxy distribution? Finally, if we have a proxy distribution which closely approximates training data distribution, how can we use it to improve the performance of adversarial training. We delve deeper into each question individually below.}

%% Our next key objective is to utilize synthetic samples, i.e., samples from the proxy distribution, to improve robustness on current image datasets. However, proxy distribution is only an approximation of the true distribution of image datasets. Thus, it's unclear whether robustness acquired for proxy distribution will transfer to samples from the true data distribution. This motivates us to pursue the following goal. 

%% However, adversarially trained networks, when trained on a limited number of images available in curated datasets such as CIFAR-10~\citep{krizhevsky2009learning}, suffers from a large generalization gap in robust accuracy. In this work, we approach adversarial training on these datasets in conjunction with a \textit{proxy} distribution. We refer to approximations of the underlying distribution of these curated datasets as proxy distributions. Our use of proxy distributions allows us to target the following two objectives. 1) Since we can sample an unlimited number of samples from the proxy distribution, it allows us to investigate the effect of the number of training samples on the robust generalization of adversarial training 2) Using samples from proxy distribution to reduce the robust generalization gap in adversarial training.

%% \Snote{Alternative Questions for 1. Question 1: Can we achieve robustness on proxy distributions by performing adversarial training on large datasets sampled from them? }
%% \noindent \textbf{Q.} \textit{How does increasing number of training samples benefit adversarial training in \Snote{Maybe we can say "image classification" instead of "deep neural networks"} deep neural networks?}
%% % \noindent \textbf{Goal-1.} \textit{An empirical investigation into intriguing properties of adversarial training in the limit of infinite training samples.}
%% \bluetext{\Snote{Maybe we can say: our first step in investigating our main goal is to explore the case where proxy distribution is exactly the same as data distribution. }We aim to answer this question by analyzing intriguing properties of adversarial training on networks training on increasing number of training samples (we use 5k-10M training samples)}. We first analyze the sample complexity of adversarial training. Earlier works \citep{wei2019allLayerMargin, bhagoji2019lowerBounds, schmidt2018AdvMoreData} have derived sample complexity bounds in simplified settings such as classifying a mixture of Gaussian. We empirically demonstrate that more data continues to improve adversarial robustness but at a slower rate than clean accuracy. Recently, \citep{chen2020dataHurtsAdv, min2020datahurts} provide theoretical results suggesting more data may hurt generalization in adversarial training. We observe that both clean and robust generalization continues to improve with the number of training samples. Finally, we analyze the accuracy vs robustness trade-off where earlier works showed that robustness in adversarial training is achieved at a cost of clean accuracy of deep neural networks~\citep{Raghunathan2020advtradeoff, javanmard2020preciseTradeoff}. \textcolor{red}{rephrase: We demonstrate that increase in training samples can mitigate this trade-off for deep neural networks. }

%% We first investigate the effect of the number of training samples in adversarial training. Earlier works~\citep{carmon2019unlabeled, alayrac2019unsupadv} demonstrated improved generalization of adversarial training by expanding the training dataset size using an additional set of curated images. Recently~\citet{min2020datahurts} argued that more training data can both help or hurt generalization based on the strength of the adversary in adversarial training. However,~\citet{min2020datahurts} works with simple problems such as Gaussian mixture classification or a two-dimensional classification. It remains unclear how adversarial training behaves with the number of samples on the scale of computer vision tasks and deep neural networks. We answer this question by training a deep neural network on an increasing number of images (ranging from $1$K to $2$M). We observe that both clean and robust test accuracy continues to improve with the number of samples. 

%% \noindent \textbf{Q.} \textit{When does adversarial robustness transfers between two data distributions?}

%% We study this problem in a generic setting where we adversarially train a classifier on one data distribution and test on another distribution. We prove that the difference in robustness of a classifier on the two distributions is \textit{tightly} upper bounded by the conditional Wasserstein distance between them. It confirms the intuition that samples from a proxy distribution that closely approximates training dataset distribution should be able to boost robustness. We also empirically validate this intuition where we show that adversarial training on samples from the proxy distribution indeed achieves non-trivial robustness with samples from the true distribution.  

%% Next, we ask when incorporating additional samples from the proxy distribution will help in improving robustness on datasets such as CIFAR-10? Here we provide a theoretical analysis on how robustness of a classifier trained on one distribution transfers to the other. In particular, we prove that the difference in robustness of a classifier on the two distributions is upper bounded by the Wasserstein distance between them. It confirms the intuition that samples from a proxy distribution that closely approximates training dataset distribution should be able to boost robustness. \vikash{Cite empirical results also where training on synthetic brings robustness on CIFAR-10 itself.}

%% Our work focuses on this generalization gap with a two-fold goal: 1) Develop a deeper understanding of generalization of robustness between distributions 2) Making further improvements in closing this generalization gap.

%% To understand the generalization of robustness we work with the following generic setting. We assume access to two data distributions. First is the \textit{source} distribution on which we train the model, and second is the \textit{target} distribution, a shifted version of the source distribution, on which we test the model. This setting also allows us to model scenarios where inference time inputs are not exactly respecting training distribution, as often is the case in real-world deployment (cite ood) or even in independent replication of classic datasets (cite).

%% We find that robustness is much harder to generalize than clean accuracy between the two distributions. We train multiple models with an increasing number of training samples from the source distribution and test on samples from the target distribution. While clean accuracy improves consistently with an increase in training samples, improvement in robust accuracy is much smaller. To further understand the relationship between robustness on these two distributions, we complement our experiments with a theoretical analysis. In particular, we prove that the difference in robustness on these two distributions is upper bounded by the Wasserstein distance between them. This result verifies the intuition that robustness achieved on one distribution can transfer to another distribution, if they are close, at test time. 

%% \noindent \textbf{Q.} \textit{How to improve state-of-the-art in adversarial training using proxy distributions?}

%% \noindent \textbf{Contributions.} We make the following key contributions.
%% \begin{itemize}
%%     \item We provide a theoretical understanding as well as an empirical validation of the transfer of adversarial robustness between data distributions. In particular, we provide a tight upper bound on the difference between the robustness of a classifier on two data distributions. 
%%     \item We propose to combine adversarial training with proxy distributions. By leveraging additional images sampled from \approxdist distributions, we improve robust accuracy by up to $6.1$\% and $5.7$\% in $l_{\infty}$ and $l_2$ threat models, respectively, and certified robust accuracy by $6.7$\% on the CIFAR-10 dataset.
%%     \item We provide the \textit{first} large scale empirical investigation of accuracy vs robustness trade-off and sample complexity of adversarial training by training deep neural networks on $2$K to $10$M images.
% \end{itemize}

%% 1) We investigate the effect of increasing number of training samples (from $1$K to $2$M) on the performance of adversarial training with deep neural networks,  2) we provide theoretical insights on how robustness of a classifier on one distribution transfer to another distribution. In particular, we provide a tight upper bound on the difference of the robustness of a classifier between the distributions, and 3) by leveraging additional images sampled from the \approxdist distributions, we improve robust accuracy up to $6.5$\% and $5.0$\% in $l_{\infty}$ and $l_2$ threat model, respectively, on the CIFAR-10 dataset.

%% In robust ML goal is to make robust. However there remain a large generalization gap between training and test data. In understand the generalization we assume this generic setting. two distributions: source distribution on which model is trained and target on which model is tested. We assume some shift between them, which can easily occur in real-world application or even in a replication effort. Two fold goal: 1) Understand the generalization of robustness between shifted distribution 2) Taking advantage of another shifted distribution when available. 

%% We find that robustness is much harder to generalize than clean accuracy. Here we training different models with increasing number of samples from source distribution and test on both source and target. While clean accuracy on target consistently improves, robust accuracy improves super slowly. This shed light on how small distribution shift can adversely effect generalization of robustness. Intriguing question is how does robustness on these two distributions relate. Here, we prove an upper bound on the robustness gap, which is only a function of distribution distance. Verifying the intuition that smaller distribution shift will lead to smaller generalization gap. 

%% Motivated by aforementioned results, we now seek to take advantage proxy distributions, i.e., distribution closely approximating original distribution, in order to close the gap between train and test set. We find that recent generative models, closely approximate source distribution on dataset such as CIFAR-10. A test we do is to robustly train on them and test on original and these model achieve a highly non-trivial performance. 

%% Here we first use training set to train the generative models, followed by sampling a specified set of synthetic images. Next we combine these synthetic images with original training test, and robustly trained a classifier. Our experimental results demonstrate that use of synthetic images improves robustness accuracy up to 6.4\% on CIFAR-10 dataset. We observe such improvements across different networks architectures and threat models. 


%% Generalization in robust machine learning is hard, between training and test set. We study it in more generic setting where we look into generalization between two slightly shifted distributions. Slight distribution shift can happen, practical or just replication efforts. |||||
%% understanding Robustness - Robustness is hard to generalize between distributions. However we prove that such difference is upper bounded by a distance. ||||| 
%% Improving robustness - On baseline dataset. Motivate this by saying that closely approximated distribution can generalize robustness to baseline distribution. We find that recent generative model achieve this and we use them. |||||
%% Discussion  - Future work should focus on bringing two distributions closer. 
%% \begin{itemize}
%%     \item Goal improve adversarial robustness. Similar to supervised, more data helps with robust learning. While exactly replicating original distribution is hard (Berkeley paper) - proper calibration, cleaning etc, an approximate distribution can be obtained. This could be an generating model approximating/\approxdist original data. Our goal is to leverage shifted/synthetic distribution to improve adversarial robustness.  
%%     \item Our first step is to understand the impact of synthetic/original distribution overlap on transfer of robustness between them. Here we prove that robustness on synthetic and original dataset is upper bounded by distribution distance. It supported the hypothesis that when synthetic distribution closely approximate the true distribution, it can help improving robustness (big leap from generalization to help)
%%     \item 
%% \end{itemize}


==> Proxy distributions [ICLR 2022]/sections/methods.tex <==
% We first provide a brief overview of adversarial training in deep neural networks. Before integrating proxy distributions in the adversarial training, we first delve deeper into the question of whether adversarial robustness will transfer from the proxy distribution to the original training data distribution. After answering it affirmatively, we integrate proxy distributions in both adversarial training and randomized smoothing, where the latter is used to achieve certified adversarial robustness.
In this section we propose to use samples from proxy distributions to improve robustness. We first provide analytical bounds on the transfer of adversarial robustness from \approxdist to \realdist distribution. Next, using robust discriminators we provide a metric based on our analytical bound, which can accurately determine the relative ranking of different proxy distributions in terms of robustness transfer. Our metric can be calculated empirically (using samples from both distributions) and does not require the knowledge of the \approxdist or \realdist distribution. Finally, we present our robust training formulation (PORT) which uses synthetic samples generated by the generative model, together with real samples.

% We refer an approximation of the \realdist distribution, learned using limited training samples from it, as proxy distribution. 

\noindent \textbf{Notation.} We represent the input space by $\mathcal{X}$ and corresponding label space as $\mathcal{Y}$. Data is sampled from a joint distribution $D$ that is supported on $\mathcal{X}\times \mathcal{Y}$. For a label $y$, we use $D\mid y$ to denote the conditional distribution of class $y$. 
% We refer to the underlying distribution of current image datasets, such as CIFAR-10, as $\dtrain$.
We denote the proxy distribution as $\dsyn$.  We denote the neural network for classification by $f: \cX \rightarrow \cZ$, parameterized by $\theta$, which maps input images to output probability vectors ($z$). We use $h$ to refer to the classification functions that output labels. For a set $\cS$ sampled from a distribution $D$, we use $\hat{\cS}$ to denote the empirical distribution with respect to set $\cS$. We use $\mathcal{S}\sim D$ to denote the sampling of a dataset from a distribution $D$. We use $(x,y)\gets D$ to denote the sampling of a single point from $D$.

% is to minimize the training loss on adversarial examples obtained with adversarial attacks, such as projected gradient descent (PGD)~\citep{madry2017towards} based attacks, under the following formulation.
% \begin{equation*}
%     %\label{eq: advtrain}
%     \underset{\theta}{min} \underset{(x,y)\sim \dtrain}{\E} L_{adv}(\theta, x, y, \Omega),~~~~~~~~L_{adv}(\theta, x, y, \Omega) = \ell(\theta, {PGD}(x, \Omega), y)
% \end{equation*}
% where $\Omega$ is the threat model which includes the magnitude of adversarial perturbations ($\epsilon$), number of attack steps, and the size of each step. 


% \begin{equation}
%     \underset{\theta}{min} \underset{(x,y)\sim \dsyn}{\E} L_{adv}(\theta, x, y, \Omega)
% \end{equation}

\subsection{Understanding transfer of adversarial robustness between data distributions} \label{sec: theory_robstness_bound}
\bluetext{
Since our goal is to use samples from proxy distribution to improve robustness on \realdist distribution, we first study the transfer of adversarial robustness between two data distributions.
}

% \begin{comment}
% As explained above, our goal is to use samples from a proxy distribution $\tilde{D}$ instead of the actual distribution $D$. We consider two distributions $D$ and $\tilde{D}$ supported on $X \times Y$ which is the space of labeled examples. We use a classifier $h: X \rightarrow Y$ to predict class label of an input sample. We first define the average robustness of a classifier on a distribution followed by the definition of conditional Wasserstein distance, a measure of the distance between two labeled distributions.
% \end{comment}

\begin{definition}[Average Robustness]
We define average robustness for a classifier $h$  on a distribution $D$ according to a distance metric $d$ as follows: $\Rob_d(h,D)=\Ex_{(x,y)\gets D}[\inf_{h(x')\neq y } d(x',x)].$
where classifier $h: \cX \rightarrow \cY$ predicts class label of an input sample
\footnote{This notion of robustness is also used in ~\citet{gilmer2018adversarial,diochnos2018adversarial} and \citet{mahloujifar2019curse}.}.\end{definition}
This definition refers to the expected distance to the closest adversarial example for each~sample. 

% \begin{comment}
% In contrast to robust accuracy, which measures whether an adversarial example exists within a given distance, we calculate the distance to the closest adversarial example. 
% Having this definition, we can now explain our goal using the following decomposition of adversarial error. Let $L$ be a learning algorithm (e.g. adversarial training). In robust learning from a proxy distribution, we are interested in bounding the average robustness of the classifier obtained by $L$, on distribution $D$, when the training set is a set $S$ of $n$ labeled examples sampled from a proxy distribution $\tilde{D}$, denoted by $\tilde{D}^n$. In particular we want to provide a lower bound on the following quantity $$\Ex_{\substack{S\gets \tilde{D}^n\\ h\gets L(S)}}[\Rob_d(h,D)].$$
% \end{comment}

\noindent \textbf{Formalizing transfer of robustness from \approxdist to \realdist  distribution.} In robust learning from a proxy distribution, we are interested in bounding the average robustness of the classifier obtained by a learning algorithm ($L$), on distribution $D$, when the training set is a set $\cS$ of $n$ labeled examples sampled from a proxy distribution $\tilde{D}$. In particular we want to provide a lower bound on the \bluetext{transferred average robustness} i.e, $\Ex_{\substack{\cS \sim \tilde{D}\\ h\gets L(S)}}[\Rob_d(h,D)].$


In order to understand this quantity better, suppose $h$ is a classifier trained on a set $\cS$ that is sampled from $\tilde{D}$, using algorithm $L$. We decompose $\Rob_d(h,D)$ to three quantities as follows:
\begin{align*}
\Rob_d(h,D) = \big(\Rob_d(h,D)-\Rob_d(h,\tilde{D})\big) + \big(\Rob_d(h,\tilde{D}) - \Rob_d(h,\hat{\cS})\big) + \Rob_d(h,\hat{\cS}).
\end{align*}
Using this decomposition, by linearity of expectation and triangle inequality we can bound transferred average robustness from below by
\begin{align*}
\small
\underbrace{\Ex_{\substack{\cS\gets \tilde{D}^n\\ h\gets L(\cS)}}[\Rob_d(h,\hat{\cS})]}_{\textbf{Empirical robustness}} \:-\:  \underbrace{\big|\Ex_{\substack{\cS\gets \tilde{D}^n\\ h\gets L(\cS)}}[\Rob_d(h,\tilde{D}) \:-\: \Rob_d(h,\hat{\cS})]\big|}_{\textbf{Generalization penalty}} \:-\: \underbrace{\big|\Ex_{\substack{S\gets \tilde{D}^n\\ h\gets L(\cS)}}[\Rob_d(h,D)-\Rob_d(h,\tilde{D})]\big|}_{\textbf{Distribution-shift penalty}}.
\end{align*}

As the above decomposition suggests, in order to bound the average robustness, we need to bound both the generalization penalty and the distribution shift penalty.
%Indeed, if $D$ and $\tilde{D}$ were identical, we would be in the standard robust learning setting and we would have to only deal with the generalization penalty. The generalization penalty has been studied before in multiple works \citep{cullina2018pac,montasser2019vc,cchmidt2018robustgeneralization}  where distribution-independent bounds on robust generalization of adversarial training on VC classes are provided. 
The generalization penalty has been rigorously studied before in multiple works \citep{cullina2018pac,montasser2019vc,schmidt2018adversarially}. Hence, we focus on bounding the distribution shift penalty. Our goal is to provide a bound on the distribution-shift penalty that is independent of the classifier in hand and is only related to the properties of the distributions. With this goal, we define a notion of distance between two distributions.

\begin{definition}[Conditional Wasserstein distance]\label{def:cwd}
For two labeled distributions $D$ and $\tilde{D}$ supported on $\cX\times \cY$, we define $\cwd$ according to a distance metric $d$ as follows:
$$\cwd_d(D,\tilde{D})=\Ex_{(\cdot,y)\gets D}\left[\inf_{J\in \mathcal{J}(D\mid y,\tilde{D}\mid y)}\Ex_{(x,x')\gets J}[d(x,x')]\right]$$
where $\mathcal{J}(D,\tilde{D})$ is the set of joint distributions whose marginals are identical to $D$ and $\tilde{D}$. 
\end{definition}
It is simply the expectation of Wasserstein distance between conditional distributions for each class. 
% It is feasible to obtain an approximate/\approxdist distribution ($\dsyn$) approximating the original data distribution ($\dtrain$). Before developing techniques to benefit from ($\dsyn$), we ask whether robustness obtained on one distribution transfers to the other? In particular, we provide an upper bound on the difference between the robustness of the two distributions. 
%Note that Wasserstein distance is indeed used as a metric to measure the quality of generative models~\citep{Heusel2017FID}. 
Now, we are ready to state our main theorem that bounds the distribution shift penalty for any learning algorithm based only on the Wasserstein distance of the two distributions.

\begin{theorem}[Bounding distribution-shift penalty] \label{th: robustbound} 
Let $D$ and $\tilde{D}$ be two labeled distributions supported on $\cX\times \cY$ with identical label distributions, i.e., $\forall y^* \in \cY, \Pr_{(x,y)\gets D}[y=y^*] =  \Pr_{(x,y)\gets \tilde{D}}[y=y^*]$. Then for any classifier $h:\cX\to \cY$
$$|\Rob_d(h,\tilde{D}) - \Rob_d(h,D)| \leq  \cwd_d(D,\tilde{D}).$$
\end{theorem}


Theorem \ref{th: robustbound} shows how one can bound the distribution-shift penalty by minimizing the conditional Wasserstein distance between the two distributions. \bluetext{We provide its proof and empirical validation in Appendix~\ref{app: theory}}. \bluetext{Even if we successfully reduce the generalization penalty, the distribution-shift penalty may remain the dominant factor in  transferred robustness.} This theorem enables us to switch our attention from robust generalization to creating %high-quality 
generative models for which the underlying distribution is close to the original distribution. \bluetext{In Appendix \ref{app: theory}, we also provide two other theorems about the tightness of Theorem \ref{th: robustbound} and the effect of combining clean and proxy data together.}
% \begin{comment}
%     Importantly, it gives a method of measuring the quality of a proxy distribution for robust training. Note that, despite the generalization penalty, the distribution-shift penalty does not decrease when more data is provided. Hypothetically, we can have many samples from the proxy distribution which reduces the effect of generalization penalty and makes the distribution-shift penalty the dominant factor in reducing robustness. Although there are interesting theoretical results showing the effect of sample complexity on the generalization penalty, these bounds do not apply to neural networks and we take an empirical approach to show that the generalization penalty indeed approaches zero when more samples from the proxy distribution is provided (See Section \ref{sec:samp_com_syn}). This shows the importance of Theorem \ref{th: robustbound} in understanding robustness we get by training on proxy distributions. In other words, this theorem enables us to switch our attention from robust generalization to creating high quality generative models for which the underlying distributions is close to the original distribution.
%     \vikash{Commenting this part for two reason 1) Pitching CWD as the to go metric hurts us, as we ourselves don't use it. 2) Latter half reads more like discussion, thus we can bring it back there}
% \end{comment}




% \noindent \textbf{Approximating training data distribution using proxy distributions.} We refer approximations of the underlying data distribution ($\dtrain$) of a given training dataset as proxy distributions ($\dsyn$).
% We requires sample efficient approximations since often only a limited amount of training samples are available. We use latest models from Generative adversarial networks (GAN)~\citep{goodfellow2014GAN} and diffusion probabilistic models~\citep{ho2020denoisingdiffusion}, as both class of networks achieve state-of-the-art performance in approximating underlying data distribution of common image datasets. 

% \subsection{Investigating adversarial training using proxy distributions} 
% \noindent \textbf{Proxy distributions.} We refer approximations of the underlying data distribution ($\dtrain$) of a given training dataset as proxy distributions ($\dsyn$). \vikash{Formalize it. Mention that we create another training set Sp from it.}

% In real world datasets underlying data distribution ($\dtrain$) is unknown, thus we can solve Equation~\ref{eq: advtrain} on a limited number of training samples available. However, access to proxy distribution allows us to sample potentially infinite amount of samples. We train a classifier only on samples from proxy distribution solving following optimization problem: $\underset{\theta}{min} \underset{(x,y)\sim \dsyn}{\E} L_{adv}(\theta, x, y, \Omega)$. We approximate it using Empirical risk minimization and vary the number of training samples from different instances of a classifier. We validate the performance of trained classifier on both samples from both proxy ($\dsyn$) and true distribution ($\dtrain$).
% \vikash{Expand this section} Include itemize list of how we evaluate each of the key adv. training properties.

\subsection{Which \approxdist distribution to choose? - Approximating \cwdfull using robust discriminators} \label{sec: theory_arc}

Our analytical results suggest that a proxy distribution that has small \cwdfull to the \realdist can improve robustness. This means that optimizing for \cwdfull in a proxy distribution (e.g., a generative model) can potentially lead to improvements in adversarial robustness. Unfortunately, it is generally a hard task to empirically calculate the \cwdfull using only samples from the distributions \citep{mahloujifar2019empirically,bhagoji2019lowerBounds}. In this section, we introduce a metric named \emph{\aurpc} as a surrogate for \cwdfull that can be calculated when we only have sample access to the data distributions. Before defining our metric, we need to define the notion of \emph{robust discrimination} between two distributions.





\begin{wrapfigure}{r}{.4\textwidth}
    \vspace{-15pt}
    \begin{minipage}{\linewidth}
        \centering\captionsetup[subfigure]{justification=centering}
        \begin{minipage}{0.48\linewidth}
            \includegraphics[width=0.98\linewidth]{images/binary_classification.pdf}
            \subcaption{\scriptsize Original samples.}
            \label{fig: explain_blowup_base}
        \end{minipage}
        \begin{minipage}{0.48\linewidth}
            \includegraphics[width=0.98\linewidth]{images/binary_classification_adv_perturbations.pdf}
            \subcaption{\scriptsize Perturbed samples.}
            \label{fig: explain_blowup_adv}
        \end{minipage}
    \end{minipage}
    \vspace{-5pt}
    \caption{\newbluetext{Why robust discrimination is effective.} (a) Without adversarial perturbations, a non-robust discriminator can perfectly distinguish both proxy distributions from the real distribution. (b) Under adversarial perturbations, classification between real and proxy-1 is much harder compared to real and proxy-2 distribution. The success of a robust discriminator is dependent on the proximity of real and proxy distributions.
    %Making discrimination dependent on the geometry of distributions by using robust discriminators. In figure~\ref{fig: explain_blowup_base}, the non-robust discriminator can perfectly distinguish both proxy distributions from the real distribution. However, the robust discrimination between proxy distribution 1 and real distribution is harder than that of proxy distribution 2, suggesting that proxy distribution 1 is closer to real data.
    }
    \label{fig: explain_blowup}
    \vspace{-20pt}
\end{wrapfigure}
\noindent \textbf{Robust discrimination.} Our metric works based on how well a discriminator can \emph{robustly} distinguish between samples from the real and proxy distributions. Compared to a typical discriminator, the robust discriminator should be accurate even when there is an adversary who can perturb the sampled instance by a perturbation of size $\epsilon$. Intuitively, if there exists a successful and robust discriminator for two distributions $D$ and $\tilde{D}$, then it means that no adversary can make instances of $D$ to look like instances of $\tilde{D}$ even by making perturbations of size $\epsilon$. This means that $D$ and $\tilde{D}$ are far away from each other (Figure~\ref{fig: explain_blowup_adv}). \bluetext{ On the other hand, if no robust discriminator exists, then it means that the adversary can ''align`` most of the mass of proxy distribution with that of real distribution by making perturbations of size at most $\epsilon$.  This notion is closely related to the optimal transport between the proxy and real distribution. In particular, the optimal adversary here corresponds to a transport $J\in \cJ(D,\tilde{D})$ that minimizes $\Pr_{(x,x')\gets J(D,\tilde{D})}[d(x,x')\leq \epsilon]$ (Compare with Definition \ref{def:cwd}).}
To be more specific, the goal of a robust discriminator $\sigma$ is to maximize its robust accuracy\footnote{All the definitions of accuracy and robust accuracy in this section are defined for true distributions. However, in the experiments we work with their empirical variant.}:
\begin{equation*}
    \Racc_\epsilon (\sigma, D, \tilde{D}) = \tfrac{1}{2} \cdot \text{\normalfont Pr}_{x \gets D} \left[\forall x' \in Ball_\epsilon(x); \sigma(x')=1\right] + \tfrac{1}{2} \cdot \text{\normalfont Pr}_{x \gets \tilde{D}} \left[\forall x' \in \newbluetext{Ball_\epsilon(x)}; \sigma(x') =0\right]. 
\end{equation*}

 We use $\Racc_\epsilon^*(D,\tilde{D})$ to denote the accuracy of best existing robust discriminator, namely, $\Racc_\epsilon^*(D,\tilde{D})=\min_\sigma \Racc_\epsilon(\sigma, D,\tilde{D})$. Note that as $\epsilon$ grows from $0$ to $\infty$, the robust accuracy of any discriminator will decrease to at most $50\%$. If two distributions $D$ and $\tilde{D}$ are close to each other, this drop in accuracy happens much faster since the adversary can make images from two distributions to look alike by adding smaller perturbations. We use this intuition and define our metric \emph{\aurpc} as follows: $$\aurpcsf(D,\tilde{D})=\int_0^\infty (\Racc^*_\epsilon(D,\tilde{D}) - \frac{1}{2}) d\epsilon.$$
 
In other words, the \emph{\aurpc} metric is equal to the area under the robust discrimination accuracy v.s. perturbation curve (See Figure \ref{fig: aurpc} for a sample of this curve.) In Section \ref{sec:AURCP_calculation}, we discuss how this metric can be calculated with only samples from the \realdist and \approxdist distributions. \bluetext{When selecting a proxy distribution, we choose the one with the smallest \emph{\aurpc} value, since it is expected to be closest to \realdist distribution. We also demonstrate that \emph{\aurpc} metric is directly related to \cwdfull.} In particular, we have the following Theorem:
\begin{theorem} \label{thm:arc}
For any two distributions $\tilde{D}$ and $D$ with equal class probabilities we have $\cwd(D,\tilde{D})\geq 4\cdot \aurpcsf(D,\tilde{D})$.  Moreover, if for all labels $y$ , $(D\mid y)$ and $(\tilde{D}\mid y)$ are two concentric uniform spheres, then we have
$\cwd(D,\tilde{D}) = 4\cdot \aurpcsf(D,\tilde{D})$.
\end{theorem}


% When we expand each sample $x$ using an $\epsilon$-ball, denoted by $Ball_x(\epsilon)$, the discrimination objective is to classify all samples in the ball correctly. For samples at close proximity, even small $\epsilon$ will lead to ball intersection, making the classification infeasible (as highlighted in Figure~\ref{fig: explain_blowup_adv}). However, due to the high-dimensional nature of images, it's not feasible to evaluate the discriminator on all samples in the balls. Instead, we use robust accuracy ($Racc$) of the discriminator as a surrogate metric. We define robust accuracy of a discriminator on a set of real ($S_D$) and synthetic images ($S_{\tilde{D}}$) as follows:

% \begin{equation*}
%     \Racc (\sigma, D, \tilde{D}) = \tfrac{1}{2} \times \text{\normalfont Pr}_{x \in S_D} \left[\max_{x_i \in Ball_x(\epsilon)} f(x_i) < 0.5\right] + \tfrac{1}{2} \times \text{\normalfont Pr}_{x \in S_{\tilde{D}}} \left[\min_{x_i \in Ball_x(\epsilon)} f(x_i) \geq 0.5\right] 
% \end{equation*}

% Robust accuracy considers the worst-case prediction over the $\epsilon$-ball which can be efficiently searched using gradient-based optimization algorithms. Note that the discriminator is also robustly trained, i.e., using worse-case prediction over balls, to maximize its robust accuracy. 

% \noindent \textbf{Blowing up distributions to make discrimination correlate with proximity.} We blowup each sample ($x$) using a $\ell_p$ balls, denoted by $Ball_x(\epsilon)$ where $\epsilon$ is the maximum perturbation budget. Now the objective become discriminating between blowed up distributions, $\mathscr{D}$ and $\mathscr{\tilde{D}}$, respectively. Discrimination between blowed up distribution is now effected by proximity, since close proximity would lead to multiple ball intersections, making the classification infeasible (Figure~\ref{fig: explain_blowup_base}). We concretely define this objective below.

% % $\frac{1}{N}\sum\limits_{i=1}^N f(x_i)$
% With blowed up distributions, we are interested into how well the discriminator classifies all points in the ball correctly. Given very high dimensional nature of most dataset, empirically estimating the prediction across all samples in the ball is not feasible. We consider the worst-case classification with in the balls, which acts as a lower bounds on the empirical mean of predicted probabilities over the ball. If this worst-case prediction is also correct, it implies that the classifier is able to successfully discriminate between blowed up distributions. These worst-case predictions can be easily found using a few gradient based optimization steps.
% % where $\overline{f(Ball_x(\epsilon))}$ is the empirical mean of output probability vectors over all all samples in the $Ball_x(\epsilon)$. 

% \noindent \textbf{Aggregating robust accuracy over different perturbations budgets ($\epsilon$) to derive a metric.} we hypothesize that with increasing perturbation budget discrimination will become harder, thus lower robust accuracy, for proxy distributions which are in close proximity of \orgdist distribution. We gradually increase the perturbation budget to blow up distribution and measure the robust accuracy ($Racc$) at each perturbation. We use the area under this robustness vs perturbation budget curve (\emph{AURPC}) as the key metric to rank different proxy distributions. Thus proxy distributions that are closer to \realdist data distribution will likely have smaller \emph{AURPC} value compared to other distributions. 

% Before delving deeper into our approach, we first discuss why we (non-robust) discriminators are not enough to measure the proximity.



% However, we specifically use $\epsilon$-expanded set of both synthetic and real data, i.e., each sample is expanded using $\ell_p$ balls of size $\epsilon$. Before delving deeper into our approach, we first discuss the need for $\epsilon$-expansion. 


% \paragraph{Calculating \aurpc.} To calculate \aurpc, We gradually increase the perturbation budget measure the robust accuracy ($\Racc$) at each perturbation for a robust discriminator that we train using adversarial training with the same perturbation budget. Then, we calculate the area under this robustness vs perturbation budget curve. 

\noindent \textbf{Why non-robust discrimination is not an effective metric.} Deep neural networks are commonly used as a discriminator between synthetic and real images~\citep{goodfellow2014GAN, gui2020ganreview}. % Due to high expressive power, deep neural network can successfully discriminate between two distributions, even on close proximity. 
In our experiments, we find that even a four-layer convolutional network can achieve near 100\% classification accuracy on all selected proxy distributions (Appendix~\ref{app: nonrobust_disc}). This result shows that non-robust discrimination is not an effective measure of proximity (as highlighted in Figure~\ref{fig: explain_blowup_base}). 
% On a theoretical of point of view, non-robust discrimination does not have meaningful connections to \cwdfull. However, it can be seen as a way to measure the \emph{Total Variations Distance} between two distributions which is independent of the geometry of the two distributions. For example, imagine two image distributions that are exactly the same except that in one of them there is a small signature in the corner of each image. The total variations distance between these two distributions is $1$ and it is easy to distinguish between them. However, robustness can provably transfer from one distribution to another as the norm of the added signatures are small. \vikash{Can we make this tight?}




% \begin{comment}
% \begin{definition}[Defining distinguishability as a function of learnability]
% Given a real distribution ($D$) and \approxdist distribution ($\tilde{D}$), we measure distinguishability as the accuracy of the binary classifier ($f$) trained to discriminate between the two distributions.

% \begin{equation*}
%     acc(f, D, \tilde{D}) = \tfrac{1}{2}\:\left(\text{\normalfont Pr}_{x \sim D} [f(x) < 0.5] + \tfrac{1}{2}\:\text{\normalfont Pr}_{x \sim \tilde{D}} [f(x) \geq 0.5]\right)
% \end{equation*}
% \end{definition}

% This approach bears resemblance to the discriminator in generative adversarial networks (cite) where the objective is to classify synthetic and real images. If a proxy distribution is hard to distinguish from real distribution, performs will likely transfer from it the the \orgdist.
% When using deep neural network as an discriminator, we find that they are highly successful in achieving near $100$\% classification accuracy for all proxy distributions, irrespective of their proximity to the \orgdist distribution. \vikash{We tried resnet18, but would a 4-layer cnn would achieve same.} This is likely because of high expressive power of deep networks, which enables then to draw complex decision boundaries (Figure~\ref{fig: explain_blowup_base}). \vikash{Mention use of validation set.}
% \end{comment}



% \paragraph{Other metrics.} A natural approach for measuring the proximity of two distributions is to use a sample-based measures of proximity, such as Euclidean distance between samples from both distributions or FID \saeed{FID is not sample based, right?}, a widely used measure of distance between synthetic and real-world images. We find that both metrics failed to adequately determine which proxy distributions lead to the highest transfer of robustness to \realdist. 
% % \begin{comment}

% \textit{Connecting back to theory.} Note that our proposed metric (AURPC) also approximate the CWD.
% \vikash{@Saeed: May be here we can connect this metric back to the theorem.}

% \vikash{While we follow use learnability, it is natural to ask why not use minimum lp distance in the pixel space (its an approximate Wasserstein distance too}.  

% \newcommand{\mix}{\mathrm{mix}}
% \newcommand{\RobDist}{\mathrm{robAcc}}
% \newcommand{\avbud}{\overline{\mathrm{budget}}}
% \begin{definition}[Robust Distinguishing Accuracy] Let $D$ and $\tilde{D}$ be two distributions and let $\mix(D,\tilde{D})\equiv\frac{1}{2}(D,0) + \frac{1}{2}(\tilde{D},1)$ be the uniform mixture of these two distributions with labels. distributions  and a distinguishing function $f$ and an attack algorithm $A:\Supp(\mix(D,\tilde{D})) \to \Supp(\mix(D,\tilde{D}))$ we define the robust distinguishing advantage of $f$ in distinguishing between $D$ and $\tilde{D}$ in presence of $f$ as follows:

% $$\RobDist(A,f,D,\tilde{D}) = \Ex_{(x,b)\gets \mix(D,\tilde{D})}\big[f(A(x))=b].$$
%  and the average budget of $A$ (according to norm $d$) is defined as 
% $$\avbud_d(A,D,\tilde{D})=\Ex_{(x,b)\gets \mix(D,\tilde{D})}[d(x,A(x))]$$
% \end{definition}

% \begin{theorem}\label{thm:metric1}
% For any two distribution $D$ and $\tilde{D}$ and any norm $d$ there exists an attack $A^*$ such that
% $$\avbud_d(A,D,\tilde{D})=\cwd(D,\tilde{D},d)$$
% and
% $$\max_f  \RobDist(A,f, D,\tilde{D}) = 0.5.$$
% \end{theorem}



% \begin{theorem}\label{thm:metric2}
% If an attack $A$ has the property that $$\max_f;  \RobDist_d(A,f, D,\tilde{D}) = 0.5.$$ then, we have

% $$\avbud(A,D,\tilde{D})\geq \cwd(D,\tilde{D})$$
% \end{theorem}

% Theorems \ref{thm:metric1} and \ref{thm:metric2} implies that $\cwd(D,\tilde{D},d)$ is solution to the following optimization problem,

% $$\min_A \avbud_d(A,D,\tilde{D}) \text{~~~s.t.~~~} \max_f \RobDist(A,f,D,\tilde{D})=0.5$$

% \end{comment}

\subsection{Bringing it all together: Improving adversarial robustness using \approxdist distributions} \label{sec: theory_sota}
\noindent \textbf{Overview of robust training.}
The key objective in robust training is to solve $\underset{\theta}{min} \underset{(x,y)\sim \dtrain}{\E} L_{adv}(\theta, x, y, \Omega)$, where $L_{adv}$ is determined by the training objective and $\Omega$ is the threat model. In adversarial training~\citep{madry2017towards, zhang2019tradeoff, carmon2019unlabeled, pang2021bagoftricks}, we train against projected gradient descent based (PGD) adversarial examples by selecting $L_{adv} (.) = \ell(\theta, {PGD}(x, \Omega), y)$.  In randomized smoothing~\citep{cohen2019certified, salman2019AdvSmooth, sehwag2020Hydra, carmon2019unlabeled}, where the objective is to achieve certified robustness~\citep{wong2018provable}, we aim to achieve invariance to random Gaussian Noise by selecting $L_{adv} (.) = \ell(\theta, x, y) + \beta D_{kl}(f_{\theta}(x), f_{\theta}(x + \delta))$, where $\delta \sim \mathrm{N}(0, \sigma^2I)$, and $D_{kl} (., .)$ is the KL-divergence. This loss function~\citep{zheng2016stabilityTrain}, referred to as robust stability training (RST), performs better than using $\ell(\theta,x+\delta,y)$~\citep{carmon2019unlabeled}. We refer the $L_{adv}$ in adversarial training and randomized smoothing as $L_{pgd}$ and $L_{smooth}$, respectively. We represent the cross-entropy loss function, which is used to train the classifier, as $\ell(.)$, where $\ell(\theta, x, y) = \langle-log(f_{\theta}(x)), \boldsymbol{y}\rangle$ and $\boldsymbol{y}$ is the one-hot vector encoding of $y$.

Our objective is to integrate synthetic samples from Proxy distributions in Robust Training (PORT). In particular, we use the following robust training formulation that combines samples from a real training dataset with synthetic samples.
% Now we focus on improving robustness on original training data distribution ($\dtrain$) using synthetic samples from proxy distributions.
%As Theorem~\ref{th: robustbound} states, robust training on a close \approxdist distribution ($\dsyn$) can generalize to the \truedist data distribution. Therefore, to improve robustness on $\dtrain$, we propose to augment original training set with samples from $\dsyn$. 
\begin{align*} 
% \label{eq: advtrainours}
    \underset{\theta}{min}\:L_{agg};\:\:\:L_{agg} = \gamma \underset{(x,y)\sim \dtrain}{\E} L_{adv}(\theta, x, y, \Omega) + (1-\gamma) \underset{(x,y)\sim \dsyn}{\E} L_{adv}(\theta, x, y, \Omega)
\end{align*}
where $\gamma\in [0,1]$ and $L_{agg}$ is the aggregated adversarial loss over both $\dtrain$ and $\dsyn$. Depending on training objective, we select either $L_{pgd}$ or $L_{smooth}$ as $L_{adv}$. 
% \begin{align*} 
% % \label{eq: advtrainours}
%     \underset{\theta}{min}~\left[\gamma * \underset{(x,y)\sim \dtrain}{\E} L_{adv}(\theta, x, y, \Omega) + (1-\gamma) * \underset{(x,y)\sim \dsyn}{\E} L_{adv}(\theta, x, y, \Omega)\right],\:\:\:
%     \text{where}\:\gamma\in [0,1]
% \end{align*}
We approximate the aggregated loss using available training samples from the \realdist distribution ($\dtrain$) and a set of synthetic images sampled from the proxy distribution ($\dsyn$). We select $\gamma$ through a hyperparameter search. 
% Since increasing the number of synthetic samples helps (Appendix~\ref{app: sample_complexity}), we use a significantly larger number of synthetic samples than available training samples from $\dtrain$.

% We approach it as an empirical risk minimization problem where we estimate the loss on original training data distribution using available samples in its training set. Similarly, we estimate loss on the proxy distribution using a set of synthetic images sampled from it. Since increasing the number of synthetic samples helps (Section~\ref{sec:samp_com_syn}), we use a significantly large number of synthetic samples than available training samples from $\dtrain$. \vikash{Improve this paragraph. Add discussion of choice of gamma and number of training images.}

\noindent \textbf{\newtext{Which synthetic samples to choose?}} In particular, which set ($S$) of $N$ synthetic samples from the proxy distribution ($\tilde{D}$) leads to maximum transferred robustness on real data, i.e., $\Ex_{\substack{f\gets \hat{L}(S)}}[\Rob_d(f,D)]$, where $\hat{L}$ is a robust learning algorithm.
% i.e., solution to following optimization problem: $\max_{\substack{S \sim \tilde{D}}} \Ex_{\substack{f\gets \hat{L}(S)}}[\Rob_d(f,D)]$\saeed{I think this optimization is not clear. What does $\max_{s\sim \tilde{D}}$ mean? I think we should write it this way: $$\max_{\cE\subseteq \cX} \Ex_{\cS\sim\tilde{D}\mid \cE, f\gets \hat{L}(\cS)}[\Rob_d(f,D)]$$ and then, we can say we replace it by $$\min_{\cE\subseteq \cX} ARC(\tilde{D}\mid \cE,D)$$}, 
While it can be solved in many different ways, we follow a rejection sampling based approach. In particular, we measure proximity of each synthetic sample to \realdist distribution and use it as a metric to accept or reject a sample. We use output probability score from our trained \newbluetext{robust} discriminators as a measure of proximity. In particular we define $\textrm{\textit{synthetic-score}}(x) = \newbluetext{\min_{x_i \in {Ball_\epsilon (x)}}\sigma(x_i)}$ as the final score for each synthetic sample, where samples with lowest score are prioritized in the selection.
% \saeed{Can we phrase this as a heuristic way to improve ARC metric? something like this: One can use any off-the-shelf generative model in the formulation above. However, as suggested in Section \ref{s}, we need the distributions $D$ and $\tilde{D}$ to be ``close''. Specifically, as discussed in Section \ref{}, we expect a strong correlation between our ARC metric and the transfer of robustness. Here, we propose an adaptive sampling technique, as a way to bring a distribution $\tilde{D}$ closer to the original distribution in terms of ARC distance. In particular, we do a rejection sampling operation where we only pick samples.... This technique changes $\tilde{D}$ to a different distribution $\tilde{D_s}$ which incures lower ARC distance from the original distribution. Hence, we expect it to show a better transfer of robustness. ...}

% \begin{comment}
%     In choosing \approxdist distribution, we use proximity of \approxdist to \orgdist as an criterion. We measured this proximity as the success of a discriminator in classifying the blowed up version of the two distributions. Now we ask which samples from the selected \approxdist distribution contribute most to the transfer of performance to \orgdist distribution. 
%     We argue that a proximity of each synthetic sample to \orgdist can be a effective measure of it. Even more, output statistics from our trained discriminators can efficiently measure this proximity. In particular we define $\textrm{\textit{synthetic-score}} = \min_{x_i \in Ball_x(\epsilon)} f(x_i)$ as the final score for each synthetic sample, where samples with lowest score are closer to \orgdist distribution. It measures the minimum output probability of any point with the ball being classified as synthetic. Unlike calculating empirical mean of output probability over the whole balls, this worst-case prediction can be efficient search using a gradient based optimization techniques. \vikash{Add details on rejection sampling using this score.}
% \end{comment}


% Next, we aim to also improve certified robustness on the training data distribution ($\dtrain$). We use randomized smoothing~\citep{cohen2019certified} to certify robustness as it provides better performance and scalability than alternative techniques~\citep{Wong2018ScalingProve, Zhang2020crownIbp}. Similar to our modification in adversarial training, we propose to train on samples from both proxy distribution ($\dsyn$) and original training data distribution ($\dtrain$).

% \begin{align*} 
%     \underset{\theta}{min} \left[\gamma* \underset{(x,y)\sim \dtrain}{\E} L_{smooth}(\theta, x, y) +  (1-\gamma)*\underset{(x,y)\sim \dsyn}{\E} L_{smooth}(\theta, x, y)\right]
% \end{align*}
% where $\gamma \in [0,1],\:\: L_{smooth}(\theta, x, y) = \ell(\theta, x, y) + \beta D_{kl}(f_{\theta}(x), f_{\theta}(x + \delta)),\:\: 
%     \delta \sim \mathrm{N}(0, \sigma^2I)$, and  $D_{kl} (., .)$ is the KL-divergence.

% We use the combination of both cross-entropy loss over unperturbed images and KL-divergence loss on images perturbed with Gaussian noise. This loss function, originally proposed for stability training~\citep{zheng2016stabilityTrain}, performs better than using $\ell(\theta,x+\delta,y)$ as $L_{smooth}$~\citep{carmon2019unlabeled}, where $\ell(.)$ is the cross-entropy loss function.

% \vikash{Use Wasserstein-2 (FID) and confidence in robust binary classification work to rank generative models. Add formualation of adversarial blowup. Not like adv. training but more like optimizing for clean accuracy when adv. balls are there around data points. }


% \begin{figure}[!htb]
%     \centering
%     \includegraphics[width=0.9\linewidth]{images/overview.png}
%     \caption{Sketch of our experimental pipeline. We train on both but test on test set from original.}
%     \label{fig:overview}
% \end{figure}


% \noindent \textbf{Choice of \approxdist distribution.} 
% We use state-of-the-art generative model, as they can approximate the \truedist distribution from a limited number of training samples, as a model of \approxdist distribution. We use \textit{classification robustness score (CRS)} as a metric to choose the generative model. Similar to classification accuracy score~\citep{ravuri2019CAS}, we train a classifier only on synthetic samples from the generative model and test performance on samples from original \truedist distribution. However, we perform robust training and use robust accuracy as the key metric. Such classification based score encapsulate both image quality and diversity of \approxdist dataset. We argue that models with higher \textit{CRS}, are likely to achieve higher improvement in robust accuracy.  



% We consider a generative model, approximating the \truedist distribution, as a model of \approxdist distribution. Since it approximate \truedist distribution, thus likely achieve small conditional Wasserestein distance, it will show some generalization of robustness to \truedist distribution (Theorem~\ref{th: robustbound}).

==> Proxy distributions [ICLR 2022]/sections/old_introduction.tex <==
Deep neural networks are powerful tools but their success depends strongly on the amount of training data~\citep{sun2017revisitData, mahajan2018BillionWSL}. 
Recent works show %have shown 
that for improving robust training against adversarial examples~\citep{biggio2013evasion, Szegedy2013IntrigueAdv, biggio2018wildPatterns}, additional training data is 
helpful~\citep{carmon2019unlabeled, schmidt2018AdvMoreData, alayrac2019unsupadv, deng2020AdvExtraOutDomain}.
However, curating more real-world data from the actual data distribution is usually 
challenging and costly~\citep{recht2019ImageNetv2}. 
To circumvent this challenge, we ask: can robust training be enhanced using a proxy distribution, i.e., an approximation of the \realdist distribution? 
In particular, can additional samples from a proxy distribution, that is perhaps cheaper to sample from, improve robustness. If so, can generative models that are trained on limited training images 
in small scale datasets~\citep{lecun2010mnist, krizhevsky2014cifar}, act as such a proxy distribution?\footnote{Proxy distributions may not necessarily be modeled by generative models. When a proxy distribution is the output of a generative model, we call it \emph{synthetic distribution} and refer to data sampled from it as \emph{synthetic data}.}

When training on synthetic samples from generative models, a natural question is whether robustness on synthetic data will also transfer to real world data. Even if it does, can we determine the features of synthetic data that enable this \emph{synthetic-to-real} robustness transfer and optimize our selection of generative models based on these features? Finally, can we also optimize the selection of individual synthetic samples to maximize the robustness transfer? \vikashnew{Rewrite it.}

\emph{Q.1} \emph{When does robustness transfer from proxy distribution to real data distribution?} This question is fundamental to develop a better understanding of whether a proxy distribution will help. \bluetext{For a classifier trained on only synthetic samples, we argue that in addition to empirical and generalization error, \emph{distribution shift} penalty also determines its robustness on the real data distribution.} We prove that this penalty is upper bounded by the \cwdfull between the \approxdist distribution and \realdist data distribution.

\emph{Q.2} \emph{\newtext{How effective are proxy distributions in boosting adversarial robustness on real-world dataset?}}
Our experimental results demonstrate that the use of samples from the Proxy distribution in Robust Training (PORT) can significantly improve robustness. We use \bluetext{state-of-the-art} \ddpm~\citep{ho2020denoisingdiffusion} model on CIFAR-10~\citep{krizhevsky2014cifar} dataset since it achieves the highest robustness transfer among seven generative models that we tested, and sample $10$M images from it based on the proposed synthetic score metric. \bluetext{Using this optimized set of images, PORT achieves up to $7.5$\% improvement in adversarial robustness over existing state-of-the-art~\citep{croce2020robustbench}.} \bluetext{We also observe that success of synthetic samples is dependent on the distribution of real data. Our analysis reveals that state-of-the-art in generative modeling on ImageNet~\citep{deng2009imagenet} dataset has not reached an inflection point where it leads to improvement in robustness.}







% \saeed{do we need both "synthetic" and "proxy"? Can we use just one of them?}?

% . We prove that difference between the average robustness of a classifier on the \approxdist and \realdist distribution is upper bounded by the \cwdfull between them. 
% It validates that intuition that \approxdist distributions that closely approximate \realdist distribution should be able to improve robustness on the latter. 
% In other words, samples from a proxy distribution that is indistinguishable from \realdist distribution\saeed{This is tricky to say. Inistinguishability has a formal meaning and it does not necessarily imply robustness. It is also clear from some of our experiments. Isn't the first sentence sufficient?} should be helpful. 
Thus robustness will transfer from proxy distributions that are in close proximity to \realdist distribution with respect to \cwdfull. 

% Next, we delve deeper into the question of which proxy distribution to choose and can our theoretical results inspire an effective selection criterion. Though CWD can't be computed exactly, since real data distribution is generally not known, it motivates the use of proxy distribution close to \realdist distribution. But how do we empirically measure proximity?

\emph{Q.2} \emph{Can we empirically predict robustness transfer from synthetic-to-real data?} Though \cwdfull can predict robustness transfer, calculating it requires knowledge of the underlying distribution of \realdist which is generally not known. Our theory motivates the design of a measure of proximity between two empirical distributions that incorporates the geometry of the distributions and can empirically predict transfer of robustness.
% But how do we empirically measure the proximity of synthetic and real samples?
We first test existing distance metrics: Euclidean distance between synthetic samples and nearest real samples as well as the widely used Fréchet Inception Distance (FID)~\citep{Heusel2017FID}.
% We first test existing distance metrics. A simple baseline is to use Euclidean distance of synthetic samples to nearest real samples. Another widely used distance metric is Fréchet Inception Distance (FID)~\citep{Heusel2017FID}
%\footnote{ In general, calculating FID is as hard as calculating \cwdfull. However prior work measure the FID of two distributions in \emph{feature space} by first fitting a Gaussian distribution and then calculating the distance between Gaussians. This is what we refer to as FID.}. 
In our analysis with \textit{seven} different generative models, we find that both metrics predict robustness transfer incorrectly for more than half of the models.
%As euclidean distance is neither necessary nor sufficient to capture semantic differences~\citep{sharif2018lpNormsNotSuitable}, it fails to predict the transfer of performance from synthetic-to-real data. \saeed{we can stop this para here. It will not be clear to a general audience what the next few sentences mean.} 
%A widely used metric is Fréchet Inception Distance (FID), which measures Fréchet distance between synthetic and real data in the feature space of an Inception v3 network trained on the ImageNet dataset. Apparently, FID performs even \emph{worse} than nearest neighbour distance. 

We propose a robust learning based approach where we use the success of a discriminator in distinguishing adversarially perturbed samples of synthetic and real data as a measure of proximity. Discriminating between synthetic and real data is a common practice~\citep{goodfellow2014GAN, gui2020ganreview}. 
\bluetext{However, we find that considering adversarial perturbations on synthetic and real data samples is the key to making the discriminator an effective measure for this task.}
%However, we find that its the robust learning against adversarial perturbations that makes the discriminator success an effective measure for this task. 
We demonstrate that the rate of decrease in discriminator success with an increasing size of perturbations can effectively measure proximity and it accurately predicts the relative transfer of robustness from different generative models. 

% $\epsilon$-expanded sets of synthetic and real data as a measure of proximity. We expand these sets, as without them even a four-layer convolutional network achieves near-perfect classification accuracy on all seven proxy distributions we considered. For samples at close proximity, even small values of $\epsilon$ will lead to ball intersection, making the classification infeasible. We demonstrate that the rate of decrease in discriminator success with an increasing value of $\epsilon$ can effectively measure proximity where it accurately predicts the relative transfer of robustness from different generative models. 


% We take a learning-based approach where we use success of disc how well a deep neural network can distinguish these two sets of samples. It turns out that deep networks almost perfectly distinguish all proxy distributions from real data, irrespective of their proximity, in our experiments. To make discrimination success dependent on proximity, we expand our samples by adding perturbations bounded by a $\ell_{p}$ ball. Now the objective is to correctly classify all samples within the $\ell_p$ ball. Thus proxy distributions at close proximity will have an intersection with \realdist data distribution even under a small perturbation budget. We use the discriminator success at increasing perturbation budgets and demonstrate that it accurately predicts synthetic-to-real performance transfer. \vikash{Add a link to theory.}

% \saeed{Can we optimize the proxy distribution base on our metric?}
\emph{Q.3} \emph{Can we optimize on which synthetic samples to choose?} We find that some samples lead to higher robustness transfer than others from a proxy distribution. Understanding this sample-wise importance can enable us to adaptively sample the most helpful data points. We use the proximity of each synthetic sample to \realdist distribution, referred to as \textit{synthetic score}, as a metric to judge their importance. This score can be computed using output probability from a discriminator that is robustly trained to distinguish between adversarially perturbed samples from \approxdist and \realdist distribution. We use rejection sampling based on this score where we discard samples with a score higher than a predetermined threshold. 

% A lower synthetic score implies a small distance to \realdist data distribution. As we experimentally demonstrate, samples with the lowest synthetic score contribute most to synthetic-to-real performance transfer. Using synthetic score as a criterion, we adaptively sample a large set of synthetic samples and demonstrate that it improves performance over real data compared to a randomly sampled set of synthetic images. 

% \saeed{Alternative question: Can we use enumerate environment instead of saying Q1, Q2...} \saeed{ our optimized sample generation improves ...} 
\emph{Q.4} \emph{Finally, how effective are proxy distributions in boosting adversarial robustness?}
Our experimental results demonstrate that the use of samples from the Proxy distribution in Robust Training (PORT) can significantly improve robustness. We use \bluetext{state-of-the-art} \ddpm~\citep{ho2020denoisingdiffusion} model on CIFAR-10~\citep{krizhevsky2014cifar} dataset since it achieves the highest robustness transfer among seven generative models that we tested, and sample $10$M images from it based on the proposed synthetic score metric. \bluetext{Using this optimized set of images, PORT achieves up to $7.5$\% improvement in adversarial robustness over existing state-of-the-art~\citep{croce2020robustbench}.} \bluetext{We also observe that success of synthetic samples is dependent on the distribution of real data. Our analysis reveals that state-of-the-art in generative modeling on ImageNet~\citep{deng2009imagenet} dataset has not reached an inflection point where it leads to improvement in robustness.}


% While for the MNIST~\citep{lecun2010mnist} dataset samples from an \bluetext{elementary} deep convolutional GAN~\citep{radford2015dcgan} suffice, even state-of-the-art models, including \ddpm, fail to bring any improvement on the ImageNet dataset. {\color{red} Update this.}

% Using these samples, we improve robust accuracy by up to $7.5$\% and $6.7$\% in $l_{\infty}$ and $l_2$ threat models, respectively, over baselines not using proxy distributions on the CIFAR-10 dataset. 
%In the category of not using any extra real-world data, our models achieve the first rank on RobustBench~\citep{croce2020robustbench} \saeed{I think this violates the anonymity. Let's remove it.}, a standardized benchmark for adversarial training. 
% We also improve the certified robust accuracy~\citep{cohen2019certified} by up to $7.6$\% with randomized smoothing on the CIFAR-10 dataset. \vikash{Add MNIST, ImageNet results when they are available.} \vikash{Does using roubustbench info violates double blind submission policies?}

% \saeed{I feel like the contributions below are a bit redundant. Can we merge them with paragraphs above? another idea is to move it to conclusion section.}
\noindent \textbf{Contributions.}
We make the following key contributions.
\begin{itemize}[noitemsep, topsep=0pt]
    \item We provide an analytical bound on the transfer of robustness from proxy distributions to \realdist distribution and further validate it experimentally.
    \item In selecting proxy distribution, we show that existing metrics, such as FID, fail to determine the synthetic-to-real transfer of robustness. We propose a new metric (\emph{\aurpc}) based on the distinguishability of adversarially perturbed synthetic and real data, that accurately determines the performance transfer.  
    \item We also develop a metric, named \emph{synthetic score}, to determine the importance of each synthetic sample in synthetic-to-real robustness transfer. We demonstrate that choosing samples with lower synthetic scores provide better results than randomly selected samples. 
    \item Overall, using additional synthetic images sampled from \approxdist distributions, we improve robust accuracy by up to $7.5$\% and $6.7$\% in $\ell_{\infty}$ and $\ell_2$ threat models, respectively, and certified robust accuracy ($\ell_2$) by $7.6$\% on the CIFAR-10 dataset. \bluetext{We also improve clean accuracy, simultaneously.}
\end{itemize}

%  given high expressive power of deep network, 
%Given dataset bias, ImageNet trained network may not best capture semantics of CIFAR-10 classes, so we also measure FID in the feature space of a 
% which measure proximity of synthetic samples to real data,
% In our analytical results, we use \cwdfull between synthetic and \realdist distribution to determine this. 
% However underlying distribution of \realdist is unknown, making it infeasible to calculate this bound. 


% To achieve robustness against adversarial examples, adversarial training remains the most effective technique~\citep{madry2017towards, zhang2019tradeoff, pang2021bagoftricks}. However, it is largely used with limited training samples available in current image datasets (such as only 50,000 training images in the CIFAR-10 dataset) where it suffers from multiple challenges, such as poor generalization on the test set~\citep{madry2017towards} and accuracy vs robustness trade-off~\citep{Raghunathan2020advtradeoff}. Recent works have demonstrated that more training data can improve the performance of adversarial training~\citep{schmidt2018AdvMoreData, alayrac2019unsupadv, deng2020AdvExtraOutDomain}. However, this approach runs into the challenge of curating a large set of real-world images for training. We circumvent this challenge using proxy distributions, distributions that closely approximate the underlying distribution of the original training dataset. Note that the proxy distributions are modeled using only available training images in current datasets. Proxy distributions when modeled with deep neural networks, such as Generative adversarial networks (GAN), allow us to generate a potentially unlimited number of high-fidelity images~\citep{goodfellow2014GAN, gui2020ganreview, ho2020denoisingdiffusion}. Our key goal is to improve the adversarial robustness of deep neural networks by taking advantage of samples from such proxy distributions.

% Note that proxy distributions are only an approximation of the underlying distribution of the training data. This begs the question of whether robustness achieved on samples from the proxy distribution will transfer to the original dataset. A more generic version of this question is \textit{how much the robustness of a classifier transfers between data distributions?} We prove that the difference in the robustness of a classifier on two distributions is \textit{tightly} upper bounded by the conditional Wasserstein distance between them. We refer to Wasserstein distance conditioned on class labels as conditional Wasserstein distance. This result confirms the intuition that samples from a proxy distribution that closely approximates training data distribution should be able to improve robustness on the latter. We also empirically validate this claim where we show that adversarial training only on samples from the proxy distribution indeed achieves non-trivial robustness on samples from the original distribution. 

% To improve adversarial robustness on current datasets, we aim to leverage samples from a \approxdist distribution which \textit{closely} approximates the underlying distribution of these datasets. Here we propose to simultaneously train on both the original training set and a set of additional images sampled from the \approxdist distribution. We use state-of-the-art generative models as a model for proxy distribution since they can closely approximate the data distribution from only a limited number of training samples~\citep{karras2020styleganAda, ho2020denoisingdiffusion, gui2020ganreview}.  Our experimental results demonstrate that the use of samples from the proxy distribution improves robust accuracy by up to $6.1$\% and $5.7$\% in $l_{\infty}$ and $l_2$ threat models, respectively, over baselines not using proxy distributions on the CIFAR-10 dataset. In the category of not using any extra real-world data, our models achieve the first rank on RobustBench~\citep{croce2020robustbench}, a standardized benchmark for adversarial training. We also improve the certified robust accuracy~\citep{cohen2019certified} by up to $6.7$\% with randomized smoothing on the CIFAR-10 dataset. Intriguingly, we achieve better certified robust accuracy with proxy distribution samples than using an additional set of $500$K curated real-world images~\citep{carmon2019unlabeled}.

% Since access to proxy distributions gives us the ability to generate a large number of images, this allows us to delve deeper into the relationship of adversarial robustness with the number of training samples on the scale of image classification with deep neural networks. Next, we work solely with a proxy distribution, where we train multiple networks with an increasing amount of training images (we use $2$K-$10$M training images) and test each on another fixed set of images from it. Our goal is to analyze multiple intriguing properties of the adversarial training w.r.t. the number of training samples. We first analyze the sample complexity of adversarial training. Earlier works \citep{wei2019allLayerMargin, bhagoji2019lowerBounds, schmidt2018AdvMoreData} have derived sample complexity bounds in simplified settings such as classifying a mixture of Gaussian distributions. On the scale of deep neural networks for image classification, we empirically demonstrate that more data continues to improve adversarial robustness. 
% %%Recently, \citep{chen2020dataHurtsAdv} and \citep{min2020datahurts} provided theoretical results suggesting more data may hurt generalization in adversarial training. We observe that both clean and robust generalization continue to improve with the number of training samples. 
% Next, we analyze the accuracy vs robustness trade-off: earlier works showed that robustness in adversarial training is achieved at a cost of clean accuracy of deep neural networks~\citep{Raghunathan2020advtradeoff, javanmard2020preciseTradeoff}. We demonstrate that increase in the number of training samples significantly reduces this trade-off for deep neural networks. To the best of our knowledge, this is the \textit{first} empirical investigation into adversarial training of deep neural networks on millions of images on the scale of CIFAR-10 dataset. \vikash{Add a summary of key results in a table.}

%% However, without access to the training data distribution, we are bounded by the limited training images available in these datasets. We aim to circumvent this issue using proxy distributions. We refer to approximations of the underlying distribution of these datasets as proxy distributions. Since we have access to this distribution, we can now sample a potentially unlimited number of samples from it, overcoming the challenges of limited training samples in current datasets\Snote{why do we have unlimited access to proxy distributions? would be good to elaborate on this.}.} 

%% \Snote{We can make a better connection to next sentense here. For example, saying generalization requires more data->we don't have more data -> we have proxy data} In this work, we analyze adversarial training through the lens of \textit{proxy} distributions. 
% We refer to approximations of the underlying distribution of these curated datasets as proxy distributions. In contrast to the limited number of training samples in the current dataset, we can now sample a potentially unlimited number of images from the proxy distribution. Our key goals are following. 

%% \bluetext{Our key goal is to improve the performance of adversarial training using samples from the proxy distribution. Though this integration looks straightforward, it poses multiple intriguing questions. Since the key advantage of a proxy distribution is to allow sampling of unlimited data points, the first question is how much does increase the number of training samples help in adversarial training on deep neural networks? Note that our goal is to improve robustness on the underlying data distribution of the training dataset. Proxy distributions remain an approximation of the underlying data distribution. So even if more training images improve robustness significantly, would it help if they are sampled from a proxy distribution? Finally, if we have a proxy distribution which closely approximates training data distribution, how can we use it to improve the performance of adversarial training. We delve deeper into each question individually below.}

%% Our next key objective is to utilize synthetic samples, i.e., samples from the proxy distribution, to improve robustness on current image datasets. However, proxy distribution is only an approximation of the true distribution of image datasets. Thus, it's unclear whether robustness acquired for proxy distribution will transfer to samples from the true data distribution. This motivates us to pursue the following goal. 

%% However, adversarially trained networks, when trained on a limited number of images available in curated datasets such as CIFAR-10~\citep{krizhevsky2009learning}, suffers from a large generalization gap in robust accuracy. In this work, we approach adversarial training on these datasets in conjunction with a \textit{proxy} distribution. We refer to approximations of the underlying distribution of these curated datasets as proxy distributions. Our use of proxy distributions allows us to target the following two objectives. 1) Since we can sample an unlimited number of samples from the proxy distribution, it allows us to investigate the effect of the number of training samples on the robust generalization of adversarial training 2) Using samples from proxy distribution to reduce the robust generalization gap in adversarial training.

%% \Snote{Alternative Questions for 1. Question 1: Can we achieve robustness on proxy distributions by performing adversarial training on large datasets sampled from them? }
%% \noindent \textbf{Q.} \textit{How does increasing number of training samples benefit adversarial training in \Snote{Maybe we can say "image classification" instead of "deep neural networks"} deep neural networks?}
%% % \noindent \textbf{Goal-1.} \textit{An empirical investigation into intriguing properties of adversarial training in the limit of infinite training samples.}
%% \bluetext{\Snote{Maybe we can say: our first step in investigating our main goal is to explore the case where proxy distribution is exactly the same as data distribution. }We aim to answer this question by analyzing intriguing properties of adversarial training on networks training on increasing number of training samples (we use 5k-10M training samples)}. We first analyze the sample complexity of adversarial training. Earlier works \citep{wei2019allLayerMargin, bhagoji2019lowerBounds, schmidt2018AdvMoreData} have derived sample complexity bounds in simplified settings such as classifying a mixture of Gaussian. We empirically demonstrate that more data continues to improve adversarial robustness but at a slower rate than clean accuracy. Recently, \citep{chen2020dataHurtsAdv, min2020datahurts} provide theoretical results suggesting more data may hurt generalization in adversarial training. We observe that both clean and robust generalization continues to improve with the number of training samples. Finally, we analyze the accuracy vs robustness trade-off where earlier works showed that robustness in adversarial training is achieved at a cost of clean accuracy of deep neural networks~\citep{Raghunathan2020advtradeoff, javanmard2020preciseTradeoff}. \textcolor{red}{rephrase: We demonstrate that increase in training samples can mitigate this trade-off for deep neural networks. }

%% We first investigate the effect of the number of training samples in adversarial training. Earlier works~\citep{carmon2019unlabeled, alayrac2019unsupadv} demonstrated improved generalization of adversarial training by expanding the training dataset size using an additional set of curated images. Recently~\citet{min2020datahurts} argued that more training data can both help or hurt generalization based on the strength of the adversary in adversarial training. However,~\citet{min2020datahurts} works with simple problems such as Gaussian mixture classification or a two-dimensional classification. It remains unclear how adversarial training behaves with the number of samples on the scale of computer vision tasks and deep neural networks. We answer this question by training a deep neural network on an increasing number of images (ranging from $1$K to $2$M). We observe that both clean and robust test accuracy continues to improve with the number of samples. 

%% \noindent \textbf{Q.} \textit{When does adversarial robustness transfers between two data distributions?}

%% We study this problem in a generic setting where we adversarially train a classifier on one data distribution and test on another distribution. We prove that the difference in robustness of a classifier on the two distributions is \textit{tightly} upper bounded by the conditional Wasserstein distance between them. It confirms the intuition that samples from a proxy distribution that closely approximates training dataset distribution should be able to boost robustness. We also empirically validate this intuition where we show that adversarial training on samples from the proxy distribution indeed achieves non-trivial robustness with samples from the true distribution.  

%% Next, we ask when incorporating additional samples from the proxy distribution will help in improving robustness on datasets such as CIFAR-10? Here we provide a theoretical analysis on how robustness of a classifier trained on one distribution transfers to the other. In particular, we prove that the difference in robustness of a classifier on the two distributions is upper bounded by the Wasserstein distance between them. It confirms the intuition that samples from a proxy distribution that closely approximates training dataset distribution should be able to boost robustness. \vikash{Cite empirical results also where training on synthetic brings robustness on CIFAR-10 itself.}

%% Our work focuses on this generalization gap with a two-fold goal: 1) Develop a deeper understanding of generalization of robustness between distributions 2) Making further improvements in closing this generalization gap.

%% To understand the generalization of robustness we work with the following generic setting. We assume access to two data distributions. First is the \textit{source} distribution on which we train the model, and second is the \textit{target} distribution, a shifted version of the source distribution, on which we test the model. This setting also allows us to model scenarios where inference time inputs are not exactly respecting training distribution, as often is the case in real-world deployment (cite ood) or even in independent replication of classic datasets (cite).

%% We find that robustness is much harder to generalize than clean accuracy between the two distributions. We train multiple models with an increasing number of training samples from the source distribution and test on samples from the target distribution. While clean accuracy improves consistently with an increase in training samples, improvement in robust accuracy is much smaller. To further understand the relationship between robustness on these two distributions, we complement our experiments with a theoretical analysis. In particular, we prove that the difference in robustness on these two distributions is upper bounded by the Wasserstein distance between them. This result verifies the intuition that robustness achieved on one distribution can transfer to another distribution, if they are close, at test time. 

%% \noindent \textbf{Q.} \textit{How to improve state-of-the-art in adversarial training using proxy distributions?}

%% \noindent \textbf{Contributions.} We make the following key contributions.
%% \begin{itemize}
%%     \item We provide a theoretical understanding as well as an empirical validation of the transfer of adversarial robustness between data distributions. In particular, we provide a tight upper bound on the difference between the robustness of a classifier on two data distributions. 
%%     \item We propose to combine adversarial training with proxy distributions. By leveraging additional images sampled from \approxdist distributions, we improve robust accuracy by up to $6.1$\% and $5.7$\% in $l_{\infty}$ and $l_2$ threat models, respectively, and certified robust accuracy by $6.7$\% on the CIFAR-10 dataset.
%%     \item We provide the \textit{first} large scale empirical investigation of accuracy vs robustness trade-off and sample complexity of adversarial training by training deep neural networks on $2$K to $10$M images.
% \end{itemize}

%% 1) We investigate the effect of increasing number of training samples (from $1$K to $2$M) on the performance of adversarial training with deep neural networks,  2) we provide theoretical insights on how robustness of a classifier on one distribution transfer to another distribution. In particular, we provide a tight upper bound on the difference of the robustness of a classifier between the distributions, and 3) by leveraging additional images sampled from the \approxdist distributions, we improve robust accuracy up to $6.5$\% and $5.0$\% in $l_{\infty}$ and $l_2$ threat model, respectively, on the CIFAR-10 dataset.

%% In robust ML goal is to make robust. However there remain a large generalization gap between training and test data. In understand the generalization we assume this generic setting. two distributions: source distribution on which model is trained and target on which model is tested. We assume some shift between them, which can easily occur in real-world application or even in a replication effort. Two fold goal: 1) Understand the generalization of robustness between shifted distribution 2) Taking advantage of another shifted distribution when available. 

%% We find that robustness is much harder to generalize than clean accuracy. Here we training different models with increasing number of samples from source distribution and test on both source and target. While clean accuracy on target consistently improves, robust accuracy improves super slowly. This shed light on how small distribution shift can adversely effect generalization of robustness. Intriguing question is how does robustness on these two distributions relate. Here, we prove an upper bound on the robustness gap, which is only a function of distribution distance. Verifying the intuition that smaller distribution shift will lead to smaller generalization gap. 

%% Motivated by aforementioned results, we now seek to take advantage proxy distributions, i.e., distribution closely approximating original distribution, in order to close the gap between train and test set. We find that recent generative models, closely approximate source distribution on dataset such as CIFAR-10. A test we do is to robustly train on them and test on original and these model achieve a highly non-trivial performance. 

%% Here we first use training set to train the generative models, followed by sampling a specified set of synthetic images. Next we combine these synthetic images with original training test, and robustly trained a classifier. Our experimental results demonstrate that use of synthetic images improves robustness accuracy up to 6.4\% on CIFAR-10 dataset. We observe such improvements across different networks architectures and threat models. 


%% Generalization in robust machine learning is hard, between training and test set. We study it in more generic setting where we look into generalization between two slightly shifted distributions. Slight distribution shift can happen, practical or just replication efforts. |||||
%% understanding Robustness - Robustness is hard to generalize between distributions. However we prove that such difference is upper bounded by a distance. ||||| 
%% Improving robustness - On baseline dataset. Motivate this by saying that closely approximated distribution can generalize robustness to baseline distribution. We find that recent generative model achieve this and we use them. |||||
%% Discussion  - Future work should focus on bringing two distributions closer. 
%% \begin{itemize}
%%     \item Goal improve adversarial robustness. Similar to supervised, more data helps with robust learning. While exactly replicating original distribution is hard (Berkeley paper) - proper calibration, cleaning etc, an approximate distribution can be obtained. This could be an generating model approximating/\approxdist original data. Our goal is to leverage shifted/synthetic distribution to improve adversarial robustness.  
%%     \item Our first step is to understand the impact of synthetic/original distribution overlap on transfer of robustness between them. Here we prove that robustness on synthetic and original dataset is upper bounded by distribution distance. It supported the hypothesis that when synthetic distribution closely approximate the true distribution, it can help improving robustness (big leap from generalization to help)
%%     \item 
%% \end{itemize}


==> Proxy distributions [ICLR 2022]/sections/proof_ARC_CWD.tex <==

\subsection{Proof of Theorem 2}
\paragraph{Theorem 2.}
\textit{
For any two distributions $\tilde{D}$ and $D$ with equal class probabilities we have $\cwd(D,\tilde{D})\geq 4\aurpcsf(D,\tilde{D})$.  Moreover, if for all labels $y$ , $(D\mid y)$ and $(\tilde{D}\mid y)$ are two concentric uniform $l_p$ spheres, then we have
$\cwd(D,\tilde{D}) = 4\aurpcsf(D,\tilde{D})$.\footnote{The statement of theorem in the main body has a typographical error that is fixed here.}
}
\begin{proof}
We start by proving a lemma.
\begin{lemma}\label{lem:totalvar}
Let $J \in \cJ(D,\tilde{D})$ be an arbitrary transport between $D$ and $\tilde{D}$. Then, for any discriminator $\sigma$ we have,
$$\Racc_{\epsilon/2}(\sigma,D,\tilde{D}) \leq \frac{1}{2} +\frac{\Pr_{(x,x')\gets J}\big[d(x,x')> \epsilon\big]}{2}.$$
\end{lemma}
\begin{proof}
Consider an adversary $A^\epsilon_J$ that on input $x$ sampled from $D$, samples a pair $(x,x')\gets J \mid J[1] = x$ from the transport and return a center point $x''$ between $x$ and $x'$ such that $d(x,x'')=d(x',x'') = d(x,x')/2$ if $d(x,x')\leq \epsilon$. Otherwise, it returns $x$. Also, on a in input $x'$ sampled from $\tilde{D}$ it samples a pair $(x,x')\gets J \mid J[2] = x'$ from the transport and return a center point $x''$ between $x$ and $x'$ such that $d(x,x'')=d(x',x'') = d(x,x')/2$ if $d(x,x')\leq \epsilon$. Otherwise, it returns $x'$.

Denote $D_A\equiv A^\epsilon_J\#D$ to be the push-forward of $D$ under $A_J$. And also denote $\tilde{D}_A\equiv A^\epsilon_J\#\tilde{D}$. Now we have, $\delta(D_A,\tilde{D}_A) \leq \Pr_{(x,x')\gets J}[d(x,x')>\epsilon]$ where $\delta$ is the total variational distance. Therefore, no discriminator $\sigma$ can distinguish $D'$ from $\tilde{D}$ with accuracy more than $\frac{1 +\Pr_{(x,x')\gets J}[d(x,x')>\epsilon]}{2}$.
\end{proof}
Now, let $J^* = \sum_{y=1}^l \alpha_y J^*_y$ be a transport between $D$ and $\tilde{D}$ where $J^*_y$ is the optimal transport between $\tilde{D}\mid y$ and $D \mid y$ and $\alpha_y$ is the probability of class $y$ for $D$ and $\tilde{D}$. using Lemma \ref{lem:totalvar} we have
$$\Racc^*_\epsilon(D,\tilde{D}) -\frac{1}{2}\leq \frac{\Pr_{(x,x')\gets J^*}[d(x,x')>2\epsilon]}{2}.$$
Therefore we have

\begin{equation}\label{eq0000}
\int_0^\infty [\Racc^*_\epsilon(D,\tilde{D}) -\frac{1}{2}] d\epsilon \leq \int_0^\infty \frac{\Pr_{(x,x')\gets J^*}[d(x,x')>2\epsilon]}{2} d\epsilon =\int_0^\infty \frac{\Pr_{(x,x')\gets J^*}[d(x,x')>\epsilon]}{4} d\epsilon .
\end{equation}
% Now, by integral by parts we have  we have
% $$\int_0^\infty \frac{\Pr_{(x,x')\gets J}[d(x,x')>\epsilon]}{2} d\epsilon=\int_0^\infty \frac{1-\Pr_{(x,x')\gets J}[d(x,x')\leq \epsilon]}{2}$$
Now, by integration by parts we have 
\begin{align*}\int_0^\infty \Pr_{(x,x')\gets J^*}[d(x,x')> \epsilon] d\epsilon  &= \epsilon \Pr_{(x,x')\gets J^*}[d(x,x')> \epsilon]\Big|_0^\infty + \int_0^\infty \Pr_{(x,x')\gets J^*}[d(x,x')=\epsilon]\epsilon   d\epsilon\\
&=0 + \Ex_{(x,x')\gets J^*}[d(x,x')]\\
&=\cwd(D,\tilde{D}).
\end{align*}
Therefore, we have
$$\aurpcsf(D,\tilde{D}) = \int_0^\infty [\Racc^*_\epsilon(D,\tilde{D}) -\frac{1}{2}] d\epsilon \leq \frac{\cwd(D,\tilde{D})}{4}.$$
Now to prove the second part of theorem about the case of concentric spheres we start by following lemma. 
\begin{lemma}\label{lem:totalvarasphere}
Let $D_y=D\mid y$ and $\tilde{D}_y=\tilde{D}\mid y$. Assume $\tilde{D}_y$ and $D_y$ are two concentric spheres according to the some $l_p$ norm. Also let $J^* \in \cJ(D_y,\tilde{D}_y)$ be the optimal transport between $D_y$ and $\tilde{D}_y$ with respect to the same norm.  Then we have,
$$\Racc^*_{\epsilon/2}(D,\tilde{D}) = \frac{1}{2} +\frac{\Pr_{(x,x')\gets J^*}\big[d(x,x')> \epsilon\big]}{2}.$$
\end{lemma}
\begin{proof}
let $D$ be the uniform sphere centered at point $c$ and with radius $r$ and let $\tilde{D}$ be the uniform sphere centered at point $c$ and with radios $\tilde{r}>r$. Observe that the optimal robust distinguisher for any $\epsilon<\frac{r+\tilde{r}}{2}$ is the one that assigns $0$ to $x$ if $d(c,x)<\frac{\tilde{r}-r}{2}$ and assigns $1$ otherwise and for any $\epsilon< \frac{\tilde{r}-r}{2}$ we have
\begin{equation}\label{eq:0001}
    \Racc^*_{\epsilon/2}(D,\tilde{D})=1.
\end{equation}
On the other hand, for any $\epsilon\geq \frac{\tilde{r}-r}{2}$ we have 
\begin{equation}\label{eq:0002}
    \Racc^*_{\epsilon/2}(D,\tilde{D})=0.5.
\end{equation}


Now consider optimal transport $J^*$ between $D$ and $\tilde{D}$. Observe that this transport is equivalent to the following distribution: $$J^*\equiv (D, (D-c)\cdot \tilde{r}/r)$$
Therefore,  we have 
$\Pr_{(x,x')\gets J^*}[d(x,x')=\tilde{r}-r]=1$ 
Which implies for any $\epsilon<\tilde{r}-r$ we have
\begin{equation}\label{eq:0003}
\Pr_{(x,x')\gets J^*}[d(x,x')> \epsilon]=1
\end{equation}
and for any $\epsilon\geq\tilde{r}-r$
\begin{equation}\label{eq:0004}
\Pr_{(x,x')\gets J^*}[d(x,x')> \epsilon]=0.
\end{equation}
Putting Equations \eqref{eq:0001}, \eqref{eq:0002}, \eqref{eq:0003}, and \eqref{eq:0004} together, we finish the proof of Lemma. 
\end{proof}
Having Lemma \ref{lem:totalvarasphere}, we can follow the same steps as before except that instead of Inequality \eqref{eq0000} we have an equality of the following form.

\begin{align*}\label{eq0000eq}
\int_0^\infty [\Racc^*_\epsilon(D,\tilde{D}) -\frac{1}{2}] d\epsilon &= \int_0^\infty \frac{\Pr_{(x,x')\gets J^*}[d(x,x')>2\epsilon]}{2} d\epsilon\\ &=\int_0^\infty \frac{\Pr_{(x,x')\gets J^*}[d(x,x')>\epsilon]}{4} d\epsilon\\
&=\frac{\cwd(D,\tilde{D})}{4}.
\end{align*}
\end{proof}

==> sections/background.tex <==
% Adversarial training~\citep{Goodfellow2014ExplainAdv, madry2017towards, zhang2019tradeoff, gowal2020uncoveringadv, wu2020adversarial} remains the most effective defense against adversarial examples~\citep{szegedy2013intriguing}. 
% % Subsequent works further improve its performance using larger architectures~\citep{gowal2020uncoveringadv}, early stopping~\citep{rice2020overfitadv}, smooth activations~\citep{xie2020smooth}, weight perturbations~\citep{wu2020adversarial}.
% However, earlier works have also shown that adversarial training suffers from a large robust generalization gap~\citep{cchmidt2018robustgeneralization, raghunathan2019adversarialgen}. We refer the reader to RobustBench~\citep{croce2020robustbench} for comparison and overview of state-of-the-art methods. 

% In our work, we also find that state-of-the-art diffusion process-based models provide much higher gain than state-of-the-art GAN. 

% Recent works have also explored the use of synthetic samples in training deep neural networks~\citep{ravuri2019CAS, shmelkov2018good}. While these earlier works focus on benign training our focus is on adversarial training. Another concurrent work~\citep{rebuffi2021fixingaugmentation} also uses samples from generative models to improve adversarial robustness. While ~\citet{rebuffi2021fixingaugmentation} broadly focuses on the effect of data augmentation, our goal is to understand the effect of different proxy distributions. However, similar benefits of using the generative model from two independent works further ascertain the importance of this direction. 


\subsection{Robust Machine learning}

\noindent \textbf{Adversarial examples.} Adversarial examples, crafted using an adversarial attack, aim to evade the classifier at the test time~\citep{biggio2013evasion, Szegedy2013IntrigueAdv, biggio2018wildPatterns}. While we focus on $\ell_p$ perturbation based adversarial examples~\citep{Goodfellow2014ExplainAdv}, there exist multiple other threat models~\citep{wong2019wassersteinAdv, sehwag2019analyzing, hosseini2018semanticAdv, Laidlaw2019functionalAdv, kang2019unforseenAdv}. Adversarial examples have been successful against almost all applications of machine learning~\citep{xu2020AdvImageGraphText, xu2016autoEvadePdfAdv, rahman2019mockingbird}. 

\noindent \textbf{On use of $l_p$ threat model.} We consider $\ell_p$ perturbation based adversarial examples since it's the most widely studied threat model~\citep{croce2020robustbench}. Additionally, robustness achieved in this threat model has also led to further benefits in  explainability~\citep{chalasani2020advExplain}, image recognition~\citep{xie2020advImproveCV, salman2020Unadversarial}, transfer learning~\citep{Salman2020AdvTransfer, utrera2021AdvTransfer}, self-supervised learning~\citep{Ho2020SSLAdvExamples}, and image synthesis~\citep{Santurkar2019AdvImageSynthesis}. 

\noindent \textbf{Adversarial training.} 
Adversarial training~\citep{Goodfellow2014ExplainAdv, madry2017towards} still remains the most effective defense against adversarial examples. The performance of the baseline technique~\citep{madry2017towards} is further improved using adaptive loss functions~\citep{zhang2019tradeoff}, larger networks~\citep{gowal2020uncoveringadv}, pretraining~\citep{hendrycks2019AdvPretrain}, smooth activation function~\citep{xie2020smooth}, and weight perturbations~\citep{wu2020adversarial}. The fundamental min-max robust optimization behind adversarial training has also been successful in robustifying other model architectures, such as decision trees \citep{chen2019robustTree} and graph neural networks~\citep{feng2019AdvTraingraph}, while also extending to other domains like reinforcement learning~\citep{Gleave2020AdvRL} and natural language processing~\citep{liu2020advTrainNLP}.

\noindent \textbf{Progress on improving adversarial robustness.}
Improving adversarial robustness in deep neural networks remains a challenging problem and its progress has been slow, as tracked by the RobustBench~\citep{croce2020robustbench}. Following initial success of baseline adversarial training in \citep{madry2017towards}, robust accuracy has improved by only $12$\% in the setting where networks architecture is fixed to \wrn{28-10} and no extra real-world images are used (from $44.0$\% in \citet{madry2017towards} to $56.2$\% in \citet{wu2020adversarial}). Additionally, there have been more than twenty failed attempts in improving it over the baseline~\citep{croce2020robustbench}. To put our work in context, we further improve robust accuracy on the CIFAR-10 dataset to $59.5$\%, without using additional techniques like smooth activations or weight perturbations.


\noindent \textbf{Certified robustness.} Here the goal is to certify the robustness of each examples~\citep{Wong2018ScalingProve, cohen2019certified, Zhang2020crownIbp}. Certified robustness provides a lower bound on the adversarial robustness against all attacks in the threat model. We use randomized smoothing~\citep{cohen2019certified} to achieve certified robustness, since it achieves much better performance over other methods in this domain~\citep{cohen2019certified, carmon2019unlabeled}. Further improvements in randomized smoothing includes integration with adversarial training~\citep{salman2019AdvSmooth}, using sub-networks~\citep{sehwag2020Hydra}, and using sample-specific smoothing~\citep{alfarra2020dataDependSmooth}.

\subsection{Intriguing properties of adversarial training}

\noindent \textbf{Sample complexity of adversarial training.} Multiple earlier works provide theoretical results studying the effect of the number of training samples on adversarial robustness~\citep{wei2019allLayerMargin, bhagoji2019lowerBounds, schmidt2018AdvMoreData, chen2020dataHurtsAdv, min2020datahurts}. \citet{chen2020dataHurtsAdv} and \citet{min2020datahurts} further suggest that more data may hurt generalization in adversarial training. We explore this direction empirically by adversarial training deep neural networks on an increasing number of training images.

\noindent \textbf{Trade-off in adversarial training.} There also exists an accuracy vs robustness trade-off where improvement in robust accuracy comes at the cost of clean accuracy in adversarial training~\citep{Raghunathan2020advtradeoff, balaji2019instAdaptAdvtrain, javanmard2020preciseTradeoff}. We empirically demonstrate that increase in the number of training samples can significantly reduce this trade-off. 

\noindent \textbf{Transfer of adversarial robustness.}
This line of work focuses on the transfer of adversarial robustness, i.e., correct classification even under adversarial perturbations, when testing the model on different data distributions~\citep{shafahi2020AdvRobustTransfer, sehwag2019analyzing}. Note that this is different from just achieving correct classification on unmodified images across different distributions~\citep{taori2020NatShiftRobust, hendrycks2019CommonCorrupt}. Here we provide a theoretical analysis of the transfer of adversarial robustness between data distributions. 
%\vikash{Are we first to do it. Not likely. Can also include complementary works.}


\noindent \textbf{Using extra curated real-world data.} Prior works \citep{zhai2019advJustmoreData, carmon2019unlabeled, alayrac2019unsupadv, najafi2019advIncompleteData, deng2020AdvExtraOutDomain} have argued for using more training data in adversarial training and often resort to curating additional real-world samples. In contrast, we don't require additional real-world samples, as we model the proxy distribution from the limited training images available and sample additional synthetic images from this distribution. %In spirit, our approach is similar to techniques like mixup~\citep{zhang2018mixup, Pang2020MixupInfer}, which adds novel samples in training by interpolating along samples in the available training data. 


% Cite the result for the gaussian case. Cite min et al. for a more convoluted case. We put this to rest by conducting an experiment with 1k-10M training images. Some earlier works to study this are following: \citep{wei2019allLayerMargin, bhagoji2019lowerBounds, schmidt2018AdvMoreData}. 

% \noindent \textbf{More data in adversarial training.} Both \citep{chen2020dataHurtsAdv, min2020datahurts} provide theoretical results suggesting more data may hurt in adversarial training.  Empirically earlier work \citep{zhai2019advJustmoreData, carmon2019unlabeled, alayrac2019unsupadv, najafi2019advIncompleteData, deng2020AdvExtraOutDomain} have argued for using more data and often resort to curating additional real-world samples.

\subsection{Using generative models for proxy distributions}
\noindent \textbf{Generative models for proxy distributions.}
State-of-the-art generative models are capable of modeling the distribution of current large-scale image datasets. In particular, generative adversarial networks (GANs) have excelled at this task~\citep{goodfellow2014GAN, karras2020styleganAda, gui2020ganreview}. Though GANs generate images with high fidelity, they often lack high diversity~\citep{ravuri2019CAS}. However, samples from recently proposed diffusion process based models achieve both high diversity and fidelity~\citep{ho2020denoisingdiffusion, nichol2021improvedDdpm}.

\noindent \textbf{Evaluating quality of samples from a generative model.} Fréchet Inception Distance (FID)~\citep{Heusel2017FID} and Inception Score (IS)~\citep{Heusel2017FID} are two key metrics to evaluate the quality of samples from generative models. While IS considers only generated images, FID considers both generative and real-world images. We find that better FID or Inception score may not translate to higher robustness with synthetic data. Another line of work evaluates generative models by training a classifier on its generated samples and testing it on real-world data~\citep{ravuri2019CAS, semeniuta2018accGanEval}. \vikash{\url{https://www.cs.cmu.edu/~clean-fid/} More evidence on subtle nature of FID.}

\noindent \textbf{Using generative models to improve adversarial robustness.} Earlier works have used generative models to learn training data manifold and the use it to map input samples to data manifold~\citep{samangouei2018defenseGan, jalal2017robustmanifold, Xu2018featsqueeze}. However, most of these techniques are broken against adaptive attacks~\citep{athalye2018obfuscatedGrad, Tramer2020AdaptiveAttack}. We use generative models to sample additional training samples which lead to further improvement in adversarial robustness. 
%\vikash{Make sure we aren't missing any work here.}

\noindent \textbf{Additional applications of proxy distributions.} While we use proxy distributions to improve robustness, synthetic samples from proxy distributions are also useful in privacy-preserving healthcare~\citep{jordon2018pateGan}, autonomous driving~\citep{mayer2016synDriving}, crowd-counting~\citep{wang2019countCrowd}, text recognition~\citep{jaderberg2014synTextReco, ye2018AnotherCaptcha}, and natural language processing~\citep{marzoev2020unnaturalLangProcess, puri2020syntheticQA}. Earlier works have also created dedicated synthetic datasets for some of these applications~\citep{gaidon2016virtualkitti, mayer2018viewSynthetic}. \vikash{Add domain randomization citation.}

\noindent \textbf{Comparison with} \citep{rebuffi2021fixingaugmentation}\textbf{.}  A concurrent work by ~\citep{rebuffi2021fixingaugmentation} also uses samples from generative models to improve adversarial robustness. While it broadly focuses on the effect of different data augmentations, with synthetic samples from a proxy distribution being one of them, our goal is to delve deeper into the integration of proxy distribution in adversarial training. This includes providing tight bounds on the transfer of adversarial robustness from the proxy distribution followed by empirical analysis of the transfer of robustness, accuracy vs robustness trade-off, and sample complexity of adversarial training. We also demonstrate an improvement in certified robust accuracy using proxy distributions. However, despite the differences, similar benefits of using generative models in two independent works further ascertain the importance of this research direction. 
%\vikash{Go over todo list again.}
\vikash{Relate to active learning, core-set estimation. Relate to Sanjeev's Simons'17 talk on how bounded capacity discriminator can have hard time distinguishing this may not achieve sufficient diversity. We can also see if smaller networks can still distiguish between real and synthetic.}

==> sections/old_introduction.tex <==
Deep neural networks are powerful tools but their success depends strongly on the amount of training data~\citep{sun2017revisitData, mahajan2018BillionWSL}. 
Recent works show %have shown 
that for improving robust training against adversarial examples~\citep{biggio2013evasion, Szegedy2013IntrigueAdv, biggio2018wildPatterns}, additional training data is 
helpful~\citep{carmon2019unlabeled, schmidt2018AdvMoreData, alayrac2019unsupadv, deng2020AdvExtraOutDomain}.
However, curating more real-world data from the actual data distribution is usually 
challenging and costly~\citep{recht2019ImageNetv2}. 
To circumvent this challenge, we ask: can robust training be enhanced using a proxy distribution, i.e., an approximation of the \realdist distribution? 
In particular, can additional samples from a proxy distribution, that is perhaps cheaper to sample from, improve robustness. If so, can generative models that are trained on limited training images 
in small scale datasets~\citep{lecun2010mnist, krizhevsky2014cifar}, act as such a proxy distribution?\footnote{Proxy distributions may not necessarily be modeled by generative models. When a proxy distribution is the output of a generative model, we call it \emph{synthetic distribution} and refer to data sampled from it as \emph{synthetic data}.}

When training on synthetic samples from generative models, a natural question is whether robustness on synthetic data will also transfer to real world data. Even if it does, can we determine the features of synthetic data that enable this \emph{synthetic-to-real} robustness transfer and optimize our selection of generative models based on these features? Finally, can we also optimize the selection of individual synthetic samples to maximize the robustness transfer? \vikashnew{Rewrite it.}

\emph{Q.1} \emph{When does robustness transfer from proxy distribution to real data distribution?} This question is fundamental to develop a better understanding of whether a proxy distribution will help. \bluetext{For a classifier trained on only synthetic samples, we argue that in addition to empirical and generalization error, \emph{distribution shift} penalty also determines its robustness on the real data distribution.} We prove that this penalty is upper bounded by the \cwdfull between the \approxdist distribution and \realdist data distribution.

\emph{Q.2} \emph{\newtext{How effective are proxy distributions in boosting adversarial robustness on real-world dataset?}}
Our experimental results demonstrate that the use of samples from the Proxy distribution in Robust Training (PORT) can significantly improve robustness. We use \bluetext{state-of-the-art} \ddpm~\citep{ho2020denoisingdiffusion} model on CIFAR-10~\citep{krizhevsky2014cifar} dataset since it achieves the highest robustness transfer among seven generative models that we tested, and sample $10$M images from it based on the proposed synthetic score metric. \bluetext{Using this optimized set of images, PORT achieves up to $7.5$\% improvement in adversarial robustness over existing state-of-the-art~\citep{croce2020robustbench}.} \bluetext{We also observe that success of synthetic samples is dependent on the distribution of real data. Our analysis reveals that state-of-the-art in generative modeling on ImageNet~\citep{deng2009imagenet} dataset has not reached an inflection point where it leads to improvement in robustness.}







% \saeed{do we need both "synthetic" and "proxy"? Can we use just one of them?}?

% . We prove that difference between the average robustness of a classifier on the \approxdist and \realdist distribution is upper bounded by the \cwdfull between them. 
% It validates that intuition that \approxdist distributions that closely approximate \realdist distribution should be able to improve robustness on the latter. 
% In other words, samples from a proxy distribution that is indistinguishable from \realdist distribution\saeed{This is tricky to say. Inistinguishability has a formal meaning and it does not necessarily imply robustness. It is also clear from some of our experiments. Isn't the first sentence sufficient?} should be helpful. 
Thus robustness will transfer from proxy distributions that are in close proximity to \realdist distribution with respect to \cwdfull. 

% Next, we delve deeper into the question of which proxy distribution to choose and can our theoretical results inspire an effective selection criterion. Though CWD can't be computed exactly, since real data distribution is generally not known, it motivates the use of proxy distribution close to \realdist distribution. But how do we empirically measure proximity?

\emph{Q.2} \emph{Can we empirically predict robustness transfer from synthetic-to-real data?} Though \cwdfull can predict robustness transfer, calculating it requires knowledge of the underlying distribution of \realdist which is generally not known. Our theory motivates the design of a measure of proximity between two empirical distributions that incorporates the geometry of the distributions and can empirically predict transfer of robustness.
% But how do we empirically measure the proximity of synthetic and real samples?
We first test existing distance metrics: Euclidean distance between synthetic samples and nearest real samples as well as the widely used Fréchet Inception Distance (FID)~\citep{Heusel2017FID}.
% We first test existing distance metrics. A simple baseline is to use Euclidean distance of synthetic samples to nearest real samples. Another widely used distance metric is Fréchet Inception Distance (FID)~\citep{Heusel2017FID}
%\footnote{ In general, calculating FID is as hard as calculating \cwdfull. However prior work measure the FID of two distributions in \emph{feature space} by first fitting a Gaussian distribution and then calculating the distance between Gaussians. This is what we refer to as FID.}. 
In our analysis with \textit{seven} different generative models, we find that both metrics predict robustness transfer incorrectly for more than half of the models.
%As euclidean distance is neither necessary nor sufficient to capture semantic differences~\citep{sharif2018lpNormsNotSuitable}, it fails to predict the transfer of performance from synthetic-to-real data. \saeed{we can stop this para here. It will not be clear to a general audience what the next few sentences mean.} 
%A widely used metric is Fréchet Inception Distance (FID), which measures Fréchet distance between synthetic and real data in the feature space of an Inception v3 network trained on the ImageNet dataset. Apparently, FID performs even \emph{worse} than nearest neighbour distance. 

We propose a robust learning based approach where we use the success of a discriminator in distinguishing adversarially perturbed samples of synthetic and real data as a measure of proximity. Discriminating between synthetic and real data is a common practice~\citep{goodfellow2014GAN, gui2020ganreview}. 
\bluetext{However, we find that considering adversarial perturbations on synthetic and real data samples is the key to making the discriminator an effective measure for this task.}
%However, we find that its the robust learning against adversarial perturbations that makes the discriminator success an effective measure for this task. 
We demonstrate that the rate of decrease in discriminator success with an increasing size of perturbations can effectively measure proximity and it accurately predicts the relative transfer of robustness from different generative models. 

% $\epsilon$-expanded sets of synthetic and real data as a measure of proximity. We expand these sets, as without them even a four-layer convolutional network achieves near-perfect classification accuracy on all seven proxy distributions we considered. For samples at close proximity, even small values of $\epsilon$ will lead to ball intersection, making the classification infeasible. We demonstrate that the rate of decrease in discriminator success with an increasing value of $\epsilon$ can effectively measure proximity where it accurately predicts the relative transfer of robustness from different generative models. 


% We take a learning-based approach where we use success of disc how well a deep neural network can distinguish these two sets of samples. It turns out that deep networks almost perfectly distinguish all proxy distributions from real data, irrespective of their proximity, in our experiments. To make discrimination success dependent on proximity, we expand our samples by adding perturbations bounded by a $\ell_{p}$ ball. Now the objective is to correctly classify all samples within the $\ell_p$ ball. Thus proxy distributions at close proximity will have an intersection with \realdist data distribution even under a small perturbation budget. We use the discriminator success at increasing perturbation budgets and demonstrate that it accurately predicts synthetic-to-real performance transfer. \vikash{Add a link to theory.}

% \saeed{Can we optimize the proxy distribution base on our metric?}
\emph{Q.3} \emph{Can we optimize on which synthetic samples to choose?} We find that some samples lead to higher robustness transfer than others from a proxy distribution. Understanding this sample-wise importance can enable us to adaptively sample the most helpful data points. We use the proximity of each synthetic sample to \realdist distribution, referred to as \textit{synthetic score}, as a metric to judge their importance. This score can be computed using output probability from a discriminator that is robustly trained to distinguish between adversarially perturbed samples from \approxdist and \realdist distribution. We use rejection sampling based on this score where we discard samples with a score higher than a predetermined threshold. 

% A lower synthetic score implies a small distance to \realdist data distribution. As we experimentally demonstrate, samples with the lowest synthetic score contribute most to synthetic-to-real performance transfer. Using synthetic score as a criterion, we adaptively sample a large set of synthetic samples and demonstrate that it improves performance over real data compared to a randomly sampled set of synthetic images. 

% \saeed{Alternative question: Can we use enumerate environment instead of saying Q1, Q2...} \saeed{ our optimized sample generation improves ...} 
\emph{Q.4} \emph{Finally, how effective are proxy distributions in boosting adversarial robustness?}
Our experimental results demonstrate that the use of samples from the Proxy distribution in Robust Training (PORT) can significantly improve robustness. We use \bluetext{state-of-the-art} \ddpm~\citep{ho2020denoisingdiffusion} model on CIFAR-10~\citep{krizhevsky2014cifar} dataset since it achieves the highest robustness transfer among seven generative models that we tested, and sample $10$M images from it based on the proposed synthetic score metric. \bluetext{Using this optimized set of images, PORT achieves up to $7.5$\% improvement in adversarial robustness over existing state-of-the-art~\citep{croce2020robustbench}.} \bluetext{We also observe that success of synthetic samples is dependent on the distribution of real data. Our analysis reveals that state-of-the-art in generative modeling on ImageNet~\citep{deng2009imagenet} dataset has not reached an inflection point where it leads to improvement in robustness.}


% While for the MNIST~\citep{lecun2010mnist} dataset samples from an \bluetext{elementary} deep convolutional GAN~\citep{radford2015dcgan} suffice, even state-of-the-art models, including \ddpm, fail to bring any improvement on the ImageNet dataset. {\color{red} Update this.}

% Using these samples, we improve robust accuracy by up to $7.5$\% and $6.7$\% in $l_{\infty}$ and $l_2$ threat models, respectively, over baselines not using proxy distributions on the CIFAR-10 dataset. 
%In the category of not using any extra real-world data, our models achieve the first rank on RobustBench~\citep{croce2020robustbench} \saeed{I think this violates the anonymity. Let's remove it.}, a standardized benchmark for adversarial training. 
% We also improve the certified robust accuracy~\citep{cohen2019certified} by up to $7.6$\% with randomized smoothing on the CIFAR-10 dataset. \vikash{Add MNIST, ImageNet results when they are available.} \vikash{Does using roubustbench info violates double blind submission policies?}

% \saeed{I feel like the contributions below are a bit redundant. Can we merge them with paragraphs above? another idea is to move it to conclusion section.}
\noindent \textbf{Contributions.}
We make the following key contributions.
\begin{itemize}[noitemsep, topsep=0pt]
    \item We provide an analytical bound on the transfer of robustness from proxy distributions to \realdist distribution and further validate it experimentally.
    \item In selecting proxy distribution, we show that existing metrics, such as FID, fail to determine the synthetic-to-real transfer of robustness. We propose a new metric (\emph{\aurpc}) based on the distinguishability of adversarially perturbed synthetic and real data, that accurately determines the performance transfer.  
    \item We also develop a metric, named \emph{synthetic score}, to determine the importance of each synthetic sample in synthetic-to-real robustness transfer. We demonstrate that choosing samples with lower synthetic scores provide better results than randomly selected samples. 
    \item Overall, using additional synthetic images sampled from \approxdist distributions, we improve robust accuracy by up to $7.5$\% and $6.7$\% in $\ell_{\infty}$ and $\ell_2$ threat models, respectively, and certified robust accuracy ($\ell_2$) by $7.6$\% on the CIFAR-10 dataset. \bluetext{We also improve clean accuracy, simultaneously.}
\end{itemize}

%  given high expressive power of deep network, 
%Given dataset bias, ImageNet trained network may not best capture semantics of CIFAR-10 classes, so we also measure FID in the feature space of a 
% which measure proximity of synthetic samples to real data,
% In our analytical results, we use \cwdfull between synthetic and \realdist distribution to determine this. 
% However underlying distribution of \realdist is unknown, making it infeasible to calculate this bound. 


% To achieve robustness against adversarial examples, adversarial training remains the most effective technique~\citep{madry2017towards, zhang2019tradeoff, pang2021bagoftricks}. However, it is largely used with limited training samples available in current image datasets (such as only 50,000 training images in the CIFAR-10 dataset) where it suffers from multiple challenges, such as poor generalization on the test set~\citep{madry2017towards} and accuracy vs robustness trade-off~\citep{Raghunathan2020advtradeoff}. Recent works have demonstrated that more training data can improve the performance of adversarial training~\citep{schmidt2018AdvMoreData, alayrac2019unsupadv, deng2020AdvExtraOutDomain}. However, this approach runs into the challenge of curating a large set of real-world images for training. We circumvent this challenge using proxy distributions, distributions that closely approximate the underlying distribution of the original training dataset. Note that the proxy distributions are modeled using only available training images in current datasets. Proxy distributions when modeled with deep neural networks, such as Generative adversarial networks (GAN), allow us to generate a potentially unlimited number of high-fidelity images~\citep{goodfellow2014GAN, gui2020ganreview, ho2020denoisingdiffusion}. Our key goal is to improve the adversarial robustness of deep neural networks by taking advantage of samples from such proxy distributions.

% Note that proxy distributions are only an approximation of the underlying distribution of the training data. This begs the question of whether robustness achieved on samples from the proxy distribution will transfer to the original dataset. A more generic version of this question is \textit{how much the robustness of a classifier transfers between data distributions?} We prove that the difference in the robustness of a classifier on two distributions is \textit{tightly} upper bounded by the conditional Wasserstein distance between them. We refer to Wasserstein distance conditioned on class labels as conditional Wasserstein distance. This result confirms the intuition that samples from a proxy distribution that closely approximates training data distribution should be able to improve robustness on the latter. We also empirically validate this claim where we show that adversarial training only on samples from the proxy distribution indeed achieves non-trivial robustness on samples from the original distribution. 

% To improve adversarial robustness on current datasets, we aim to leverage samples from a \approxdist distribution which \textit{closely} approximates the underlying distribution of these datasets. Here we propose to simultaneously train on both the original training set and a set of additional images sampled from the \approxdist distribution. We use state-of-the-art generative models as a model for proxy distribution since they can closely approximate the data distribution from only a limited number of training samples~\citep{karras2020styleganAda, ho2020denoisingdiffusion, gui2020ganreview}.  Our experimental results demonstrate that the use of samples from the proxy distribution improves robust accuracy by up to $6.1$\% and $5.7$\% in $l_{\infty}$ and $l_2$ threat models, respectively, over baselines not using proxy distributions on the CIFAR-10 dataset. In the category of not using any extra real-world data, our models achieve the first rank on RobustBench~\citep{croce2020robustbench}, a standardized benchmark for adversarial training. We also improve the certified robust accuracy~\citep{cohen2019certified} by up to $6.7$\% with randomized smoothing on the CIFAR-10 dataset. Intriguingly, we achieve better certified robust accuracy with proxy distribution samples than using an additional set of $500$K curated real-world images~\citep{carmon2019unlabeled}.

% Since access to proxy distributions gives us the ability to generate a large number of images, this allows us to delve deeper into the relationship of adversarial robustness with the number of training samples on the scale of image classification with deep neural networks. Next, we work solely with a proxy distribution, where we train multiple networks with an increasing amount of training images (we use $2$K-$10$M training images) and test each on another fixed set of images from it. Our goal is to analyze multiple intriguing properties of the adversarial training w.r.t. the number of training samples. We first analyze the sample complexity of adversarial training. Earlier works \citep{wei2019allLayerMargin, bhagoji2019lowerBounds, schmidt2018AdvMoreData} have derived sample complexity bounds in simplified settings such as classifying a mixture of Gaussian distributions. On the scale of deep neural networks for image classification, we empirically demonstrate that more data continues to improve adversarial robustness. 
% %%Recently, \citep{chen2020dataHurtsAdv} and \citep{min2020datahurts} provided theoretical results suggesting more data may hurt generalization in adversarial training. We observe that both clean and robust generalization continue to improve with the number of training samples. 
% Next, we analyze the accuracy vs robustness trade-off: earlier works showed that robustness in adversarial training is achieved at a cost of clean accuracy of deep neural networks~\citep{Raghunathan2020advtradeoff, javanmard2020preciseTradeoff}. We demonstrate that increase in the number of training samples significantly reduces this trade-off for deep neural networks. To the best of our knowledge, this is the \textit{first} empirical investigation into adversarial training of deep neural networks on millions of images on the scale of CIFAR-10 dataset. \vikash{Add a summary of key results in a table.}

%% However, without access to the training data distribution, we are bounded by the limited training images available in these datasets. We aim to circumvent this issue using proxy distributions. We refer to approximations of the underlying distribution of these datasets as proxy distributions. Since we have access to this distribution, we can now sample a potentially unlimited number of samples from it, overcoming the challenges of limited training samples in current datasets\Snote{why do we have unlimited access to proxy distributions? would be good to elaborate on this.}.} 

%% \Snote{We can make a better connection to next sentense here. For example, saying generalization requires more data->we don't have more data -> we have proxy data} In this work, we analyze adversarial training through the lens of \textit{proxy} distributions. 
% We refer to approximations of the underlying distribution of these curated datasets as proxy distributions. In contrast to the limited number of training samples in the current dataset, we can now sample a potentially unlimited number of images from the proxy distribution. Our key goals are following. 

%% \bluetext{Our key goal is to improve the performance of adversarial training using samples from the proxy distribution. Though this integration looks straightforward, it poses multiple intriguing questions. Since the key advantage of a proxy distribution is to allow sampling of unlimited data points, the first question is how much does increase the number of training samples help in adversarial training on deep neural networks? Note that our goal is to improve robustness on the underlying data distribution of the training dataset. Proxy distributions remain an approximation of the underlying data distribution. So even if more training images improve robustness significantly, would it help if they are sampled from a proxy distribution? Finally, if we have a proxy distribution which closely approximates training data distribution, how can we use it to improve the performance of adversarial training. We delve deeper into each question individually below.}

%% Our next key objective is to utilize synthetic samples, i.e., samples from the proxy distribution, to improve robustness on current image datasets. However, proxy distribution is only an approximation of the true distribution of image datasets. Thus, it's unclear whether robustness acquired for proxy distribution will transfer to samples from the true data distribution. This motivates us to pursue the following goal. 

%% However, adversarially trained networks, when trained on a limited number of images available in curated datasets such as CIFAR-10~\citep{krizhevsky2009learning}, suffers from a large generalization gap in robust accuracy. In this work, we approach adversarial training on these datasets in conjunction with a \textit{proxy} distribution. We refer to approximations of the underlying distribution of these curated datasets as proxy distributions. Our use of proxy distributions allows us to target the following two objectives. 1) Since we can sample an unlimited number of samples from the proxy distribution, it allows us to investigate the effect of the number of training samples on the robust generalization of adversarial training 2) Using samples from proxy distribution to reduce the robust generalization gap in adversarial training.

%% \Snote{Alternative Questions for 1. Question 1: Can we achieve robustness on proxy distributions by performing adversarial training on large datasets sampled from them? }
%% \noindent \textbf{Q.} \textit{How does increasing number of training samples benefit adversarial training in \Snote{Maybe we can say "image classification" instead of "deep neural networks"} deep neural networks?}
%% % \noindent \textbf{Goal-1.} \textit{An empirical investigation into intriguing properties of adversarial training in the limit of infinite training samples.}
%% \bluetext{\Snote{Maybe we can say: our first step in investigating our main goal is to explore the case where proxy distribution is exactly the same as data distribution. }We aim to answer this question by analyzing intriguing properties of adversarial training on networks training on increasing number of training samples (we use 5k-10M training samples)}. We first analyze the sample complexity of adversarial training. Earlier works \citep{wei2019allLayerMargin, bhagoji2019lowerBounds, schmidt2018AdvMoreData} have derived sample complexity bounds in simplified settings such as classifying a mixture of Gaussian. We empirically demonstrate that more data continues to improve adversarial robustness but at a slower rate than clean accuracy. Recently, \citep{chen2020dataHurtsAdv, min2020datahurts} provide theoretical results suggesting more data may hurt generalization in adversarial training. We observe that both clean and robust generalization continues to improve with the number of training samples. Finally, we analyze the accuracy vs robustness trade-off where earlier works showed that robustness in adversarial training is achieved at a cost of clean accuracy of deep neural networks~\citep{Raghunathan2020advtradeoff, javanmard2020preciseTradeoff}. \textcolor{red}{rephrase: We demonstrate that increase in training samples can mitigate this trade-off for deep neural networks. }

%% We first investigate the effect of the number of training samples in adversarial training. Earlier works~\citep{carmon2019unlabeled, alayrac2019unsupadv} demonstrated improved generalization of adversarial training by expanding the training dataset size using an additional set of curated images. Recently~\citet{min2020datahurts} argued that more training data can both help or hurt generalization based on the strength of the adversary in adversarial training. However,~\citet{min2020datahurts} works with simple problems such as Gaussian mixture classification or a two-dimensional classification. It remains unclear how adversarial training behaves with the number of samples on the scale of computer vision tasks and deep neural networks. We answer this question by training a deep neural network on an increasing number of images (ranging from $1$K to $2$M). We observe that both clean and robust test accuracy continues to improve with the number of samples. 

%% \noindent \textbf{Q.} \textit{When does adversarial robustness transfers between two data distributions?}

%% We study this problem in a generic setting where we adversarially train a classifier on one data distribution and test on another distribution. We prove that the difference in robustness of a classifier on the two distributions is \textit{tightly} upper bounded by the conditional Wasserstein distance between them. It confirms the intuition that samples from a proxy distribution that closely approximates training dataset distribution should be able to boost robustness. We also empirically validate this intuition where we show that adversarial training on samples from the proxy distribution indeed achieves non-trivial robustness with samples from the true distribution.  

%% Next, we ask when incorporating additional samples from the proxy distribution will help in improving robustness on datasets such as CIFAR-10? Here we provide a theoretical analysis on how robustness of a classifier trained on one distribution transfers to the other. In particular, we prove that the difference in robustness of a classifier on the two distributions is upper bounded by the Wasserstein distance between them. It confirms the intuition that samples from a proxy distribution that closely approximates training dataset distribution should be able to boost robustness. \vikash{Cite empirical results also where training on synthetic brings robustness on CIFAR-10 itself.}

%% Our work focuses on this generalization gap with a two-fold goal: 1) Develop a deeper understanding of generalization of robustness between distributions 2) Making further improvements in closing this generalization gap.

%% To understand the generalization of robustness we work with the following generic setting. We assume access to two data distributions. First is the \textit{source} distribution on which we train the model, and second is the \textit{target} distribution, a shifted version of the source distribution, on which we test the model. This setting also allows us to model scenarios where inference time inputs are not exactly respecting training distribution, as often is the case in real-world deployment (cite ood) or even in independent replication of classic datasets (cite).

%% We find that robustness is much harder to generalize than clean accuracy between the two distributions. We train multiple models with an increasing number of training samples from the source distribution and test on samples from the target distribution. While clean accuracy improves consistently with an increase in training samples, improvement in robust accuracy is much smaller. To further understand the relationship between robustness on these two distributions, we complement our experiments with a theoretical analysis. In particular, we prove that the difference in robustness on these two distributions is upper bounded by the Wasserstein distance between them. This result verifies the intuition that robustness achieved on one distribution can transfer to another distribution, if they are close, at test time. 

%% \noindent \textbf{Q.} \textit{How to improve state-of-the-art in adversarial training using proxy distributions?}

%% \noindent \textbf{Contributions.} We make the following key contributions.
%% \begin{itemize}
%%     \item We provide a theoretical understanding as well as an empirical validation of the transfer of adversarial robustness between data distributions. In particular, we provide a tight upper bound on the difference between the robustness of a classifier on two data distributions. 
%%     \item We propose to combine adversarial training with proxy distributions. By leveraging additional images sampled from \approxdist distributions, we improve robust accuracy by up to $6.1$\% and $5.7$\% in $l_{\infty}$ and $l_2$ threat models, respectively, and certified robust accuracy by $6.7$\% on the CIFAR-10 dataset.
%%     \item We provide the \textit{first} large scale empirical investigation of accuracy vs robustness trade-off and sample complexity of adversarial training by training deep neural networks on $2$K to $10$M images.
% \end{itemize}

%% 1) We investigate the effect of increasing number of training samples (from $1$K to $2$M) on the performance of adversarial training with deep neural networks,  2) we provide theoretical insights on how robustness of a classifier on one distribution transfer to another distribution. In particular, we provide a tight upper bound on the difference of the robustness of a classifier between the distributions, and 3) by leveraging additional images sampled from the \approxdist distributions, we improve robust accuracy up to $6.5$\% and $5.0$\% in $l_{\infty}$ and $l_2$ threat model, respectively, on the CIFAR-10 dataset.

%% In robust ML goal is to make robust. However there remain a large generalization gap between training and test data. In understand the generalization we assume this generic setting. two distributions: source distribution on which model is trained and target on which model is tested. We assume some shift between them, which can easily occur in real-world application or even in a replication effort. Two fold goal: 1) Understand the generalization of robustness between shifted distribution 2) Taking advantage of another shifted distribution when available. 

%% We find that robustness is much harder to generalize than clean accuracy. Here we training different models with increasing number of samples from source distribution and test on both source and target. While clean accuracy on target consistently improves, robust accuracy improves super slowly. This shed light on how small distribution shift can adversely effect generalization of robustness. Intriguing question is how does robustness on these two distributions relate. Here, we prove an upper bound on the robustness gap, which is only a function of distribution distance. Verifying the intuition that smaller distribution shift will lead to smaller generalization gap. 

%% Motivated by aforementioned results, we now seek to take advantage proxy distributions, i.e., distribution closely approximating original distribution, in order to close the gap between train and test set. We find that recent generative models, closely approximate source distribution on dataset such as CIFAR-10. A test we do is to robustly train on them and test on original and these model achieve a highly non-trivial performance. 

%% Here we first use training set to train the generative models, followed by sampling a specified set of synthetic images. Next we combine these synthetic images with original training test, and robustly trained a classifier. Our experimental results demonstrate that use of synthetic images improves robustness accuracy up to 6.4\% on CIFAR-10 dataset. We observe such improvements across different networks architectures and threat models. 


%% Generalization in robust machine learning is hard, between training and test set. We study it in more generic setting where we look into generalization between two slightly shifted distributions. Slight distribution shift can happen, practical or just replication efforts. |||||
%% understanding Robustness - Robustness is hard to generalize between distributions. However we prove that such difference is upper bounded by a distance. ||||| 
%% Improving robustness - On baseline dataset. Motivate this by saying that closely approximated distribution can generalize robustness to baseline distribution. We find that recent generative model achieve this and we use them. |||||
%% Discussion  - Future work should focus on bringing two distributions closer. 
%% \begin{itemize}
%%     \item Goal improve adversarial robustness. Similar to supervised, more data helps with robust learning. While exactly replicating original distribution is hard (Berkeley paper) - proper calibration, cleaning etc, an approximate distribution can be obtained. This could be an generating model approximating/\approxdist original data. Our goal is to leverage shifted/synthetic distribution to improve adversarial robustness.  
%%     \item Our first step is to understand the impact of synthetic/original distribution overlap on transfer of robustness between them. Here we prove that robustness on synthetic and original dataset is upper bounded by distribution distance. It supported the hypothesis that when synthetic distribution closely approximate the true distribution, it can help improving robustness (big leap from generalization to help)
%%     \item 
%% \end{itemize}

